Bayesian inference of T Tauri star properties using multi-wavelength survey photometry

There are many pertinent open issues in the area of star and planet formation. Large statistical samples of young stars across star-forming regions are needed to trigger a breakthrough in our understanding, but most optical studies are based on a wide variety of spectrographs and analysis methods, which introduces large biases. Here we show how graphical Bayesian networks can be employed to construct a hierarchical probabilistic model which allows pre-main sequence ages, masses, accretion rates, and extinctions to be estimated using two widely available photometric survey databases (IPHAS r/i/Halpha and 2MASS J-band magnitudes.) Because our approach does not rely on spectroscopy, it can easily be applied to homogeneously study the large number of clusters for which Gaia will yield membership lists. We explain how the analysis is carried out using the Markov Chain Monte Carlo (MCMC) method and provide Python source code. We then demonstrate its use on 587 known low-mass members of the star-forming region NGC 2264 (Cone Nebula), arriving at a median age of 3.0 Myr, an accretion fraction of 20+/-2% and a median accretion rate of 10^-8.4 Msol/yr. The Bayesian analysis formulated in this work delivers results which are in agreement with spectroscopic studies already in the literature, but achieves this with great efficiency by depending only on photometry. It is a significant step forward from previous photometric studies, because the probabilistic approach ensures that nuisance parameters, such as extinction and distance, are fully included in the analysis with a clear picture on any degeneracies.

==> tables/table_param.tex <==
C11059 & $-0.41 \pm 0.44$ & $-0.61 \pm 0.08$ & $6.91 \pm 0.09$ & $1.45 \pm 0.54$ & $-4.5 \pm 0.6$ &  & \\
C11997 & $-0.39 \pm 0.40$ & $-0.49 \pm 0.07$ & $6.50 \pm 0.10$ & $1.79 \pm 0.16$ & $-3.6 \pm 0.2$ & $-9.1 \pm 0.8$ & CTTS\\
C12135 & $-0.33 \pm 0.38$ & $-0.51 \pm 0.07$ & $6.77 \pm 0.09$ & $-0.20 \pm 0.85$ & $-5.8 \pm 0.9$ &  & \\
C12598 & $0.27 \pm 0.39$ & $-0.18 \pm 0.17$ & $6.56 \pm 0.31$ & $1.59 \pm 0.86$ & $-3.1 \pm 1.0$ & $-8.5 \pm 1.4$ & CTTS\\
C13507 & $0.19 \pm 0.73$ & $-0.34 \pm 0.28$ & $6.83 \pm 0.44$ & $1.41 \pm 2.86$ & $-3.8 \pm 3.0$ & $-8.8 \pm 3.3$ & CTTS\\
C14005 & $-0.42 \pm 0.42$ & $-0.41 \pm 0.07$ & $6.28 \pm 0.07$ & $0.49 \pm 1.13$ & $-4.5 \pm 1.2$ &  & \\
C15152 & $-0.33 \pm 0.40$ & $-0.36 \pm 0.09$ & $6.12 \pm 0.08$ & $-0.61 \pm 1.18$ & $-5.3 \pm 1.2$ &  & \\
C15247 & $-0.48 \pm 0.41$ & $-0.29 \pm 0.10$ & $6.59 \pm 0.19$ & $1.00 \pm 0.98$ & $-3.9 \pm 1.0$ &  & \\
C15285 & $0.21 \pm 0.27$ & $-0.32 \pm 0.14$ & $7.04 \pm 0.24$ & $-0.86 \pm 0.92$ & $-6.2 \pm 0.9$ &  & \\
C15519 & $-0.36 \pm 0.45$ & $-0.32 \pm 0.12$ & $6.27 \pm 0.13$ & $-0.44 \pm 1.44$ & $-5.2 \pm 1.5$ &  & \\
C16567 & $0.30 \pm 0.32$ & $-0.25 \pm 0.16$ & $6.96 \pm 0.33$ & $-0.90 \pm 1.02$ & $-6.0 \pm 1.1$ &  & \\
C16928 & $0.38 \pm 0.32$ & $-0.33 \pm 0.17$ & $7.03 \pm 0.27$ & $-0.76 \pm 0.91$ & $-6.1 \pm 1.0$ &  & \\
C17553 & $-0.31 \pm 0.41$ & $-0.44 \pm 0.10$ & $6.53 \pm 0.16$ & $-0.39 \pm 0.99$ & $-5.6 \pm 1.0$ &  & \\
C17614 & $-0.27 \pm 0.40$ & $-0.38 \pm 0.10$ & $6.68 \pm 0.15$ & $2.00 \pm 0.11$ & $-3.2 \pm 0.2$ & $-8.7 \pm 0.7$ & CTTS\\
C18487 & $-0.32 \pm 0.47$ & $-0.47 \pm 0.10$ & $6.53 \pm 0.10$ & $1.76 \pm 0.21$ & $-3.6 \pm 0.3$ & $-9.1 \pm 0.8$ & CTTS\\
C18627 & $-0.13 \pm 0.46$ & $-0.32 \pm 0.15$ & $6.05 \pm 0.13$ & $1.96 \pm 0.47$ & $-2.6 \pm 0.5$ & $-7.4 \pm 1.0$ & CTTS\\
C18688 & $-0.43 \pm 0.38$ & $-0.48 \pm 0.06$ & $6.77 \pm 0.08$ & $0.02 \pm 0.93$ & $-5.5 \pm 0.9$ &  & \\
C19191 & $-0.58 \pm 0.36$ & $-0.28 \pm 0.08$ & $6.97 \pm 0.20$ & $0.22 \pm 1.11$ & $-5.0 \pm 1.1$ &  & \\
C19299 & $-0.01 \pm 0.28$ & $-0.27 \pm 0.11$ & $7.08 \pm 0.26$ & $-0.81 \pm 0.89$ & $-6.0 \pm 0.9$ &  & \\
C19556 & $-0.47 \pm 0.42$ & $-0.80 \pm 0.13$ & $6.52 \pm 0.14$ & $1.94 \pm 0.21$ & $-4.2 \pm 0.3$ & $-9.8 \pm 0.8$ & CTTS\\
C19649 & $-0.42 \pm 0.46$ & $-0.42 \pm 0.11$ & $6.44 \pm 0.20$ & $0.70 \pm 1.06$ & $-4.4 \pm 1.1$ &  & \\
C19751 & $-0.41 \pm 0.38$ & $-0.56 \pm 0.06$ & $6.85 \pm 0.09$ & $2.69 \pm 0.09$ & $-3.1 \pm 0.1$ & $-8.4 \pm 0.7$ & CTTS\\
C19877 & $-0.42 \pm 0.36$ & $-0.24 \pm 0.11$ & $6.31 \pm 0.18$ & $-0.77 \pm 1.10$ & $-5.4 \pm 1.1$ &  & \\
C20156 & $-0.25 \pm 0.43$ & $-0.41 \pm 0.10$ & $6.90 \pm 0.14$ & $2.24 \pm 0.10$ & $-3.2 \pm 0.2$ & $-8.7 \pm 0.7$ & CTTS\\
C20254 & $-0.41 \pm 0.39$ & $-0.46 \pm 0.06$ & $6.38 \pm 0.07$ & $-0.12 \pm 1.02$ & $-5.3 \pm 1.0$ &  & \\
C20428 & $-0.34 \pm 0.40$ & $-0.53 \pm 0.08$ & $6.54 \pm 0.07$ & $-0.24 \pm 0.89$ & $-5.8 \pm 0.9$ &  & \\
C20504 & $0.41 \pm 0.51$ & $-0.31 \pm 0.29$ & $6.29 \pm 0.52$ & $1.60 \pm 0.86$ & $-3.0 \pm 1.2$ & $-8.1 \pm 1.7$ & CTTS\\
C20506 & $-0.37 \pm 0.39$ & $-0.42 \pm 0.07$ & $6.60 \pm 0.09$ & $1.84 \pm 0.14$ & $-3.4 \pm 0.2$ & $-9.0 \pm 0.7$ & CTTS\\
C20522 & $0.41 \pm 0.26$ & $-0.21 \pm 0.18$ & $6.52 \pm 0.38$ & $-1.53 \pm 1.06$ & $-6.2 \pm 1.1$ &  & \\
C20623 & $-0.41 \pm 0.46$ & $-0.62 \pm 0.13$ & $6.52 \pm 0.14$ & $0.30 \pm 0.95$ & $-5.4 \pm 1.0$ &  & \\
C20696 & $-0.39 \pm 0.41$ & $-0.58 \pm 0.08$ & $6.70 \pm 0.09$ & $2.15 \pm 0.11$ & $-3.6 \pm 0.2$ & $-9.2 \pm 0.7$ & CTTS\\
C20824 & $-0.42 \pm 0.41$ & $-0.53 \pm 0.07$ & $6.67 \pm 0.08$ & $0.79 \pm 0.91$ & $-4.8 \pm 0.9$ &  & \\
C20830 & $-0.40 \pm 0.42$ & $-0.72 \pm 0.13$ & $6.99 \pm 0.14$ & $2.08 \pm 0.13$ & $-4.2 \pm 0.3$ & $-10.1 \pm 0.8$ & CTTS\\
C20939 & $-0.49 \pm 0.38$ & $-0.19 \pm 0.06$ & $7.46 \pm 0.28$ & $-0.66 \pm 0.96$ & $-5.8 \pm 0.9$ &  & \\
C21090 & $-0.38 \pm 0.48$ & $-0.42 \pm 0.14$ & $5.49 \pm 0.27$ & $0.93 \pm 1.12$ & $-3.5 \pm 1.2$ &  & \\
C21202 & $-0.48 \pm 0.45$ & $-0.60 \pm 0.13$ & $6.05 \pm 0.18$ & $0.03 \pm 1.06$ & $-5.3 \pm 1.0$ &  & \\
C21501 & $-0.21 \pm 0.49$ & $-0.32 \pm 0.13$ & $6.31 \pm 0.18$ & $1.36 \pm 0.93$ & $-3.4 \pm 1.0$ & $-8.9 \pm 1.6$ & CTTS\\
C21607 & $-0.35 \pm 0.47$ & $-0.57 \pm 0.12$ & $6.76 \pm 0.12$ & $1.82 \pm 0.18$ & $-3.9 \pm 0.3$ & $-9.7 \pm 0.8$ & CTTS\\
C21959 & $-0.40 \pm 0.35$ & $-0.29 \pm 0.09$ & $6.53 \pm 0.16$ & $-0.68 \pm 1.08$ & $-5.6 \pm 1.1$ &  & \\
C22078 & $-0.31 \pm 0.38$ & $-0.62 \pm 0.09$ & $6.86 \pm 0.10$ & $-0.17 \pm 0.70$ & $-6.1 \pm 0.7$ &  & \\
C22226 & $-0.45 \pm 0.41$ & $-0.51 \pm 0.09$ & $6.36 \pm 0.12$ & $0.00 \pm 1.07$ & $-5.3 \pm 1.1$ &  & \\
C22323 & $-0.45 \pm 0.43$ & $-0.66 \pm 0.09$ & $6.52 \pm 0.06$ & $0.24 \pm 0.94$ & $-5.6 \pm 0.9$ &  & \\
C22348 & $-0.17 \pm 0.52$ & $-0.41 \pm 0.13$ & $6.05 \pm 0.10$ & $1.72 \pm 0.60$ & $-3.0 \pm 0.7$ & $-8.0 \pm 1.2$ & CTTS\\
C22501 & $-0.09 \pm 0.72$ & $-0.18 \pm 0.20$ & $6.41 \pm 0.33$ & $-0.49 \pm 2.63$ & $-5.0 \pm 2.9$ &  & \\
C22751 & $-0.18 \pm 0.43$ & $-0.34 \pm 0.15$ & $6.32 \pm 0.27$ & $-0.80 \pm 1.21$ & $-5.6 \pm 1.3$ &  & \\
C22982 & $-0.59 \pm 0.35$ & $-0.08 \pm 0.10$ & $6.64 \pm 0.30$ & $-0.40 \pm 1.00$ & $-4.9 \pm 1.0$ &  & \\
C23000 & $-0.43 \pm 0.39$ & $-0.67 \pm 0.08$ & $6.40 \pm 0.06$ & $-0.15 \pm 0.78$ & $-5.9 \pm 0.8$ &  & \\
C23061 & $-0.03 \pm 0.49$ & $-0.34 \pm 0.15$ & $6.41 \pm 0.17$ & $2.19 \pm 0.38$ & $-2.7 \pm 0.5$ & $-7.8 \pm 0.9$ & CTTS\\
C23131 & $0.16 \pm 0.38$ & $-0.15 \pm 0.17$ & $6.72 \pm 0.39$ & $2.17 \pm 0.10$ & $-2.5 \pm 0.3$ & $-7.7 \pm 0.8$ & CTTS\\
C23215 & $-0.35 \pm 0.40$ & $-0.43 \pm 0.08$ & $6.48 \pm 0.09$ & $-0.20 \pm 1.03$ & $-5.4 \pm 1.0$ &  & \\
C23314 & $-0.50 \pm 0.44$ & $-0.85 \pm 0.14$ & $6.10 \pm 0.29$ & $1.93 \pm 0.17$ & $-4.1 \pm 0.4$ &  & \\
C23474 & $-0.43 \pm 0.37$ & $-0.62 \pm 0.05$ & $6.53 \pm 0.05$ & $0.12 \pm 0.86$ & $-5.6 \pm 0.9$ &  & \\
C23553 & $-0.40 \pm 0.37$ & $-0.84 \pm 0.13$ & $6.64 \pm 0.09$ & $-0.14 \pm 0.65$ & $-6.4 \pm 0.6$ &  & \\
C23686 & $-0.37 \pm 0.39$ & $-0.52 \pm 0.06$ & $6.45 \pm 0.06$ & $-0.20 \pm 0.89$ & $-5.6 \pm 0.9$ &  & \\
C23781 & $-0.38 \pm 0.40$ & $-0.38 \pm 0.09$ & $6.58 \pm 0.13$ & $-0.32 \pm 1.08$ & $-5.5 \pm 1.1$ &  & \\
C23909 & $-0.41 \pm 0.39$ & $-0.42 \pm 0.08$ & $6.62 \pm 0.13$ & $-0.08 \pm 1.02$ & $-5.3 \pm 1.0$ &  & \\
C24113 & $-0.33 \pm 0.38$ & $-0.24 \pm 0.14$ & $6.10 \pm 0.21$ & $-0.95 \pm 1.19$ & $-5.4 \pm 1.2$ &  & \\
C24217 & $-0.31 \pm 0.43$ & $-0.39 \pm 0.12$ & $6.29 \pm 0.19$ & $-0.39 \pm 1.14$ & $-5.3 \pm 1.2$ &  & \\
C24250 & $-0.51 \pm 0.36$ & $-0.09 \pm 0.12$ & $6.42 \pm 0.31$ & $-0.57 \pm 1.08$ & $-4.9 \pm 1.1$ &  & \\
C24349 & $-0.40 \pm 0.43$ & $-0.37 \pm 0.09$ & $6.50 \pm 0.13$ & $1.03 \pm 0.95$ & $-4.0 \pm 1.0$ &  & \\
C24362 & $-0.38 \pm 0.47$ & $-0.63 \pm 0.12$ & $7.24 \pm 0.14$ & $1.70 \pm 0.26$ & $-4.5 \pm 0.4$ & $-10.7 \pm 0.9$ & CTTS\\
C24373 & $-0.33 \pm 0.44$ & $-0.55 \pm 0.09$ & $6.47 \pm 0.07$ & $-0.40 \pm 1.00$ & $-5.9 \pm 1.0$ &  & \\
C24554 & $-0.45 \pm 0.41$ & $-0.26 \pm 0.11$ & $6.53 \pm 0.19$ & $1.51 \pm 0.51$ & $-3.3 \pm 0.5$ & $-8.9 \pm 1.1$ & CTTS\\
C24602 & $-0.65 \pm 0.33$ & $0.08 \pm 0.10$ & $6.39 \pm 0.35$ & $-0.31 \pm 1.00$ & $-4.3 \pm 1.0$ &  & \\
C24893 & $-0.45 \pm 0.38$ & $-0.35 \pm 0.09$ & $6.92 \pm 0.18$ & $-0.23 \pm 1.08$ & $-5.5 \pm 1.1$ &  & \\
C24924 & $-0.44 \pm 0.43$ & $0.10 \pm 0.06$ & $7.04 \pm 0.51$ & $1.45 \pm 0.51$ & $-2.6 \pm 0.5$ & $-8.0 \pm 1.1$ & CTTS\\
C24984 & $-0.41 \pm 0.41$ & $-0.52 \pm 0.09$ & $6.51 \pm 0.08$ & $0.99 \pm 0.83$ & $-4.5 \pm 0.9$ &  & \\
C25214 & $-0.38 \pm 0.35$ & $-0.76 \pm 0.08$ & $6.78 \pm 0.07$ & $-0.11 \pm 0.65$ & $-6.3 \pm 0.7$ &  & \\
C25248 & $-0.38 \pm 0.38$ & $-0.61 \pm 0.07$ & $6.88 \pm 0.08$ & $0.03 \pm 0.81$ & $-5.9 \pm 0.8$ &  & \\
C25302 & $-0.39 \pm 0.41$ & $-0.54 \pm 0.08$ & $6.80 \pm 0.10$ & $1.65 \pm 0.33$ & $-4.0 \pm 0.4$ & $-9.9 \pm 0.9$ & CTTS\\
C25335 & $-0.28 \pm 0.39$ & $-0.34 \pm 0.11$ & $6.39 \pm 0.21$ & $2.44 \pm 0.09$ & $-2.4 \pm 0.2$ & $-7.4 \pm 0.7$ & CTTS\\
C25404 & $-0.41 \pm 0.38$ & $-0.60 \pm 0.06$ & $6.59 \pm 0.06$ & $1.65 \pm 0.28$ & $-4.1 \pm 0.3$ & $-9.8 \pm 0.8$ & CTTS\\
C25550 & $-0.39 \pm 0.41$ & $-0.64 \pm 0.10$ & $6.63 \pm 0.12$ & $0.04 \pm 0.84$ & $-5.8 \pm 0.9$ &  & \\
C25738 & $0.44 \pm 0.42$ & $-0.36 \pm 0.23$ & $6.39 \pm 0.30$ & $1.44 \pm 0.78$ & $-3.5 \pm 1.1$ & $-8.9 \pm 1.6$ & CTTS\\
C25835 & $-0.36 \pm 0.46$ & $-0.70 \pm 0.11$ & $6.77 \pm 0.07$ & $-0.07 \pm 0.87$ & $-6.1 \pm 0.9$ &  & \\
C25875 & $-0.37 \pm 0.39$ & $-0.55 \pm 0.08$ & $6.59 \pm 0.10$ & $-0.19 \pm 0.84$ & $-5.8 \pm 0.9$ &  & \\
C25891 & $-0.37 \pm 0.39$ & $-0.40 \pm 0.09$ & $6.69 \pm 0.12$ & $-0.23 \pm 1.03$ & $-5.5 \pm 1.0$ &  & \\
C25927 & $-0.35 \pm 0.42$ & $-0.47 \pm 0.08$ & $6.53 \pm 0.08$ & $-0.20 \pm 0.98$ & $-5.5 \pm 1.0$ &  & \\
C26021 & $-0.35 \pm 0.39$ & $-0.36 \pm 0.10$ & $6.22 \pm 0.16$ & $-0.29 \pm 1.10$ & $-5.1 \pm 1.1$ &  & \\
C26103 & $-0.22 \pm 0.53$ & $-0.56 \pm 0.14$ & $6.57 \pm 0.09$ & $1.90 \pm 0.14$ & $-3.7 \pm 0.4$ & $-9.3 \pm 0.9$ & CTTS\\
C26120 & $-0.26 \pm 0.43$ & $-0.45 \pm 0.11$ & $7.05 \pm 0.15$ & $2.51 \pm 0.09$ & $-3.1 \pm 0.2$ & $-8.6 \pm 0.7$ & CTTS\\
C26166 & $-0.31 \pm 0.38$ & $-0.54 \pm 0.09$ & $6.64 \pm 0.09$ & $-0.28 \pm 0.80$ & $-5.9 \pm 0.8$ &  & \\
C26216 & $-0.46 \pm 0.42$ & $-0.69 \pm 0.09$ & $6.70 \pm 0.07$ & $1.24 \pm 0.67$ & $-4.8 \pm 0.7$ &  & \\
C26264 & $-0.37 \pm 0.39$ & $-0.37 \pm 0.09$ & $6.25 \pm 0.09$ & $-0.42 \pm 1.15$ & $-5.3 \pm 1.1$ &  & \\
C26400 & $-0.37 \pm 0.41$ & $-0.49 \pm 0.09$ & $6.25 \pm 0.13$ & $-0.28 \pm 0.95$ & $-5.4 \pm 1.0$ &  & \\
C26829 & $-0.33 \pm 0.44$ & $-0.58 \pm 0.15$ & $6.49 \pm 0.20$ & $-0.12 \pm 0.86$ & $-5.7 \pm 0.9$ &  & \\
C26854 & $-0.44 \pm 0.40$ & $-0.54 \pm 0.09$ & $6.53 \pm 0.11$ & $0.21 \pm 0.96$ & $-5.3 \pm 1.0$ &  & \\
C26862 & $-0.36 \pm 0.39$ & $-0.53 \pm 0.06$ & $6.56 \pm 0.06$ & $-0.26 \pm 0.92$ & $-5.8 \pm 0.9$ &  & \\
C26966 & $-0.39 \pm 0.45$ & $-0.34 \pm 0.11$ & $6.06 \pm 0.10$ & $0.82 \pm 1.21$ & $-3.8 \pm 1.2$ &  & \\
C26999 & $-0.53 \pm 0.37$ & $-0.10 \pm 0.11$ & $6.47 \pm 0.32$ & $-0.54 \pm 1.06$ & $-5.0 \pm 1.0$ &  & \\
C27205 & $-0.30 \pm 0.39$ & $-0.36 \pm 0.10$ & $6.16 \pm 0.09$ & $-0.50 \pm 1.07$ & $-5.3 \pm 1.1$ &  & \\
C27213 & $-0.24 \pm 0.51$ & $-0.47 \pm 0.15$ & $6.40 \pm 0.22$ & $1.84 \pm 0.15$ & $-3.4 \pm 0.4$ & $-8.7 \pm 0.9$ & CTTS\\
C27301 & $-0.53 \pm 0.36$ & $-0.16 \pm 0.10$ & $6.62 \pm 0.25$ & $-0.52 \pm 1.02$ & $-5.2 \pm 1.0$ &  & \\
C27379 & $-0.48 \pm 0.38$ & $-0.20 \pm 0.10$ & $6.81 \pm 0.28$ & $-0.37 \pm 0.99$ & $-5.2 \pm 1.0$ &  & \\
C27435 & $-0.38 \pm 0.45$ & $-0.33 \pm 0.14$ & $6.09 \pm 0.23$ & $-0.73 \pm 1.46$ & $-5.3 \pm 1.5$ &  & \\
C27436 & $-0.29 \pm 0.38$ & $-0.37 \pm 0.10$ & $6.20 \pm 0.10$ & $-0.47 \pm 1.03$ & $-5.3 \pm 1.0$ &  & \\
C27558 & $-0.42 \pm 0.38$ & $-0.31 \pm 0.10$ & $6.52 \pm 0.17$ & $-0.37 \pm 1.11$ & $-5.3 \pm 1.1$ &  & \\
C27854 & $-0.38 \pm 0.39$ & $-0.21 \pm 0.13$ & $6.39 \pm 0.28$ & $-0.84 \pm 1.15$ & $-5.4 \pm 1.2$ &  & \\
C27963 & $0.11 \pm 0.66$ & $-0.16 \pm 0.24$ & $5.97 \pm 0.27$ & $0.07 \pm 2.60$ & $-4.1 \pm 2.9$ &  & \\
C28298 & $-0.34 \pm 0.38$ & $-0.62 \pm 0.08$ & $6.95 \pm 0.09$ & $-0.08 \pm 0.75$ & $-6.1 \pm 0.8$ &  & \\
C28305 & $-0.38 \pm 0.36$ & $-0.30 \pm 0.10$ & $6.59 \pm 0.17$ & $-0.55 \pm 1.06$ & $-5.5 \pm 1.1$ &  & \\
C28324 & $-0.40 \pm 0.38$ & $-0.54 \pm 0.06$ & $6.76 \pm 0.08$ & $-0.00 \pm 0.87$ & $-5.7 \pm 0.9$ &  & \\
C28457 & $-0.33 \pm 0.41$ & $-0.45 \pm 0.09$ & $6.27 \pm 0.14$ & $-0.35 \pm 1.00$ & $-5.4 \pm 1.0$ &  & \\
C28505 & $-0.49 \pm 0.38$ & $-0.16 \pm 0.12$ & $6.40 \pm 0.28$ & $-0.65 \pm 1.13$ & $-5.2 \pm 1.1$ &  & \\
C28541 & $0.23 \pm 0.59$ & $-0.11 \pm 0.20$ & $6.25 \pm 0.36$ & $1.79 \pm 2.07$ & $-2.5 \pm 2.2$ & $-7.3 \pm 3.0$ & CTTS\\
C28544 & $-0.53 \pm 0.43$ & $-0.14 \pm 0.16$ & $6.15 \pm 0.22$ & $-1.18 \pm 1.66$ & $-5.4 \pm 1.6$ &  & \\
C28772 & $-0.41 \pm 0.39$ & $-0.23 \pm 0.13$ & $6.30 \pm 0.24$ & $-1.17 \pm 1.20$ & $-5.7 \pm 1.2$ &  & \\
C28790 & $-0.35 \pm 0.39$ & $-0.46 \pm 0.08$ & $6.52 \pm 0.12$ & $-0.25 \pm 0.93$ & $-5.6 \pm 0.9$ &  & \\
C28907 & $-0.47 \pm 0.40$ & $-0.14 \pm 0.13$ & $6.32 \pm 0.27$ & $1.66 \pm 0.33$ & $-2.7 \pm 0.4$ & $-7.9 \pm 0.9$ & CTTS\\
C28949 & $-0.29 \pm 0.38$ & $-0.43 \pm 0.08$ & $6.50 \pm 0.09$ & $-0.37 \pm 0.94$ & $-5.6 \pm 0.9$ &  & \\
C28983 & $-0.56 \pm 0.36$ & $-0.00 \pm 0.07$ & $6.85 \pm 0.36$ & $-0.42 \pm 1.00$ & $-4.9 \pm 1.0$ &  & \\
C28991 & $-0.34 \pm 0.36$ & $-0.45 \pm 0.07$ & $6.75 \pm 0.09$ & $-0.22 \pm 0.87$ & $-5.7 \pm 0.9$ &  & \\
C29037 & $-0.51 \pm 0.39$ & $-0.10 \pm 0.10$ & $6.77 \pm 0.34$ & $-0.35 \pm 1.02$ & $-5.0 \pm 1.0$ &  & \\
C29082 & $-0.51 \pm 0.34$ & $-0.19 \pm 0.09$ & $6.72 \pm 0.23$ & $-0.22 \pm 0.94$ & $-5.0 \pm 0.9$ &  & \\
C29089 & $-0.46 \pm 0.38$ & $-0.41 \pm 0.08$ & $6.76 \pm 0.12$ & $0.21 \pm 1.00$ & $-5.1 \pm 1.0$ &  & \\
C29297 & $-0.39 \pm 0.47$ & $-0.34 \pm 0.12$ & $6.51 \pm 0.20$ & $-0.38 \pm 1.49$ & $-5.4 \pm 1.5$ &  & \\
C29357 & $-0.41 \pm 0.43$ & $-0.62 \pm 0.12$ & $6.52 \pm 0.07$ & $0.09 \pm 0.91$ & $-5.7 \pm 0.9$ &  & \\
C29385 & $-0.35 \pm 0.38$ & $-0.47 \pm 0.07$ & $6.61 \pm 0.08$ & $-0.26 \pm 0.92$ & $-5.6 \pm 0.9$ &  & \\
C29465 & $-0.31 \pm 0.38$ & $-0.50 \pm 0.06$ & $6.68 \pm 0.07$ & $-0.31 \pm 0.87$ & $-5.8 \pm 0.9$ &  & \\
C29467 & $-0.31 \pm 0.39$ & $-0.30 \pm 0.12$ & $6.34 \pm 0.23$ & $-0.80 \pm 1.17$ & $-5.6 \pm 1.2$ &  & \\
C29493 & $0.60 \pm 0.29$ & $-0.30 \pm 0.20$ & $6.24 \pm 0.21$ & $-1.16 \pm 1.17$ & $-5.8 \pm 1.3$ &  & \\
C29547 & $0.52 \pm 0.31$ & $-0.21 \pm 0.22$ & $5.93 \pm 0.21$ & $-1.73 \pm 1.26$ & $-6.0 \pm 1.4$ &  & \\
C29591 & $-0.37 \pm 0.41$ & $-0.50 \pm 0.08$ & $6.26 \pm 0.06$ & $-0.31 \pm 0.95$ & $-5.5 \pm 0.9$ &  & \\
C29702 & $-0.34 \pm 0.42$ & $-0.44 \pm 0.07$ & $6.40 \pm 0.08$ & $1.79 \pm 0.16$ & $-3.4 \pm 0.2$ & $-8.8 \pm 0.8$ & CTTS\\
C29785 & $-0.43 \pm 0.37$ & $-0.35 \pm 0.08$ & $6.64 \pm 0.13$ & $-0.14 \pm 1.12$ & $-5.3 \pm 1.1$ &  & \\
C29815 & $-0.37 \pm 0.36$ & $-0.36 \pm 0.09$ & $6.69 \pm 0.14$ & $-0.29 \pm 1.01$ & $-5.5 \pm 1.0$ &  & \\
C29851 & $-0.37 \pm 0.38$ & $-0.20 \pm 0.13$ & $6.31 \pm 0.26$ & $-1.01 \pm 1.15$ & $-5.5 \pm 1.1$ &  & \\
C29865 & $-0.36 \pm 0.38$ & $-0.34 \pm 0.10$ & $6.58 \pm 0.17$ & $-0.42 \pm 1.09$ & $-5.5 \pm 1.1$ &  & \\
C29916 & $-0.28 \pm 0.43$ & $-0.39 \pm 0.11$ & $6.49 \pm 0.15$ & $-0.66 \pm 1.14$ & $-5.8 \pm 1.2$ &  & \\
C30006 & $0.26 \pm 0.29$ & $-0.17 \pm 0.18$ & $6.26 \pm 0.31$ & $-1.87 \pm 1.10$ & $-6.3 \pm 1.2$ &  & \\
C30045 & $-0.26 \pm 0.57$ & $-0.59 \pm 0.16$ & $6.80 \pm 0.11$ & $1.13 \pm 0.88$ & $-4.7 \pm 1.0$ &  & \\
C30125 & $-0.31 \pm 0.47$ & $-0.56 \pm 0.21$ & $5.77 \pm 0.37$ & $-0.33 \pm 0.91$ & $-5.5 \pm 1.0$ &  & \\
C30190 & $-0.35 \pm 0.36$ & $-0.36 \pm 0.08$ & $6.42 \pm 0.11$ & $-0.41 \pm 1.06$ & $-5.4 \pm 1.1$ &  & \\
C30230 & $-0.45 \pm 0.44$ & $-0.68 \pm 0.11$ & $6.42 \pm 0.08$ & $1.73 \pm 0.23$ & $-4.0 \pm 0.3$ & $-9.6 \pm 0.8$ & CTTS\\
C30330 & $-0.37 \pm 0.39$ & $-0.41 \pm 0.10$ & $6.80 \pm 0.14$ & $-0.09 \pm 0.96$ & $-5.4 \pm 1.0$ &  & \\
C30381 & $-0.42 \pm 0.45$ & $-0.69 \pm 0.14$ & $6.61 \pm 0.14$ & $1.45 \pm 0.53$ & $-4.5 \pm 0.6$ &  & \\
C30388 & $-0.33 \pm 0.40$ & $-0.43 \pm 0.09$ & $7.13 \pm 0.15$ & $2.40 \pm 0.09$ & $-3.2 \pm 0.2$ & $-8.8 \pm 0.7$ & CTTS\\
C30443 & $-0.37 \pm 0.38$ & $-0.43 \pm 0.08$ & $6.26 \pm 0.07$ & $-0.21 \pm 0.99$ & $-5.2 \pm 1.0$ &  & \\
C30451 & $-0.45 \pm 0.41$ & $-0.61 \pm 0.08$ & $7.10 \pm 0.11$ & $0.69 \pm 0.86$ & $-5.3 \pm 0.9$ &  & \\
C30470 & $-0.50 \pm 0.36$ & $-0.24 \pm 0.10$ & $6.56 \pm 0.21$ & $-0.59 \pm 1.10$ & $-5.4 \pm 1.1$ &  & \\
C30471 & $-0.15 \pm 0.48$ & $-0.44 \pm 0.13$ & $6.72 \pm 0.12$ & $2.39 \pm 0.09$ & $-3.0 \pm 0.3$ & $-8.3 \pm 0.8$ & CTTS\\
C30512 & $-0.38 \pm 0.43$ & $-0.22 \pm 0.14$ & $6.14 \pm 0.26$ & $1.37 \pm 0.75$ & $-3.0 \pm 0.8$ & $-8.3 \pm 1.4$ & CTTS\\
C30555 & $-0.36 \pm 0.38$ & $-0.37 \pm 0.09$ & $6.80 \pm 0.16$ & $-0.31 \pm 1.03$ & $-5.6 \pm 1.0$ &  & \\
C30573 & $-0.28 \pm 0.37$ & $-0.35 \pm 0.10$ & $6.64 \pm 0.17$ & $-0.47 \pm 1.00$ & $-5.6 \pm 1.0$ &  & \\
C30656 & $-0.36 \pm 0.41$ & $-0.67 \pm 0.11$ & $6.69 \pm 0.09$ & $-0.09 \pm 0.74$ & $-6.0 \pm 0.8$ &  & \\
C30761 & $-0.37 \pm 0.39$ & $-0.38 \pm 0.09$ & $6.65 \pm 0.14$ & $-0.20 \pm 1.03$ & $-5.4 \pm 1.1$ &  & \\
C30824 & $-0.57 \pm 0.36$ & $-0.09 \pm 0.09$ & $6.76 \pm 0.30$ & $-0.36 \pm 0.99$ & $-5.0 \pm 1.0$ &  & \\
C30854 & $-0.33 \pm 0.40$ & $-0.65 \pm 0.10$ & $6.87 \pm 0.09$ & $-0.17 \pm 0.73$ & $-6.2 \pm 0.7$ &  & \\
C30856 & $-0.31 \pm 0.39$ & $-0.42 \pm 0.09$ & $6.34 \pm 0.11$ & $-0.34 \pm 0.99$ & $-5.4 \pm 1.0$ &  & \\
C30880 & $-0.33 \pm 0.38$ & $-0.30 \pm 0.11$ & $6.07 \pm 0.12$ & $-0.68 \pm 1.16$ & $-5.2 \pm 1.2$ &  & \\
C30909 & $-0.19 \pm 0.47$ & $-0.31 \pm 0.14$ & $6.27 \pm 0.15$ & $1.74 \pm 0.57$ & $-3.0 \pm 0.6$ & $-8.2 \pm 1.1$ & CTTS\\
C30967 & $-0.38 \pm 0.39$ & $-0.50 \pm 0.08$ & $6.77 \pm 0.11$ & $-0.03 \pm 0.90$ & $-5.6 \pm 0.9$ &  & \\
C30991 & $-0.45 \pm 0.34$ & $-0.25 \pm 0.09$ & $6.51 \pm 0.17$ & $-0.67 \pm 1.05$ & $-5.5 \pm 1.0$ &  & \\
C31021 & $-0.51 \pm 0.35$ & $-0.15 \pm 0.10$ & $6.49 \pm 0.26$ & $-0.48 \pm 0.99$ & $-5.0 \pm 1.0$ &  & \\
C31040 & $-0.45 \pm 0.36$ & $-0.27 \pm 0.10$ & $6.29 \pm 0.15$ & $-0.60 \pm 1.13$ & $-5.3 \pm 1.1$ &  & \\
C31147 & $-0.36 \pm 0.47$ & $-0.34 \pm 0.12$ & $6.30 \pm 0.12$ & $0.11 \pm 1.49$ & $-4.7 \pm 1.5$ &  & \\
C31149 & $-0.33 \pm 0.41$ & $-0.38 \pm 0.10$ & $6.91 \pm 0.15$ & $1.78 \pm 0.16$ & $-3.6 \pm 0.2$ & $-9.4 \pm 0.8$ & CTTS\\
C31178 & $-0.24 \pm 0.34$ & $-0.32 \pm 0.09$ & $7.27 \pm 0.22$ & $-0.50 \pm 0.86$ & $-5.9 \pm 0.9$ &  & \\
C31190 & $0.19 \pm 0.43$ & $-0.35 \pm 0.15$ & $7.48 \pm 0.24$ & $2.31 \pm 0.10$ & $-3.3 \pm 0.3$ & $-9.1 \pm 0.8$ & CTTS\\
C31293 & $-0.35 \pm 0.39$ & $-0.46 \pm 0.08$ & $6.49 \pm 0.12$ & $-0.26 \pm 0.92$ & $-5.5 \pm 0.9$ &  & \\
C31309 & $-0.32 \pm 0.41$ & $-0.45 \pm 0.09$ & $6.45 \pm 0.09$ & $-0.39 \pm 0.99$ & $-5.6 \pm 1.0$ &  & \\
C31352 & $-0.39 \pm 0.51$ & $-0.11 \pm 0.19$ & $6.18 \pm 0.38$ & $0.76 \pm 1.60$ & $-3.4 \pm 1.6$ &  & \\
C31375 & $-0.41 \pm 0.38$ & $-0.53 \pm 0.07$ & $6.71 \pm 0.09$ & $2.23 \pm 0.10$ & $-3.4 \pm 0.2$ & $-8.9 \pm 0.7$ & CTTS\\
C31411 & $-0.31 \pm 0.43$ & $-0.46 \pm 0.11$ & $6.21 \pm 0.14$ & $-0.46 \pm 1.05$ & $-5.5 \pm 1.1$ &  & \\
C31415 & $-0.33 \pm 0.44$ & $-0.61 \pm 0.08$ & $6.42 \pm 0.06$ & $-0.46 \pm 1.01$ & $-6.1 \pm 1.0$ &  & \\
C31430 & $-0.32 \pm 0.39$ & $-0.39 \pm 0.09$ & $6.33 \pm 0.09$ & $-0.36 \pm 1.04$ & $-5.3 \pm 1.0$ &  & \\
C31514 & $-0.39 \pm 0.40$ & $-0.68 \pm 0.10$ & $6.78 \pm 0.10$ & $-0.08 \pm 0.77$ & $-6.1 \pm 0.8$ &  & \\
C31556 & $-0.44 \pm 0.41$ & $-0.63 \pm 0.08$ & $7.02 \pm 0.11$ & $0.98 \pm 0.81$ & $-5.1 \pm 0.8$ &  & \\
C31566 & $-0.37 \pm 0.40$ & $-0.45 \pm 0.09$ & $6.78 \pm 0.13$ & $-0.20 \pm 0.96$ & $-5.6 \pm 1.0$ &  & \\
C31611 & $-0.36 \pm 0.44$ & $-0.62 \pm 0.14$ & $6.36 \pm 0.15$ & $-0.21 \pm 0.85$ & $-5.8 \pm 0.9$ &  & \\
C31662 & $-0.41 \pm 0.41$ & $-0.55 \pm 0.08$ & $6.46 \pm 0.06$ & $0.02 \pm 1.00$ & $-5.5 \pm 1.0$ &  & \\
C31669 & $-0.39 \pm 0.44$ & $-0.66 \pm 0.11$ & $6.73 \pm 0.08$ & $1.87 \pm 0.15$ & $-4.1 \pm 0.3$ & $-9.9 \pm 0.8$ & CTTS\\
C31681 & $-0.40 \pm 0.41$ & $-0.64 \pm 0.10$ & $6.69 \pm 0.11$ & $0.05 \pm 0.83$ & $-5.8 \pm 0.9$ &  & \\
C31682 & $-0.50 \pm 0.38$ & $-0.13 \pm 0.13$ & $6.33 \pm 0.29$ & $-0.61 \pm 1.10$ & $-5.0 \pm 1.1$ &  & \\
C31767 & $-0.45 \pm 0.40$ & $-0.54 \pm 0.05$ & $6.53 \pm 0.06$ & $1.00 \pm 0.86$ & $-4.5 \pm 0.9$ &  & \\
C31826 & $-0.47 \pm 0.38$ & $-0.74 \pm 0.09$ & $6.71 \pm 0.07$ & $0.10 \pm 0.77$ & $-6.0 \pm 0.8$ &  & \\
C31849 & $-0.35 \pm 0.40$ & $-0.45 \pm 0.08$ & $6.31 \pm 0.09$ & $-0.34 \pm 1.02$ & $-5.5 \pm 1.0$ &  & \\
C31874 & $-0.41 \pm 0.43$ & $-0.64 \pm 0.13$ & $6.52 \pm 0.10$ & $0.06 \pm 0.89$ & $-5.7 \pm 1.0$ &  & \\
C31888 & $-0.39 \pm 0.34$ & $-0.34 \pm 0.08$ & $7.08 \pm 0.18$ & $-0.19 \pm 0.87$ & $-5.6 \pm 0.9$ &  & \\
C31889 & $-0.46 \pm 0.34$ & $-0.25 \pm 0.09$ & $6.52 \pm 0.18$ & $-0.55 \pm 1.01$ & $-5.4 \pm 1.0$ &  & \\
C32005 & $-0.71 \pm 0.31$ & $-0.09 \pm 0.02$ & $7.79 \pm 0.18$ & $-0.24 \pm 0.83$ & $-5.1 \pm 0.8$ &  & \\
C32054 & $-0.43 \pm 0.36$ & $-0.22 \pm 0.11$ & $6.25 \pm 0.17$ & $-0.74 \pm 1.12$ & $-5.3 \pm 1.1$ &  & \\
C32060 & $-0.19 \pm 0.58$ & $-0.56 \pm 0.15$ & $6.35 \pm 0.11$ & $0.88 \pm 1.25$ & $-4.5 \pm 1.4$ &  & \\
C32086 & $-0.41 \pm 0.36$ & $-0.34 \pm 0.09$ & $6.60 \pm 0.14$ & $-0.35 \pm 1.06$ & $-5.4 \pm 1.1$ &  & \\
C32087 & $-0.38 \pm 0.37$ & $-0.31 \pm 0.09$ & $6.43 \pm 0.16$ & $-0.57 \pm 1.09$ & $-5.4 \pm 1.1$ &  & \\
C32167 & $-0.34 \pm 0.38$ & $-0.36 \pm 0.10$ & $6.58 \pm 0.17$ & $-0.37 \pm 1.06$ & $-5.4 \pm 1.1$ &  & \\
C32171 & $-0.28 \pm 0.44$ & $-0.27 \pm 0.17$ & $6.06 \pm 0.31$ & $-0.97 \pm 1.28$ & $-5.3 \pm 1.3$ &  & \\
C32207 & $-0.32 \pm 0.39$ & $-0.31 \pm 0.12$ & $6.18 \pm 0.16$ & $-0.60 \pm 1.18$ & $-5.2 \pm 1.2$ &  & \\
C32219 & $-0.32 \pm 0.46$ & $-0.42 \pm 0.11$ & $6.97 \pm 0.15$ & $1.56 \pm 0.38$ & $-3.9 \pm 0.5$ & $-9.9 \pm 0.9$ & CTTS\\
C32226 & $-0.37 \pm 0.38$ & $-0.46 \pm 0.06$ & $6.51 \pm 0.08$ & $-0.30 \pm 0.96$ & $-5.6 \pm 1.0$ &  & \\
C32265 & $-0.54 \pm 0.38$ & $-0.17 \pm 0.14$ & $6.19 \pm 0.25$ & $-0.68 \pm 1.31$ & $-5.0 \pm 1.3$ &  & \\
C32270 & $-0.35 \pm 0.41$ & $-0.57 \pm 0.09$ & $6.37 \pm 0.07$ & $2.04 \pm 0.12$ & $-3.4 \pm 0.2$ & $-8.7 \pm 0.8$ & CTTS\\
C32295 & $-0.26 \pm 0.42$ & $-0.28 \pm 0.14$ & $6.31 \pm 0.24$ & $-1.39 \pm 1.23$ & $-6.1 \pm 1.3$ &  & \\
C32341 & $-0.38 \pm 0.39$ & $-0.45 \pm 0.08$ & $6.60 \pm 0.13$ & $-0.19 \pm 0.96$ & $-5.5 \pm 1.0$ &  & \\
C32413 & $-0.36 \pm 0.40$ & $-0.52 \pm 0.09$ & $6.56 \pm 0.08$ & $2.04 \pm 0.12$ & $-3.5 \pm 0.2$ & $-8.9 \pm 0.7$ & CTTS\\
C32434 & $-0.40 \pm 0.42$ & $-0.57 \pm 0.08$ & $6.53 \pm 0.07$ & $1.34 \pm 0.61$ & $-4.3 \pm 0.6$ &  & \\
C32443 & $-0.58 \pm 0.39$ & $0.05 \pm 0.10$ & $6.44 \pm 0.37$ & $1.16 \pm 0.96$ & $-2.9 \pm 1.0$ & $-8.4 \pm 1.6$ & CTTS\\
C32453 & $-0.47 \pm 0.37$ & $-0.23 \pm 0.10$ & $6.62 \pm 0.23$ & $-0.59 \pm 1.11$ & $-5.4 \pm 1.1$ &  & \\
C32515 & $-0.33 \pm 0.43$ & $-0.47 \pm 0.11$ & $6.47 \pm 0.15$ & $-0.23 \pm 0.98$ & $-5.5 \pm 1.0$ &  & \\
C32540 & $-0.36 \pm 0.38$ & $-0.34 \pm 0.09$ & $6.42 \pm 0.13$ & $-0.71 \pm 1.15$ & $-5.6 \pm 1.1$ &  & \\
C32541 & $-0.10 \pm 0.43$ & $-0.43 \pm 0.13$ & $7.07 \pm 0.17$ & $2.52 \pm 0.09$ & $-3.0 \pm 0.3$ & $-8.5 \pm 0.8$ & CTTS\\
C32545 & $-0.28 \pm 0.39$ & $-0.33 \pm 0.10$ & $6.60 \pm 0.16$ & $2.59 \pm 0.08$ & $-2.4 \pm 0.2$ & $-7.5 \pm 0.7$ & CTTS\\
C32567 & $-0.49 \pm 0.36$ & $-0.21 \pm 0.10$ & $6.60 \pm 0.24$ & $-0.52 \pm 1.07$ & $-5.3 \pm 1.0$ &  & \\
C32568 & $-0.47 \pm 0.41$ & $-0.76 \pm 0.12$ & $6.73 \pm 0.12$ & $1.07 \pm 0.81$ & $-5.1 \pm 0.8$ &  & \\
C32585 & $-0.25 \pm 0.41$ & $-0.28 \pm 0.14$ & $6.20 \pm 0.27$ & $2.10 \pm 0.10$ & $-2.5 \pm 0.2$ & $-7.4 \pm 0.7$ & CTTS\\
C32812 & $-0.43 \pm 0.37$ & $-0.58 \pm 0.05$ & $6.87 \pm 0.08$ & $0.14 \pm 0.86$ & $-5.7 \pm 0.9$ &  & \\
C32824 & $-0.51 \pm 0.35$ & $-0.16 \pm 0.11$ & $6.36 \pm 0.21$ & $-0.61 \pm 1.10$ & $-5.1 \pm 1.1$ &  & \\
C32846 & $-0.41 \pm 0.39$ & $-0.62 \pm 0.06$ & $6.72 \pm 0.07$ & $0.02 \pm 0.87$ & $-5.8 \pm 0.9$ &  & \\
C32868 & $-0.33 \pm 0.43$ & $-0.55 \pm 0.14$ & $6.41 \pm 0.21$ & $-0.23 \pm 0.89$ & $-5.7 \pm 0.9$ &  & \\
C32879 & $-0.44 \pm 0.37$ & $-0.17 \pm 0.13$ & $6.17 \pm 0.28$ & $-0.76 \pm 1.11$ & $-5.1 \pm 1.1$ &  & \\
C32892 & $-0.51 \pm 0.45$ & $-0.11 \pm 0.20$ & $5.75 \pm 0.50$ & $-0.21 \pm 0.99$ & $-4.0 \pm 1.0$ &  & \\
C32919 & $-0.36 \pm 0.35$ & $-0.47 \pm 0.05$ & $6.38 \pm 0.06$ & $-0.15 \pm 0.85$ & $-5.4 \pm 0.9$ &  & \\
C32922 & $-0.48 \pm 0.42$ & $-0.73 \pm 0.12$ & $6.59 \pm 0.10$ & $0.49 \pm 0.87$ & $-5.5 \pm 0.9$ &  & \\
C32959 & $-0.41 \pm 0.38$ & $-0.56 \pm 0.07$ & $6.61 \pm 0.07$ & $0.05 \pm 0.93$ & $-5.6 \pm 0.9$ &  & \\
C32960 & $-0.36 \pm 0.42$ & $-0.48 \pm 0.10$ & $6.32 \pm 0.08$ & $-0.21 \pm 0.98$ & $-5.4 \pm 1.0$ &  & \\
C32974 & $-0.26 \pm 0.41$ & $-0.35 \pm 0.11$ & $6.43 \pm 0.13$ & $-0.70 \pm 1.16$ & $-5.7 \pm 1.2$ &  & \\
C32993 & $-0.41 \pm 0.45$ & $-0.60 \pm 0.13$ & $6.48 \pm 0.16$ & $0.38 \pm 0.98$ & $-5.3 \pm 1.0$ &  & \\
C32994 & $-0.34 \pm 0.38$ & $-0.35 \pm 0.10$ & $6.41 \pm 0.14$ & $-0.50 \pm 1.10$ & $-5.4 \pm 1.1$ &  & \\
C33060 & $-0.41 \pm 0.45$ & $-0.71 \pm 0.11$ & $6.70 \pm 0.07$ & $0.16 \pm 0.92$ & $-5.9 \pm 0.9$ &  & \\
C33066 & $-0.44 \pm 0.44$ & $-0.35 \pm 0.12$ & $5.42 \pm 0.25$ & $-3.35 \pm 1.05$ & $-7.5 \pm 1.1$ &  & \\
C33082 & $-0.36 \pm 0.46$ & $-0.30 \pm 0.12$ & $6.20 \pm 0.13$ & $-1.85 \pm 1.37$ & $-6.5 \pm 1.4$ &  & \\
C33085 & $-0.43 \pm 0.36$ & $-0.51 \pm 0.07$ & $7.27 \pm 0.12$ & $0.19 \pm 0.84$ & $-5.7 \pm 0.9$ &  & \\
C33098 & $-0.58 \pm 0.34$ & $-0.24 \pm 0.07$ & $7.12 \pm 0.22$ & $-0.10 \pm 0.93$ & $-5.3 \pm 0.9$ &  & \\
C33122 & $0.26 \pm 0.36$ & $-0.16 \pm 0.20$ & $6.04 \pm 0.21$ & $2.01 \pm 0.12$ & $-2.2 \pm 0.3$ & $-7.0 \pm 0.8$ & CTTS\\
C33153 & $-0.43 \pm 0.39$ & $-0.56 \pm 0.07$ & $6.19 \pm 0.06$ & $-0.23 \pm 0.92$ & $-5.5 \pm 0.9$ &  & \\
C33245 & $-0.35 \pm 0.36$ & $-0.37 \pm 0.08$ & $6.46 \pm 0.11$ & $-0.27 \pm 1.01$ & $-5.3 \pm 1.0$ &  & \\
C33309 & $-0.37 \pm 0.40$ & $-0.53 \pm 0.07$ & $6.62 \pm 0.07$ & $-0.20 \pm 0.89$ & $-5.8 \pm 0.9$ &  & \\
C33395 & $-0.44 \pm 0.40$ & $-0.55 \pm 0.07$ & $7.01 \pm 0.09$ & $0.37 \pm 0.91$ & $-5.4 \pm 0.9$ &  & \\
C33396 & $-0.37 \pm 0.35$ & $-0.30 \pm 0.10$ & $6.63 \pm 0.18$ & $-0.38 \pm 0.98$ & $-5.4 \pm 1.0$ &  & \\
C33404 & $-0.32 \pm 0.39$ & $-0.55 \pm 0.08$ & $6.64 \pm 0.07$ & $-0.30 \pm 0.82$ & $-5.9 \pm 0.8$ &  & \\
C33406 & $-0.32 \pm 0.41$ & $-0.45 \pm 0.11$ & $6.25 \pm 0.10$ & $-0.30 \pm 0.94$ & $-5.4 \pm 0.9$ &  & \\
C33435 & $-0.26 \pm 0.54$ & $-0.54 \pm 0.17$ & $6.38 \pm 0.24$ & $1.16 \pm 0.93$ & $-4.2 \pm 1.1$ &  & \\
C33457 & $-0.30 \pm 0.36$ & $-0.54 \pm 0.07$ & $6.49 \pm 0.06$ & $-0.30 \pm 0.79$ & $-5.8 \pm 0.8$ &  & \\
C33507 & $-0.46 \pm 0.43$ & $-0.28 \pm 0.12$ & $6.09 \pm 0.14$ & $0.37 \pm 1.45$ & $-4.1 \pm 1.5$ &  & \\
C33540 & $-0.38 \pm 0.42$ & $-0.60 \pm 0.10$ & $6.73 \pm 0.13$ & $0.03 \pm 0.87$ & $-5.8 \pm 0.9$ &  & \\
C33568 & $-0.36 \pm 0.55$ & $-0.52 \pm 0.24$ & $5.99 \pm 0.41$ & $1.21 \pm 0.77$ & $-3.9 \pm 1.0$ &  & \\
C33578 & $-0.50 \pm 0.37$ & $-0.69 \pm 0.07$ & $6.62 \pm 0.06$ & $0.22 \pm 0.82$ & $-5.8 \pm 0.8$ &  & \\
C33599 & $-0.31 \pm 0.41$ & $-0.37 \pm 0.11$ & $6.23 \pm 0.21$ & $-0.48 \pm 1.10$ & $-5.3 \pm 1.1$ &  & \\
C33600 & $-0.32 \pm 0.42$ & $-0.56 \pm 0.09$ & $7.50 \pm 0.18$ & $2.74 \pm 0.09$ & $-3.4 \pm 0.2$ & $-9.2 \pm 0.7$ & CTTS\\
C33624 & $-0.12 \pm 0.28$ & $-0.93 \pm 0.10$ & $6.07 \pm 0.26$ & $0.93 \pm 0.89$ & $-5.3 \pm 0.9$ &  & \\
C33640 & $-0.39 \pm 0.43$ & $-0.50 \pm 0.08$ & $6.21 \pm 0.09$ & $-0.29 \pm 1.03$ & $-5.4 \pm 1.0$ &  & \\
C33648 & $-0.10 \pm 0.38$ & $-0.83 \pm 0.16$ & $5.63 \pm 0.30$ & $-0.67 \pm 1.01$ & $-6.6 \pm 1.1$ &  & \\
C33700 & $-0.52 \pm 0.34$ & $-0.18 \pm 0.10$ & $6.40 \pm 0.19$ & $-0.37 \pm 0.98$ & $-4.9 \pm 1.0$ &  & \\
C33709 & $-0.35 \pm 0.47$ & $-0.49 \pm 0.13$ & $5.30 \pm 0.25$ & $-0.85 \pm 1.48$ & $-5.5 \pm 1.5$ &  & \\
C33749 & $-0.42 \pm 0.44$ & $-0.31 \pm 0.12$ & $6.42 \pm 0.25$ & $0.17 \pm 1.36$ & $-4.7 \pm 1.4$ &  & \\
C33801 & $-0.34 \pm 0.36$ & $-0.33 \pm 0.10$ & $6.38 \pm 0.15$ & $-0.47 \pm 1.07$ & $-5.3 \pm 1.1$ &  & \\
C33806 & $-0.28 \pm 0.40$ & $-0.33 \pm 0.11$ & $6.48 \pm 0.14$ & $2.08 \pm 0.11$ & $-2.9 \pm 0.2$ & $-8.1 \pm 0.7$ & CTTS\\
C33866 & $-0.46 \pm 0.42$ & $-0.26 \pm 0.14$ & $6.09 \pm 0.24$ & $0.05 \pm 1.35$ & $-4.4 \pm 1.4$ &  & \\
C33877 & $-0.40 \pm 0.52$ & $-0.32 \pm 0.18$ & $6.09 \pm 0.11$ & $-3.50 \pm 1.72$ & $-8.1 \pm 1.9$ &  & \\
C33882 & $-0.59 \pm 0.35$ & $-0.19 \pm 0.06$ & $7.32 \pm 0.26$ & $-0.17 \pm 0.93$ & $-5.3 \pm 0.9$ &  & \\
C33922 & $0.11 \pm 0.54$ & $-0.34 \pm 0.19$ & $6.25 \pm 0.21$ & $1.76 \pm 0.37$ & $-3.0 \pm 0.6$ & $-8.2 \pm 1.1$ & CTTS\\
C33944 & $-0.18 \pm 0.53$ & $-0.58 \pm 0.15$ & $6.70 \pm 0.09$ & $2.17 \pm 0.11$ & $-3.6 \pm 0.4$ & $-9.1 \pm 0.8$ & CTTS\\
C33966 & $-0.10 \pm 0.50$ & $-0.38 \pm 0.15$ & $6.76 \pm 0.20$ & $2.22 \pm 0.10$ & $-3.0 \pm 0.3$ & $-8.4 \pm 0.8$ & CTTS\\
C33976 & $-0.37 \pm 0.37$ & $-0.30 \pm 0.10$ & $6.30 \pm 0.16$ & $-0.54 \pm 1.12$ & $-5.3 \pm 1.1$ &  & \\
C33988 & $-0.32 \pm 0.39$ & $-0.42 \pm 0.09$ & $6.66 \pm 0.16$ & $-0.37 \pm 0.95$ & $-5.7 \pm 1.0$ &  & \\
C34090 & $-0.14 \pm 0.48$ & $-0.42 \pm 0.13$ & $6.70 \pm 0.14$ & $2.43 \pm 0.09$ & $-2.9 \pm 0.3$ & $-8.2 \pm 0.8$ & CTTS\\
C34127 & $-0.37 \pm 0.38$ & $-0.56 \pm 0.07$ & $6.68 \pm 0.08$ & $-0.09 \pm 0.85$ & $-5.8 \pm 0.8$ &  & \\
C34182 & $-0.31 \pm 0.41$ & $-0.49 \pm 0.09$ & $6.59 \pm 0.09$ & $-0.31 \pm 0.92$ & $-5.7 \pm 0.9$ &  & \\
C34222 & $-0.44 \pm 0.40$ & $-0.29 \pm 0.11$ & $6.64 \pm 0.19$ & $-1.06 \pm 1.23$ & $-6.0 \pm 1.2$ &  & \\
C34223 & $-0.35 \pm 0.45$ & $-0.62 \pm 0.12$ & $6.58 \pm 0.07$ & $1.79 \pm 0.17$ & $-4.0 \pm 0.3$ & $-9.7 \pm 0.8$ & CTTS\\
C34280 & $-0.31 \pm 0.41$ & $-0.56 \pm 0.12$ & $6.76 \pm 0.15$ & $-0.19 \pm 0.82$ & $-5.9 \pm 0.9$ &  & \\
C34324 & $-0.34 \pm 0.36$ & $-0.26 \pm 0.10$ & $7.08 \pm 0.25$ & $-0.70 \pm 0.95$ & $-5.9 \pm 1.0$ &  & \\
C34426 & $-0.37 \pm 0.37$ & $-0.34 \pm 0.08$ & $6.92 \pm 0.16$ & $2.32 \pm 0.09$ & $-3.0 \pm 0.1$ & $-8.4 \pm 0.7$ & CTTS\\
C34452 & $-0.45 \pm 0.42$ & $-0.71 \pm 0.10$ & $6.73 \pm 0.08$ & $0.50 \pm 0.87$ & $-5.6 \pm 0.9$ &  & \\
C34464 & $-0.30 \pm 0.40$ & $-0.43 \pm 0.08$ & $6.11 \pm 0.06$ & $-0.47 \pm 1.03$ & $-5.3 \pm 1.0$ &  & \\
C34532 & $-0.39 \pm 0.45$ & $-0.49 \pm 0.09$ & $6.49 \pm 0.08$ & $-0.15 \pm 1.14$ & $-5.5 \pm 1.2$ &  & \\
C34638 & $-0.41 \pm 0.36$ & $-0.33 \pm 0.09$ & $6.62 \pm 0.17$ & $-0.40 \pm 1.07$ & $-5.4 \pm 1.1$ &  & \\
C34671 & $-0.55 \pm 0.35$ & $-0.05 \pm 0.11$ & $6.47 \pm 0.31$ & $-0.56 \pm 1.06$ & $-4.9 \pm 1.0$ &  & \\
C34675 & $-0.47 \pm 0.47$ & $-0.70 \pm 0.13$ & $6.35 \pm 0.14$ & $1.67 \pm 0.37$ & $-4.1 \pm 0.4$ &  & \\
C34678 & $-0.37 \pm 0.42$ & $-0.56 \pm 0.09$ & $6.39 \pm 0.06$ & $-0.22 \pm 0.94$ & $-5.7 \pm 0.9$ &  & \\
C34713 & $-0.43 \pm 0.41$ & $-0.76 \pm 0.11$ & $6.91 \pm 0.11$ & $0.18 \pm 0.77$ & $-6.1 \pm 0.8$ &  & \\
C34722 & $-0.31 \pm 0.40$ & $-0.40 \pm 0.10$ & $6.56 \pm 0.14$ & $-0.37 \pm 1.02$ & $-5.5 \pm 1.0$ &  & \\
C34726 & $-0.36 \pm 0.39$ & $-0.56 \pm 0.08$ & $6.53 \pm 0.07$ & $-0.19 \pm 0.86$ & $-5.8 \pm 0.9$ &  & \\
C34733 & $-0.56 \pm 0.34$ & $-0.27 \pm 0.08$ & $6.61 \pm 0.17$ & $0.37 \pm 0.97$ & $-4.5 \pm 1.0$ &  & \\
C34739 & $-0.36 \pm 0.40$ & $-0.45 \pm 0.08$ & $6.28 \pm 0.08$ & $-0.34 \pm 1.04$ & $-5.4 \pm 1.0$ &  & \\
C34786 & $-0.36 \pm 0.40$ & $-0.47 \pm 0.09$ & $6.48 \pm 0.09$ & $-0.28 \pm 0.97$ & $-5.6 \pm 1.0$ &  & \\
C34803 & $-0.41 \pm 0.38$ & $-0.33 \pm 0.09$ & $6.65 \pm 0.16$ & $-0.51 \pm 1.14$ & $-5.6 \pm 1.1$ &  & \\
C34859 & $-0.59 \pm 0.42$ & $-0.83 \pm 0.14$ & $6.20 \pm 0.23$ & $0.03 \pm 0.84$ & $-6.0 \pm 0.8$ &  & \\
C34909 & $-0.36 \pm 0.47$ & $-0.49 \pm 0.14$ & $5.70 \pm 0.25$ & $0.12 \pm 1.15$ & $-4.7 \pm 1.2$ &  & \\
C34945 & $-0.52 \pm 0.38$ & $-0.13 \pm 0.11$ & $6.60 \pm 0.33$ & $-0.54 \pm 1.06$ & $-5.1 \pm 1.0$ &  & \\
C34989 & $0.20 \pm 0.16$ & $-0.89 \pm 0.15$ & $6.35 \pm 0.23$ & $2.10 \pm 0.14$ & $-4.1 \pm 0.3$ & $-9.5 \pm 0.8$ & CTTS\\
C35020 & $-0.39 \pm 0.41$ & $-0.54 \pm 0.10$ & $6.53 \pm 0.13$ & $0.03 \pm 0.93$ & $-5.5 \pm 1.0$ &  & \\
C35042 & $-0.29 \pm 0.38$ & $-0.33 \pm 0.11$ & $6.08 \pm 0.10$ & $-0.89 \pm 1.18$ & $-5.5 \pm 1.2$ &  & \\
C35072 & $-0.37 \pm 0.39$ & $-0.59 \pm 0.08$ & $6.55 \pm 0.07$ & $-0.12 \pm 0.86$ & $-5.8 \pm 0.8$ &  & \\
C35074 & $-0.37 \pm 0.37$ & $-0.69 \pm 0.10$ & $6.86 \pm 0.10$ & $-0.14 \pm 0.67$ & $-6.2 \pm 0.7$ &  & \\
C35091 & $-0.38 \pm 0.41$ & $-0.48 \pm 0.09$ & $6.45 \pm 0.14$ & $-0.07 \pm 0.98$ & $-5.4 \pm 1.0$ &  & \\
C35101 & $-0.35 \pm 0.39$ & $-0.43 \pm 0.07$ & $6.58 \pm 0.10$ & $-0.28 \pm 0.98$ & $-5.5 \pm 1.0$ &  & \\
C35111 & $-0.21 \pm 0.44$ & $-0.33 \pm 0.12$ & $6.46 \pm 0.14$ & $1.97 \pm 0.19$ & $-3.0 \pm 0.3$ & $-8.3 \pm 0.8$ & CTTS\\
C35119 & $-0.29 \pm 0.40$ & $-0.49 \pm 0.09$ & $6.77 \pm 0.11$ & $-0.28 \pm 0.88$ & $-5.8 \pm 0.9$ &  & \\
C35122 & $-0.35 \pm 0.39$ & $-0.44 \pm 0.07$ & $6.36 \pm 0.08$ & $-0.39 \pm 1.00$ & $-5.5 \pm 1.0$ &  & \\
C35132 & $-0.42 \pm 0.41$ & $-0.48 \pm 0.08$ & $6.64 \pm 0.10$ & $0.05 \pm 1.03$ & $-5.4 \pm 1.0$ &  & \\
C35140 & $-0.32 \pm 0.42$ & $-0.44 \pm 0.09$ & $6.28 \pm 0.08$ & $2.03 \pm 0.11$ & $-3.0 \pm 0.2$ & $-8.2 \pm 0.8$ & CTTS\\
C35186 & $0.43 \pm 0.33$ & $-0.35 \pm 0.19$ & $6.38 \pm 0.23$ & $2.04 \pm 0.13$ & $-2.9 \pm 0.5$ & $-8.1 \pm 0.9$ & CTTS\\
C35188 & $-0.52 \pm 0.41$ & $-0.80 \pm 0.11$ & $6.58 \pm 0.08$ & $0.33 \pm 0.83$ & $-5.8 \pm 0.8$ &  & \\
C35239 & $-0.40 \pm 0.38$ & $-0.60 \pm 0.09$ & $6.31 \pm 0.06$ & $-0.16 \pm 0.86$ & $-5.7 \pm 0.9$ &  & \\
C35263 & $-0.54 \pm 0.35$ & $-0.15 \pm 0.10$ & $6.67 \pm 0.27$ & $-0.50 \pm 1.04$ & $-5.2 \pm 1.0$ &  & \\
C35309 & $-0.41 \pm 0.42$ & $-0.65 \pm 0.08$ & $6.80 \pm 0.09$ & $2.26 \pm 0.10$ & $-3.7 \pm 0.2$ & $-9.3 \pm 0.7$ & CTTS\\
C35310 & $-0.41 \pm 0.39$ & $-0.62 \pm 0.08$ & $6.78 \pm 0.10$ & $0.19 \pm 0.86$ & $-5.7 \pm 0.9$ &  & \\
C35319 & $-0.49 \pm 0.36$ & $-0.15 \pm 0.14$ & $6.09 \pm 0.19$ & $-0.94 \pm 1.19$ & $-5.2 \pm 1.2$ &  & \\
C35339 & $-0.36 \pm 0.43$ & $-0.58 \pm 0.10$ & $6.46 \pm 0.07$ & $-0.17 \pm 0.97$ & $-5.8 \pm 1.0$ &  & \\
C35351 & $-0.13 \pm 0.56$ & $-0.44 \pm 0.21$ & $6.04 \pm 0.31$ & $-0.95 \pm 1.42$ & $-5.8 \pm 1.6$ &  & \\
C35443 & $-0.09 \pm 0.49$ & $-0.42 \pm 0.14$ & $6.51 \pm 0.16$ & $-0.76 \pm 1.13$ & $-6.0 \pm 1.2$ &  & \\
C35444 & $-0.41 \pm 0.45$ & $-0.59 \pm 0.12$ & $6.20 \pm 0.12$ & $1.65 \pm 0.48$ & $-3.8 \pm 0.5$ & $-9.1 \pm 1.0$ & CTTS\\
C35490 & $-0.44 \pm 0.45$ & $-0.62 \pm 0.11$ & $6.36 \pm 0.07$ & $0.05 \pm 1.13$ & $-5.5 \pm 1.1$ &  & \\
C35491 & $-0.47 \pm 0.45$ & $-0.54 \pm 0.10$ & $5.90 \pm 0.20$ & $0.21 \pm 1.10$ & $-4.8 \pm 1.1$ &  & \\
C35520 & $-0.34 \pm 0.41$ & $-0.58 \pm 0.09$ & $7.47 \pm 0.14$ & $0.14 \pm 0.75$ & $-6.0 \pm 0.8$ &  & \\
C35524 & $-0.30 \pm 0.41$ & $-0.33 \pm 0.10$ & $6.44 \pm 0.13$ & $1.67 \pm 0.26$ & $-3.2 \pm 0.3$ & $-8.7 \pm 0.8$ & CTTS\\
C35536 & $-0.34 \pm 0.35$ & $-0.34 \pm 0.09$ & $6.69 \pm 0.14$ & $-0.44 \pm 0.98$ & $-5.6 \pm 1.0$ &  & \\
C35615 & $-0.21 \pm 0.55$ & $-0.32 \pm 0.16$ & $6.24 \pm 0.21$ & $-1.29 \pm 1.68$ & $-6.0 \pm 1.9$ &  & \\
C35631 & $-0.40 \pm 0.41$ & $-0.52 \pm 0.08$ & $6.19 \pm 0.07$ & $-0.33 \pm 0.97$ & $-5.5 \pm 1.0$ &  & \\
C35673 & $-0.59 \pm 0.35$ & $-0.05 \pm 0.12$ & $6.30 \pm 0.26$ & $1.81 \pm 0.38$ & $-2.4 \pm 0.4$ & $-7.5 \pm 0.9$ & CTTS\\
C35681 & $-0.32 \pm 0.36$ & $-0.59 \pm 0.07$ & $6.83 \pm 0.08$ & $-0.18 \pm 0.74$ & $-6.0 \pm 0.7$ &  & \\
C35692 & $-0.37 \pm 0.42$ & $-0.51 \pm 0.12$ & $6.23 \pm 0.20$ & $-0.24 \pm 0.90$ & $-5.4 \pm 0.9$ &  & \\
C35697 & $-0.36 \pm 0.40$ & $-0.39 \pm 0.10$ & $6.42 \pm 0.20$ & $-0.16 \pm 1.03$ & $-5.2 \pm 1.1$ &  & \\
C35719 & $-0.39 \pm 0.39$ & $-0.41 \pm 0.08$ & $6.42 \pm 0.11$ & $-0.15 \pm 1.02$ & $-5.2 \pm 1.0$ &  & \\
C35732 & $-0.45 \pm 0.40$ & $-0.58 \pm 0.06$ & $6.79 \pm 0.07$ & $1.12 \pm 0.77$ & $-4.7 \pm 0.8$ &  & \\
C35738 & $-0.60 \pm 0.41$ & $-0.78 \pm 0.10$ & $6.25 \pm 0.21$ & $1.10 \pm 0.77$ & $-4.8 \pm 0.8$ &  & \\
C35756 & $-0.33 \pm 0.43$ & $-0.45 \pm 0.10$ & $6.59 \pm 0.17$ & $1.81 \pm 0.15$ & $-3.5 \pm 0.3$ & $-9.0 \pm 0.8$ & CTTS\\
C35800 & $-0.41 \pm 0.37$ & $-0.21 \pm 0.13$ & $6.16 \pm 0.26$ & $-0.72 \pm 1.11$ & $-5.1 \pm 1.1$ &  & \\
C35803 & $-0.36 \pm 0.36$ & $-0.28 \pm 0.11$ & $6.17 \pm 0.13$ & $-0.65 \pm 1.12$ & $-5.2 \pm 1.1$ &  & \\
C35846 & $0.16 \pm 0.47$ & $-0.41 \pm 0.18$ & $6.30 \pm 0.20$ & $-1.18 \pm 1.20$ & $-6.2 \pm 1.4$ &  & \\
C35851 & $-0.56 \pm 0.36$ & $-0.02 \pm 0.08$ & $6.82 \pm 0.36$ & $-0.41 \pm 1.03$ & $-4.9 \pm 1.0$ &  & \\
C35881 & $-0.46 \pm 0.40$ & $-0.76 \pm 0.12$ & $6.58 \pm 0.08$ & $-0.09 \pm 0.77$ & $-6.2 \pm 0.8$ &  & \\
C35894 & $-0.19 \pm 0.54$ & $-0.48 \pm 0.19$ & $5.78 \pm 0.24$ & $-0.74 \pm 1.32$ & $-5.6 \pm 1.5$ &  & \\
C35896 & $0.23 \pm 0.63$ & $-0.42 \pm 0.29$ & $6.10 \pm 0.39$ & $-0.06 \pm 1.73$ & $-4.9 \pm 2.3$ &  & \\
C35908 & $-0.08 \pm 0.53$ & $-0.40 \pm 0.15$ & $6.27 \pm 0.10$ & $1.93 \pm 0.35$ & $-3.0 \pm 0.5$ & $-8.2 \pm 0.9$ & CTTS\\
C35926 & $-0.41 \pm 0.40$ & $-0.50 \pm 0.07$ & $6.57 \pm 0.07$ & $-0.15 \pm 0.96$ & $-5.6 \pm 1.0$ &  & \\
C35931 & $-0.52 \pm 0.41$ & $-0.72 \pm 0.11$ & $6.48 \pm 0.12$ & $0.14 \pm 0.89$ & $-5.8 \pm 0.9$ &  & \\
C35942 & $-0.37 \pm 0.38$ & $-0.25 \pm 0.12$ & $6.31 \pm 0.23$ & $-0.75 \pm 1.11$ & $-5.4 \pm 1.1$ &  & \\
C35948 & $-0.50 \pm 0.37$ & $-0.77 \pm 0.09$ & $6.71 \pm 0.07$ & $1.09 \pm 0.73$ & $-5.1 \pm 0.7$ &  & \\
C35958 & $-0.36 \pm 0.48$ & $-0.68 \pm 0.12$ & $6.92 \pm 0.10$ & $0.28 \pm 0.93$ & $-5.8 \pm 0.9$ &  & \\
C36002 & $-0.39 \pm 0.45$ & $-0.41 \pm 0.10$ & $6.44 \pm 0.10$ & $0.06 \pm 1.20$ & $-5.1 \pm 1.2$ &  & \\
C36016 & $-0.46 \pm 0.38$ & $-0.57 \pm 0.05$ & $6.83 \pm 0.07$ & $0.32 \pm 0.94$ & $-5.4 \pm 1.0$ &  & \\
C36018 & $-0.55 \pm 0.36$ & $0.01 \pm 0.09$ & $6.71 \pm 0.41$ & $-0.52 \pm 1.10$ & $-4.8 \pm 1.1$ &  & \\
C36032 & $-0.37 \pm 0.45$ & $-0.48 \pm 0.13$ & $5.93 \pm 0.22$ & $1.65 \pm 0.37$ & $-3.2 \pm 0.5$ & $-8.2 \pm 0.9$ & CTTS\\
C36070 & $-0.38 \pm 0.37$ & $-0.62 \pm 0.06$ & $6.76 \pm 0.07$ & $-0.07 \pm 0.79$ & $-6.0 \pm 0.8$ &  & \\
C36071 & $-0.31 \pm 0.41$ & $-0.36 \pm 0.11$ & $6.30 \pm 0.15$ & $-0.72 \pm 1.17$ & $-5.6 \pm 1.2$ &  & \\
C36135 & $-0.34 \pm 0.38$ & $-0.32 \pm 0.13$ & $5.87 \pm 0.14$ & $-0.74 \pm 1.13$ & $-5.1 \pm 1.1$ &  & \\
C36169 & $-0.32 \pm 0.42$ & $-0.48 \pm 0.12$ & $6.60 \pm 0.20$ & $-0.19 \pm 0.90$ & $-5.6 \pm 1.0$ &  & \\
C36198 & $0.14 \pm 0.65$ & $-0.34 \pm 0.24$ & $5.97 \pm 0.22$ & $-0.34 \pm 2.28$ & $-4.9 \pm 2.7$ &  & \\
C36216 & $-0.41 \pm 0.41$ & $-0.36 \pm 0.10$ & $6.48 \pm 0.15$ & $-0.17 \pm 1.26$ & $-5.2 \pm 1.3$ &  & \\
C36252 & $-0.36 \pm 0.44$ & $-0.44 \pm 0.12$ & $6.20 \pm 0.18$ & $-0.34 \pm 1.08$ & $-5.3 \pm 1.1$ &  & \\
C36287 & $-0.31 \pm 0.41$ & $-0.41 \pm 0.10$ & $6.21 \pm 0.15$ & $-0.52 \pm 1.10$ & $-5.4 \pm 1.1$ &  & \\
C36368 & $-0.29 \pm 0.42$ & $-0.25 \pm 0.14$ & $6.38 \pm 0.19$ & $-1.08 \pm 1.25$ & $-5.8 \pm 1.3$ &  & \\
C36389 & $-0.37 \pm 0.39$ & $-0.46 \pm 0.09$ & $6.19 \pm 0.07$ & $-0.43 \pm 1.00$ & $-5.4 \pm 1.0$ &  & \\
C36407 & $-0.42 \pm 0.43$ & $-0.58 \pm 0.10$ & $6.20 \pm 0.09$ & $-0.22 \pm 0.98$ & $-5.6 \pm 1.0$ &  & \\
C36437 & $0.07 \pm 0.51$ & $-0.29 \pm 0.17$ & $6.18 \pm 0.15$ & $1.59 \pm 0.71$ & $-3.0 \pm 0.8$ & $-8.2 \pm 1.4$ & CTTS\\
C36493 & $0.43 \pm 0.60$ & $-0.30 \pm 0.32$ & $5.94 \pm 0.31$ & $-1.09 \pm 1.70$ & $-5.6 \pm 2.2$ &  & \\
C36596 & $-0.32 \pm 0.44$ & $-0.56 \pm 0.08$ & $6.58 \pm 0.07$ & $-0.47 \pm 0.96$ & $-6.1 \pm 0.9$ &  & \\
C36597 & $-0.34 \pm 0.39$ & $-0.41 \pm 0.08$ & $6.49 \pm 0.09$ & $-0.38 \pm 1.02$ & $-5.5 \pm 1.0$ &  & \\
C36634 & $-0.49 \pm 0.36$ & $-0.46 \pm 0.06$ & $7.79 \pm 0.13$ & $0.06 \pm 0.75$ & $-6.0 \pm 0.8$ &  & \\
C36662 & $-0.34 \pm 0.36$ & $-0.59 \pm 0.08$ & $6.56 \pm 0.07$ & $-0.21 \pm 0.77$ & $-5.9 \pm 0.8$ &  & \\
C36696 & $-0.34 \pm 0.37$ & $-0.47 \pm 0.06$ & $6.69 \pm 0.08$ & $-0.23 \pm 0.88$ & $-5.7 \pm 0.9$ &  & \\
C36702 & $-0.44 \pm 0.46$ & $-0.86 \pm 0.18$ & $6.25 \pm 0.23$ & $-0.23 \pm 0.77$ & $-6.3 \pm 0.8$ &  & \\
C36709 & $-0.34 \pm 0.41$ & $-0.48 \pm 0.08$ & $6.31 \pm 0.06$ & $-0.40 \pm 0.97$ & $-5.6 \pm 1.0$ &  & \\
C36710 & $-0.38 \pm 0.40$ & $-0.52 \pm 0.08$ & $6.76 \pm 0.10$ & $-0.12 \pm 0.88$ & $-5.7 \pm 0.9$ &  & \\
C36714 & $-0.39 \pm 0.40$ & $-0.55 \pm 0.09$ & $6.36 \pm 0.06$ & $-0.12 \pm 0.90$ & $-5.5 \pm 0.9$ &  & \\
C36794 & $-0.39 \pm 0.42$ & $-0.49 \pm 0.09$ & $6.57 \pm 0.13$ & $-0.09 \pm 1.00$ & $-5.5 \pm 1.0$ &  & \\
C36810 & $0.32 \pm 0.43$ & $-0.29 \pm 0.18$ & $6.62 \pm 0.22$ & $1.96 \pm 0.63$ & $-3.0 \pm 0.8$ & $-8.4 \pm 1.2$ & CTTS\\
C36813 & $-0.23 \pm 0.41$ & $-0.30 \pm 0.14$ & $6.23 \pm 0.31$ & $-0.74 \pm 1.16$ & $-5.3 \pm 1.2$ &  & \\
C36818 & $-0.32 \pm 0.40$ & $-0.33 \pm 0.10$ & $6.16 \pm 0.11$ & $-0.55 \pm 1.18$ & $-5.2 \pm 1.2$ &  & \\
C36828 & $-0.27 \pm 0.49$ & $-0.56 \pm 0.12$ & $6.68 \pm 0.12$ & $2.33 \pm 0.10$ & $-3.3 \pm 0.3$ & $-8.8 \pm 0.8$ & CTTS\\
C36831 & $-0.34 \pm 0.38$ & $-0.45 \pm 0.07$ & $6.67 \pm 0.09$ & $-0.26 \pm 0.93$ & $-5.6 \pm 0.9$ &  & \\
C36835 & $-0.44 \pm 0.42$ & $-0.57 \pm 0.06$ & $6.46 \pm 0.06$ & $0.35 \pm 1.05$ & $-5.2 \pm 1.1$ &  & \\
C36839 & $-0.45 \pm 0.38$ & $-0.53 \pm 0.06$ & $6.74 \pm 0.07$ & $0.22 \pm 0.97$ & $-5.4 \pm 1.0$ &  & \\
C36876 & $-0.39 \pm 0.35$ & $-0.48 \pm 0.07$ & $7.34 \pm 0.14$ & $0.11 \pm 0.80$ & $-5.7 \pm 0.8$ &  & \\
C36877 & $-0.43 \pm 0.35$ & $-0.30 \pm 0.09$ & $6.57 \pm 0.16$ & $-0.44 \pm 1.06$ & $-5.4 \pm 1.0$ &  & \\
C36879 & $-0.34 \pm 0.45$ & $-0.52 \pm 0.13$ & $5.53 \pm 0.27$ & $1.61 \pm 0.41$ & $-3.3 \pm 0.5$ & $-8.2 \pm 1.0$ & CTTS\\
C36887 & $-0.41 \pm 0.36$ & $-0.52 \pm 0.05$ & $6.69 \pm 0.07$ & $0.03 \pm 0.91$ & $-5.5 \pm 0.9$ &  & \\
C36888 & $-0.55 \pm 0.37$ & $-0.16 \pm 0.11$ & $6.57 \pm 0.28$ & $-0.41 \pm 1.08$ & $-5.0 \pm 1.1$ &  & \\
C36891 & $-0.13 \pm 0.55$ & $-0.47 \pm 0.17$ & $6.14 \pm 0.13$ & $-1.16 \pm 1.29$ & $-6.2 \pm 1.5$ &  & \\
C36902 & $0.23 \pm 0.26$ & $-0.75 \pm 0.18$ & $6.60 \pm 0.10$ & $2.02 \pm 0.16$ & $-4.0 \pm 0.4$ & $-9.6 \pm 0.8$ & CTTS\\
C37041 & $-0.41 \pm 0.41$ & $-0.24 \pm 0.13$ & $6.31 \pm 0.22$ & $-0.97 \pm 1.30$ & $-5.6 \pm 1.3$ &  & \\
C37068 & $-0.38 \pm 0.45$ & $-0.66 \pm 0.14$ & $6.55 \pm 0.15$ & $-0.09 \pm 0.86$ & $-5.9 \pm 0.9$ &  & \\
C37103 & $-0.50 \pm 0.35$ & $-0.12 \pm 0.13$ & $6.20 \pm 0.22$ & $-0.64 \pm 1.08$ & $-4.9 \pm 1.1$ &  & \\
C37104 & $-0.48 \pm 0.35$ & $-0.25 \pm 0.09$ & $6.61 \pm 0.19$ & $-0.32 \pm 1.03$ & $-5.2 \pm 1.0$ &  & \\
C37171 & $-0.31 \pm 0.43$ & $-0.46 \pm 0.12$ & $5.56 \pm 0.26$ & $-0.71 \pm 1.10$ & $-5.3 \pm 1.1$ &  & \\
C37217 & $-0.36 \pm 0.51$ & $-0.28 \pm 0.15$ & $6.15 \pm 0.21$ & $-0.68 \pm 1.88$ & $-5.2 \pm 2.0$ &  & \\
C37237 & $-0.47 \pm 0.39$ & $-0.28 \pm 0.09$ & $6.47 \pm 0.16$ & $1.33 \pm 0.71$ & $-3.5 \pm 0.7$ & $-9.1 \pm 1.3$ & CTTS\\
C37363 & $0.13 \pm 0.47$ & $-0.23 \pm 0.21$ & $5.99 \pm 0.25$ & $1.99 \pm 0.12$ & $-2.3 \pm 0.4$ & $-7.0 \pm 0.8$ & CTTS\\
C37366 & $0.01 \pm 0.52$ & $-0.46 \pm 0.18$ & $7.39 \pm 0.21$ & $2.38 \pm 0.13$ & $-3.4 \pm 0.5$ & $-9.2 \pm 1.0$ & CTTS\\
C37387 & $-0.43 \pm 0.39$ & $-0.56 \pm 0.06$ & $6.56 \pm 0.06$ & $0.11 \pm 0.95$ & $-5.5 \pm 0.9$ &  & \\
C37535 & $-0.35 \pm 0.41$ & $-0.42 \pm 0.11$ & $6.21 \pm 0.14$ & $-0.28 \pm 1.05$ & $-5.2 \pm 1.1$ &  & \\
C37581 & $-0.38 \pm 0.39$ & $-0.42 \pm 0.07$ & $6.53 \pm 0.09$ & $-0.23 \pm 1.03$ & $-5.4 \pm 1.0$ &  & \\
C37590 & $-0.41 \pm 0.35$ & $-0.29 \pm 0.09$ & $6.63 \pm 0.16$ & $-0.45 \pm 1.03$ & $-5.4 \pm 1.0$ &  & \\
C37612 & $0.79 \pm 0.15$ & $-0.09 \pm 0.23$ & $6.12 \pm 0.39$ & $-1.65 \pm 1.28$ & $-5.7 \pm 1.4$ &  & \\
C37707 & $-0.21 \pm 0.41$ & $-0.44 \pm 0.11$ & $7.17 \pm 0.18$ & $2.73 \pm 0.09$ & $-2.9 \pm 0.2$ & $-8.4 \pm 0.7$ & CTTS\\
C37748 & $-0.40 \pm 0.40$ & $-0.34 \pm 0.14$ & $5.60 \pm 0.26$ & $-0.55 \pm 1.09$ & $-4.8 \pm 1.1$ &  & \\
C37798 & $-0.46 \pm 0.36$ & $-0.18 \pm 0.13$ & $6.12 \pm 0.21$ & $-0.76 \pm 1.12$ & $-5.1 \pm 1.1$ &  & \\
C37800 & $-0.38 \pm 0.38$ & $-0.48 \pm 0.07$ & $6.55 \pm 0.09$ & $-0.16 \pm 0.93$ & $-5.5 \pm 0.9$ &  & \\
C37804 & $-0.06 \pm 0.55$ & $-0.45 \pm 0.18$ & $6.09 \pm 0.21$ & $2.15 \pm 0.50$ & $-2.7 \pm 0.7$ & $-7.6 \pm 1.1$ & CTTS\\
C37902 & $-0.25 \pm 0.37$ & $-0.38 \pm 0.09$ & $6.58 \pm 0.12$ & $-0.47 \pm 0.96$ & $-5.6 \pm 1.0$ &  & \\
C37904 & $-0.36 \pm 0.37$ & $-0.35 \pm 0.08$ & $6.48 \pm 0.11$ & $-0.38 \pm 1.07$ & $-5.4 \pm 1.1$ &  & \\
C37927 & $-0.46 \pm 0.39$ & $-0.46 \pm 0.06$ & $6.50 \pm 0.07$ & $0.06 \pm 1.00$ & $-5.2 \pm 1.0$ &  & \\
C38035 & $-0.36 \pm 0.40$ & $-0.53 \pm 0.10$ & $6.77 \pm 0.13$ & $-0.05 \pm 0.88$ & $-5.7 \pm 0.9$ &  & \\
C38110 & $-0.25 \pm 0.44$ & $-0.40 \pm 0.11$ & $6.17 \pm 0.09$ & $2.16 \pm 0.10$ & $-2.7 \pm 0.2$ & $-7.6 \pm 0.8$ & CTTS\\
C38146 & $-0.37 \pm 0.38$ & $-0.63 \pm 0.09$ & $6.58 \pm 0.07$ & $-0.17 \pm 0.79$ & $-6.0 \pm 0.8$ &  & \\
C38152 & $0.48 \pm 0.20$ & $-0.65 \pm 0.22$ & $5.76 \pm 0.31$ & $1.97 \pm 0.23$ & $-3.5 \pm 0.6$ & $-8.5 \pm 1.0$ & CTTS\\
C38178 & $-0.66 \pm 0.30$ & $-0.02 \pm 0.02$ & $7.71 \pm 0.21$ & $-0.07 \pm 0.89$ & $-4.6 \pm 0.9$ &  & \\
C38296 & $-0.31 \pm 0.38$ & $-0.44 \pm 0.08$ & $6.33 \pm 0.08$ & $-0.40 \pm 0.98$ & $-5.5 \pm 1.0$ &  & \\
C38384 & $-0.39 \pm 0.37$ & $-0.60 \pm 0.07$ & $6.81 \pm 0.08$ & $-0.09 \pm 0.79$ & $-5.9 \pm 0.8$ &  & \\
C38449 & $-0.33 \pm 0.37$ & $-0.30 \pm 0.11$ & $6.37 \pm 0.15$ & $-0.61 \pm 1.09$ & $-5.4 \pm 1.1$ &  & \\
C38523 & $-0.40 \pm 0.42$ & $-0.31 \pm 0.12$ & $6.35 \pm 0.21$ & $-0.58 \pm 1.32$ & $-5.4 \pm 1.3$ &  & \\
C38553 & $-0.36 \pm 0.42$ & $-0.62 \pm 0.10$ & $6.70 \pm 0.09$ & $-0.11 \pm 0.82$ & $-6.0 \pm 0.8$ &  & \\
C38598 & $-0.39 \pm 0.42$ & $-0.81 \pm 0.12$ & $6.62 \pm 0.07$ & $-0.07 \pm 0.75$ & $-6.2 \pm 0.8$ &  & \\
C38632 & $-0.39 \pm 0.37$ & $-0.36 \pm 0.08$ & $6.51 \pm 0.13$ & $-0.22 \pm 1.05$ & $-5.3 \pm 1.1$ &  & \\
C38691 & $-0.31 \pm 0.50$ & $-0.65 \pm 0.14$ & $7.14 \pm 0.15$ & $1.76 \pm 0.27$ & $-4.4 \pm 0.4$ & $-10.5 \pm 0.9$ & CTTS\\
C38841 & $-0.41 \pm 0.38$ & $-0.41 \pm 0.08$ & $6.83 \pm 0.12$ & $-0.16 \pm 0.99$ & $-5.5 \pm 1.0$ &  & \\
C39036 & $-0.54 \pm 0.35$ & $-0.02 \pm 0.03$ & $7.40 \pm 0.34$ & $-0.35 \pm 1.02$ & $-4.9 \pm 1.0$ &  & \\
C39085 & $-0.32 \pm 0.35$ & $-0.39 \pm 0.09$ & $7.06 \pm 0.16$ & $-0.23 \pm 0.85$ & $-5.7 \pm 0.9$ &  & \\
C39139 & $-0.44 \pm 0.44$ & $-0.71 \pm 0.12$ & $6.62 \pm 0.08$ & $0.15 \pm 0.88$ & $-5.8 \pm 0.9$ &  & \\
C39156 & $-0.42 \pm 0.41$ & $-0.34 \pm 0.10$ & $6.47 \pm 0.18$ & $-0.15 \pm 1.20$ & $-5.1 \pm 1.2$ &  & \\
C39192 & $-0.40 \pm 0.37$ & $-0.63 \pm 0.06$ & $6.82 \pm 0.07$ & $0.09 \pm 0.83$ & $-5.8 \pm 0.8$ &  & \\
C39235 & $-0.41 \pm 0.39$ & $-0.26 \pm 0.12$ & $6.42 \pm 0.26$ & $-0.56 \pm 1.11$ & $-5.3 \pm 1.1$ &  & \\
C39289 & $-0.31 \pm 0.41$ & $-0.39 \pm 0.10$ & $6.54 \pm 0.14$ & $-0.48 \pm 1.09$ & $-5.6 \pm 1.1$ &  & \\
C39377 & $-0.42 \pm 0.35$ & $-0.26 \pm 0.09$ & $6.64 \pm 0.20$ & $2.07 \pm 0.10$ & $-2.8 \pm 0.2$ & $-8.2 \pm 0.7$ & CTTS\\
C39439 & $-0.34 \pm 0.42$ & $-0.50 \pm 0.07$ & $6.65 \pm 0.08$ & $2.12 \pm 0.11$ & $-3.4 \pm 0.2$ & $-8.8 \pm 0.7$ & CTTS\\
C39467 & $-0.55 \pm 0.38$ & $-0.01 \pm 0.09$ & $6.69 \pm 0.36$ & $-0.32 \pm 0.98$ & $-4.7 \pm 1.0$ &  & \\
C39532 & $-0.41 \pm 0.40$ & $-0.39 \pm 0.08$ & $6.20 \pm 0.07$ & $-0.31 \pm 1.16$ & $-5.2 \pm 1.2$ &  & \\
C39676 & $-0.36 \pm 0.38$ & $-0.50 \pm 0.07$ & $6.34 \pm 0.07$ & $-0.27 \pm 0.90$ & $-5.5 \pm 0.9$ &  & \\
C39811 & $-0.56 \pm 0.37$ & $-0.16 \pm 0.11$ & $6.36 \pm 0.23$ & $1.11 \pm 0.92$ & $-3.4 \pm 0.9$ & $-9.0 \pm 1.6$ & CTTS\\
C40196 & $-0.45 \pm 0.38$ & $-0.34 \pm 0.09$ & $6.41 \pm 0.13$ & $0.12 \pm 1.18$ & $-4.8 \pm 1.2$ &  & \\
C40291 & $-0.37 \pm 0.40$ & $-0.52 \pm 0.09$ & $6.34 \pm 0.07$ & $-0.27 \pm 0.91$ & $-5.6 \pm 0.9$ &  & \\
C40299 & $-0.39 \pm 0.40$ & $-0.53 \pm 0.08$ & $6.52 \pm 0.07$ & $-0.06 \pm 0.94$ & $-5.6 \pm 0.9$ &  & \\
C40516 & $-0.40 \pm 0.41$ & $-0.58 \pm 0.08$ & $6.65 \pm 0.08$ & $0.06 \pm 0.92$ & $-5.7 \pm 0.9$ &  & \\
C40687 & $-0.22 \pm 0.36$ & $-0.37 \pm 0.09$ & $6.27 \pm 0.09$ & $-0.66 \pm 1.05$ & $-5.5 \pm 1.0$ &  & \\
C40714 & $-0.30 \pm 0.39$ & $-0.34 \pm 0.12$ & $6.47 \pm 0.23$ & $-0.36 \pm 1.03$ & $-5.3 \pm 1.1$ &  & \\
C40866 & $-0.39 \pm 0.38$ & $-0.29 \pm 0.11$ & $6.48 \pm 0.20$ & $-0.67 \pm 1.13$ & $-5.5 \pm 1.1$ &  & \\
C41332 & $-0.40 \pm 0.38$ & $-0.48 \pm 0.06$ & $6.60 \pm 0.07$ & $-0.16 \pm 0.94$ & $-5.6 \pm 0.9$ &  & \\
C41403 & $-0.41 \pm 0.40$ & $-0.52 \pm 0.08$ & $6.48 \pm 0.07$ & $-0.08 \pm 0.93$ & $-5.5 \pm 0.9$ &  & \\
C41828 & $-0.52 \pm 0.35$ & $-0.09 \pm 0.12$ & $6.09 \pm 0.23$ & $-0.61 \pm 1.05$ & $-4.7 \pm 1.0$ &  & \\
C41880 & $-0.31 \pm 0.44$ & $-0.48 \pm 0.09$ & $6.68 \pm 0.10$ & $2.58 \pm 0.09$ & $-2.9 \pm 0.2$ & $-8.1 \pm 0.8$ & CTTS\\
C42487 & $-0.39 \pm 0.45$ & $-0.65 \pm 0.12$ & $6.54 \pm 0.11$ & $1.72 \pm 0.23$ & $-4.1 \pm 0.4$ & $-9.8 \pm 0.8$ & CTTS\\
C42515 & $-0.50 \pm 0.39$ & $-0.28 \pm 0.10$ & $6.47 \pm 0.19$ & $0.10 \pm 1.22$ & $-4.7 \pm 1.2$ &  & \\
C42845 & $-0.42 \pm 0.40$ & $-0.54 \pm 0.07$ & $6.50 \pm 0.07$ & $0.08 \pm 0.96$ & $-5.4 \pm 1.0$ &  & \\
C42979 & $-0.37 \pm 0.40$ & $-0.43 \pm 0.09$ & $6.62 \pm 0.14$ & $-0.17 \pm 0.99$ & $-5.5 \pm 1.0$ &  & \\
C43103 & $-0.56 \pm 0.36$ & $-0.16 \pm 0.10$ & $6.69 \pm 0.27$ & $-0.34 \pm 1.02$ & $-5.1 \pm 1.0$ &  & \\
C43537 & $-0.64 \pm 0.31$ & $-0.07 \pm 0.02$ & $7.73 \pm 0.22$ & $-0.11 \pm 0.87$ & $-4.9 \pm 0.9$ &  & \\
C44065 & $-0.54 \pm 0.42$ & $0.00 \pm 0.10$ & $6.66 \pm 0.41$ & $1.98 \pm 0.11$ & $-2.3 \pm 0.2$ & $-7.4 \pm 0.7$ & CTTS\\
C44423 & $-0.33 \pm 0.38$ & $-0.35 \pm 0.10$ & $6.51 \pm 0.14$ & $-0.51 \pm 1.09$ & $-5.5 \pm 1.1$ &  & \\
C45081 & $0.24 \pm 0.38$ & $-0.65 \pm 0.22$ & $6.56 \pm 0.15$ & $1.66 \pm 0.46$ & $-4.1 \pm 0.7$ & $-9.8 \pm 1.1$ & CTTS\\
C45307 & $-0.35 \pm 0.39$ & $-0.47 \pm 0.07$ & $6.69 \pm 0.08$ & $1.89 \pm 0.13$ & $-3.5 \pm 0.2$ & $-9.1 \pm 0.7$ & CTTS\\
C45397 & $-0.41 \pm 0.43$ & $-0.61 \pm 0.11$ & $6.49 \pm 0.11$ & $0.15 \pm 0.95$ & $-5.5 \pm 1.0$ &  & \\
C45710 & $-0.38 \pm 0.39$ & $-0.26 \pm 0.11$ & $6.42 \pm 0.18$ & $1.91 \pm 0.12$ & $-2.8 \pm 0.2$ & $-8.1 \pm 0.7$ & CTTS\\
C45726 & $-0.35 \pm 0.38$ & $-0.57 \pm 0.07$ & $6.59 \pm 0.07$ & $-0.09 \pm 0.82$ & $-5.7 \pm 0.8$ &  & \\
C45996 & $-0.39 \pm 0.40$ & $-0.50 \pm 0.07$ & $6.44 \pm 0.07$ & $-0.19 \pm 0.94$ & $-5.5 \pm 0.9$ &  & \\
C46131 & $-0.34 \pm 0.37$ & $-0.28 \pm 0.09$ & $7.39 \pm 0.23$ & $-0.48 \pm 0.90$ & $-5.9 \pm 1.0$ &  & \\
C46271 & $-0.39 \pm 0.35$ & $-0.30 \pm 0.09$ & $6.22 \pm 0.13$ & $-0.15 \pm 1.00$ & $-4.8 \pm 1.0$ &  & \\
C46531 & $-0.59 \pm 0.35$ & $-0.03 \pm 0.08$ & $6.71 \pm 0.33$ & $-0.25 \pm 0.98$ & $-4.7 \pm 1.0$ &  & \\
C46679 & $-0.35 \pm 0.35$ & $-0.22 \pm 0.09$ & $7.04 \pm 0.27$ & $-0.61 \pm 0.89$ & $-5.7 \pm 0.9$ &  & \\
C46734 & $-0.41 \pm 0.38$ & $-0.51 \pm 0.05$ & $6.54 \pm 0.07$ & $-0.11 \pm 0.92$ & $-5.6 \pm 0.9$ &  & \\
C46974 & $-0.37 \pm 0.39$ & $-0.47 \pm 0.07$ & $6.65 \pm 0.09$ & $-0.15 \pm 0.93$ & $-5.5 \pm 0.9$ &  & \\
C47486 & $-0.56 \pm 0.36$ & $-0.11 \pm 0.11$ & $6.52 \pm 0.27$ & $-0.42 \pm 1.04$ & $-4.9 \pm 1.0$ &  & \\
C47640 & $-0.37 \pm 0.37$ & $-0.31 \pm 0.10$ & $6.46 \pm 0.15$ & $-0.56 \pm 1.10$ & $-5.5 \pm 1.1$ &  & \\
C48145 & $-0.58 \pm 0.33$ & $-0.08 \pm 0.03$ & $7.64 \pm 0.25$ & $-0.16 \pm 0.94$ & $-5.0 \pm 0.9$ &  & \\
C48240 & $-0.29 \pm 0.46$ & $-0.30 \pm 0.13$ & $6.23 \pm 0.14$ & $1.48 \pm 0.69$ & $-3.2 \pm 0.7$ & $-8.5 \pm 1.3$ & CTTS\\
C48749 & $-0.53 \pm 0.34$ & $-0.20 \pm 0.04$ & $7.59 \pm 0.24$ & $-0.37 \pm 0.82$ & $-5.6 \pm 0.8$ &  & \\
C49287 & $-0.44 \pm 0.42$ & $-0.53 \pm 0.07$ & $6.74 \pm 0.10$ & $0.75 \pm 0.97$ & $-4.9 \pm 1.0$ &  & \\
C49334 & $-0.44 \pm 0.38$ & $-0.66 \pm 0.06$ & $6.72 \pm 0.07$ & $0.05 \pm 0.82$ & $-5.9 \pm 0.8$ &  & \\
C50879 & $-0.32 \pm 0.38$ & $-0.38 \pm 0.08$ & $6.59 \pm 0.12$ & $2.41 \pm 0.09$ & $-2.8 \pm 0.2$ & $-7.9 \pm 0.7$ & CTTS\\
C51126 & $-0.38 \pm 0.36$ & $-0.15 \pm 0.08$ & $7.13 \pm 0.32$ & $-0.64 \pm 0.87$ & $-5.6 \pm 0.9$ &  & \\
C54567 & $-0.24 \pm 0.49$ & $-0.54 \pm 0.13$ & $6.80 \pm 0.10$ & $2.33 \pm 0.10$ & $-3.4 \pm 0.3$ & $-8.8 \pm 0.8$ & CTTS\\
C57195 & $-0.59 \pm 0.36$ & $-0.00 \pm 0.11$ & $6.45 \pm 0.31$ & $1.98 \pm 0.26$ & $-2.2 \pm 0.3$ & $-7.3 \pm 0.8$ & CTTS\\
C59756 & $-0.27 \pm 0.48$ & $-0.45 \pm 0.13$ & $6.84 \pm 0.17$ & $-0.29 \pm 1.08$ & $-5.8 \pm 1.1$ &  & \\
C63956 & $-0.64 \pm 0.31$ & $-0.01 \pm 0.03$ & $7.68 \pm 0.24$ & $0.04 \pm 0.96$ & $-4.4 \pm 1.0$ &  & \\
C8431 & $-0.45 \pm 0.40$ & $-0.67 \pm 0.07$ & $6.62 \pm 0.06$ & $1.88 \pm 0.15$ & $-4.0 \pm 0.2$ & $-9.7 \pm 0.7$ & CTTS\\
C8481 & $-0.38 \pm 0.41$ & $-0.56 \pm 0.08$ & $6.88 \pm 0.10$ & $1.76 \pm 0.19$ & $-4.0 \pm 0.3$ & $-9.9 \pm 0.8$ & CTTS\\
C9452 & $-0.50 \pm 0.34$ & $-0.26 \pm 0.07$ & $7.30 \pm 0.22$ & $-0.26 \pm 0.86$ & $-5.6 \pm 0.9$ &  & \\
S2779 & $-0.26 \pm 0.42$ & $-0.24 \pm 0.15$ & $5.41 \pm 0.28$ & $-2.44 \pm 1.07$ & $-6.4 \pm 1.1$ &  & \\
S2783 & $-0.49 \pm 0.38$ & $-0.22 \pm 0.11$ & $6.32 \pm 0.19$ & $1.51 \pm 0.50$ & $-3.1 \pm 0.5$ & $-8.4 \pm 1.0$ & CTTS\\
S2791 & $-0.50 \pm 0.36$ & $-0.14 \pm 0.12$ & $6.42 \pm 0.27$ & $-0.76 \pm 1.11$ & $-5.2 \pm 1.1$ &  & \\
S2795 & $-0.62 \pm 0.40$ & $0.19 \pm 0.07$ & $6.74 \pm 0.56$ & $-0.66 \pm 1.35$ & $-4.4 \pm 1.3$ &  & \\
S2818 & $-0.50 \pm 0.35$ & $0.01 \pm 0.12$ & $6.27 \pm 0.37$ & $-0.49 \pm 1.07$ & $-4.5 \pm 1.0$ &  & \\
S2985 & $-0.76 \pm 0.35$ & $0.19 \pm 0.09$ & $6.31 \pm 0.38$ & $0.45 \pm 1.14$ & $-3.3 \pm 1.1$ &  & \\
W1172 & $-0.39 \pm 0.46$ & $-0.18 \pm 0.16$ & $6.34 \pm 0.35$ & $1.51 \pm 0.61$ & $-3.0 \pm 0.7$ & $-8.3 \pm 1.2$ & CTTS\\
W1243 & $-0.40 \pm 0.40$ & $-0.30 \pm 0.12$ & $5.98 \pm 0.11$ & $-1.01 \pm 1.35$ & $-5.4 \pm 1.3$ &  & \\
W1322 & $-0.38 \pm 0.45$ & $-0.27 \pm 0.15$ & $6.18 \pm 0.28$ & $-0.47 \pm 1.46$ & $-5.0 \pm 1.5$ &  & \\
W1616 & $-0.59 \pm 0.40$ & $-0.10 \pm 0.12$ & $6.44 \pm 0.31$ & $0.73 \pm 1.22$ & $-3.7 \pm 1.2$ &  & \\
W1735 & $-0.60 \pm 0.42$ & $0.04 \pm 0.09$ & $6.57 \pm 0.39$ & $1.63 \pm 0.30$ & $-2.5 \pm 0.3$ & $-7.8 \pm 0.9$ & CTTS\\
W2320 & $-0.69 \pm 0.36$ & $0.04 \pm 0.07$ & $6.76 \pm 0.36$ & $0.38 \pm 1.20$ & $-3.9 \pm 1.2$ &  & \\
W2690 & $-0.51 \pm 0.44$ & $-0.17 \pm 0.13$ & $6.48 \pm 0.33$ & $1.09 \pm 1.10$ & $-3.5 \pm 1.1$ & $-9.1 \pm 1.8$ & CTTS\\
W3248 & $-0.33 \pm 0.46$ & $0.24 \pm 0.06$ & $7.09 \pm 0.50$ & $-0.72 \pm 1.36$ & $-4.2 \pm 1.3$ &  & \\
W3407 & $-0.55 \pm 0.42$ & $-0.13 \pm 0.15$ & $6.14 \pm 0.21$ & $-1.15 \pm 1.66$ & $-5.4 \pm 1.6$ &  & \\
W3468 & $-0.47 \pm 0.41$ & $0.20 \pm 0.04$ & $7.16 \pm 0.46$ & $-0.78 \pm 1.35$ & $-4.4 \pm 1.3$ &  & \\
W3778 & $-0.54 \pm 0.36$ & $-0.16 \pm 0.12$ & $6.42 \pm 0.25$ & $-0.73 \pm 1.17$ & $-5.3 \pm 1.1$ &  & \\
W3814 & $0.29 \pm 0.19$ & $-0.07 \pm 0.14$ & $5.31 \pm 0.21$ & $-2.93 \pm 1.20$ & $-6.4 \pm 1.3$ &  & \\
W3820 & $-0.68 \pm 0.36$ & $0.19 \pm 0.10$ & $6.31 \pm 0.39$ & $-0.24 \pm 1.01$ & $-4.0 \pm 1.0$ &  & \\
W3902 & $0.21 \pm 0.36$ & $-0.06 \pm 0.18$ & $6.44 \pm 0.33$ & $1.89 \pm 0.90$ & $-2.4 \pm 1.0$ & $-7.5 \pm 1.5$ & CTTS\\
W3905 & $-0.65 \pm 0.32$ & $0.10 \pm 0.13$ & $5.99 \pm 0.26$ & $-0.20 \pm 0.94$ & $-3.9 \pm 0.9$ &  & \\
W4031 & $-0.48 \pm 0.38$ & $-0.23 \pm 0.16$ & $5.76 \pm 0.25$ & $-0.51 \pm 1.07$ & $-4.6 \pm 1.0$ &  & \\
W4221 & $-0.53 \pm 0.38$ & $-0.02 \pm 0.11$ & $6.61 \pm 0.43$ & $-0.58 \pm 1.12$ & $-4.9 \pm 1.1$ &  & \\
W4267 & $-0.56 \pm 0.37$ & $-0.11 \pm 0.11$ & $6.43 \pm 0.25$ & $1.97 \pm 0.12$ & $-2.5 \pm 0.2$ & $-7.6 \pm 0.7$ & CTTS\\
W4317 & $-0.45 \pm 0.36$ & $-0.17 \pm 0.13$ & $6.14 \pm 0.18$ & $-0.88 \pm 1.14$ & $-5.2 \pm 1.1$ &  & \\
W4428 & $-0.39 \pm 0.40$ & $-0.29 \pm 0.13$ & $5.99 \pm 0.18$ & $-0.75 \pm 1.28$ & $-5.1 \pm 1.3$ &  & \\
W4459 & $-0.55 \pm 0.38$ & $-0.17 \pm 0.13$ & $6.18 \pm 0.23$ & $-0.45 \pm 1.29$ & $-4.8 \pm 1.3$ &  & \\
W4572 & $-0.34 \pm 0.48$ & $-0.15 \pm 0.20$ & $6.05 \pm 0.30$ & $1.21 \pm 1.16$ & $-3.0 \pm 1.2$ & $-8.1 \pm 1.9$ & CTTS\\
W4634 & $-0.58 \pm 0.38$ & $-0.16 \pm 0.10$ & $6.74 \pm 0.29$ & $-0.45 \pm 1.14$ & $-5.2 \pm 1.1$ &  & \\
W4654 & $-0.40 \pm 0.40$ & $-0.18 \pm 0.14$ & $6.20 \pm 0.29$ & $1.78 \pm 0.15$ & $-2.6 \pm 0.2$ & $-7.7 \pm 0.7$ & CTTS\\
W4657 & $-0.71 \pm 0.32$ & $0.11 \pm 0.12$ & $6.13 \pm 0.31$ & $-0.13 \pm 1.12$ & $-3.9 \pm 1.1$ &  & \\
W4658 & $-0.51 \pm 0.37$ & $-0.12 \pm 0.13$ & $6.30 \pm 0.23$ & $-0.91 \pm 1.15$ & $-5.3 \pm 1.1$ &  & \\
W4722 & $-0.55 \pm 0.43$ & $-0.19 \pm 0.14$ & $6.18 \pm 0.19$ & $-1.21 \pm 1.72$ & $-5.6 \pm 1.7$ &  & \\
W4731 & $-0.56 \pm 0.36$ & $-0.03 \pm 0.12$ & $6.36 \pm 0.34$ & $-0.38 \pm 1.03$ & $-4.6 \pm 1.0$ &  & \\
W4735 & $-0.45 \pm 0.38$ & $-0.26 \pm 0.10$ & $6.27 \pm 0.20$ & $-0.47 \pm 1.16$ & $-5.1 \pm 1.2$ &  & \\
W4790 & $-0.51 \pm 0.36$ & $-0.13 \pm 0.13$ & $6.17 \pm 0.24$ & $-0.56 \pm 1.07$ & $-4.8 \pm 1.1$ &  & \\
W4800 & $-0.50 \pm 0.34$ & $-0.05 \pm 0.12$ & $6.15 \pm 0.25$ & $-0.52 \pm 1.07$ & $-4.6 \pm 1.0$ &  & \\
W4814 & $-0.68 \pm 0.39$ & $0.11 \pm 0.07$ & $6.64 \pm 0.42$ & $0.68 \pm 1.11$ & $-3.3 \pm 1.1$ &  & \\
W4904 & $-0.40 \pm 0.39$ & $-0.21 \pm 0.14$ & $6.18 \pm 0.28$ & $-0.69 \pm 1.17$ & $-5.1 \pm 1.2$ &  & \\
W4906 & $-0.57 \pm 0.50$ & $-0.06 \pm 0.23$ & $5.87 \pm 0.50$ & $0.27 \pm 1.62$ & $-3.5 \pm 1.6$ &  & \\
W4982 & $-0.44 \pm 0.43$ & $-0.23 \pm 0.13$ & $6.25 \pm 0.23$ & $1.34 \pm 0.91$ & $-3.2 \pm 0.9$ & $-8.6 \pm 1.6$ & CTTS\\
W5004 & $-0.35 \pm 0.40$ & $-0.46 \pm 0.11$ & $5.24 \pm 0.24$ & $-0.30 \pm 1.05$ & $-4.8 \pm 1.1$ &  & \\
W5044 & $-0.66 \pm 0.34$ & $-0.04 \pm 0.11$ & $6.27 \pm 0.21$ & $0.73 \pm 1.04$ & $-3.5 \pm 1.0$ &  & \\
W5078 & $0.20 \pm 0.34$ & $-0.15 \pm 0.14$ & $5.36 \pm 0.24$ & $1.05 \pm 1.47$ & $-2.6 \pm 1.5$ &  & \\
W5088 & $-0.68 \pm 0.38$ & $0.10 \pm 0.08$ & $6.59 \pm 0.41$ & $0.33 \pm 1.09$ & $-3.7 \pm 1.1$ &  & \\
W5091 & $-0.50 \pm 0.41$ & $-0.17 \pm 0.12$ & $6.35 \pm 0.30$ & $1.59 \pm 0.42$ & $-2.9 \pm 0.5$ & $-8.1 \pm 1.0$ & CTTS\\
W510 & $-0.36 \pm 0.46$ & $-0.46 \pm 0.08$ & $6.49 \pm 0.08$ & $1.69 \pm 0.25$ & $-3.6 \pm 0.3$ & $-9.1 \pm 0.8$ & CTTS\\
W5102 & $-0.35 \pm 0.38$ & $-0.29 \pm 0.12$ & $5.97 \pm 0.11$ & $-1.09 \pm 1.21$ & $-5.5 \pm 1.2$ &  & \\
W5237 & $-0.57 \pm 0.37$ & $-0.11 \pm 0.12$ & $6.37 \pm 0.31$ & $-0.39 \pm 1.18$ & $-4.8 \pm 1.2$ &  & \\
W5314 & $-0.58 \pm 0.41$ & $0.19 \pm 0.06$ & $6.89 \pm 0.54$ & $-0.67 \pm 1.34$ & $-4.4 \pm 1.3$ &  & \\
W5350 & $-0.32 \pm 0.43$ & $-0.37 \pm 0.15$ & $6.09 \pm 0.27$ & $-0.44 \pm 1.13$ & $-5.1 \pm 1.2$ &  & \\
W5367 & $-0.56 \pm 0.39$ & $-0.02 \pm 0.13$ & $6.60 \pm 0.44$ & $-1.33 \pm 1.28$ & $-5.6 \pm 1.2$ &  & \\
W5395 & $-0.59 \pm 0.38$ & $-0.09 \pm 0.14$ & $6.37 \pm 0.31$ & $-0.73 \pm 1.35$ & $-5.1 \pm 1.3$ &  & \\
W5396 & $-0.42 \pm 0.40$ & $-0.11 \pm 0.15$ & $6.14 \pm 0.21$ & $-2.29 \pm 0.89$ & $-6.5 \pm 0.9$ &  & \\
W5405 & $-0.50 \pm 0.40$ & $0.01 \pm 0.18$ & $5.46 \pm 0.37$ & $-1.58 \pm 1.19$ & $-5.0 \pm 1.2$ &  & \\
W5411 & $-0.49 \pm 0.36$ & $-0.00 \pm 0.12$ & $6.32 \pm 0.38$ & $-0.63 \pm 1.09$ & $-4.7 \pm 1.1$ &  & \\
W5413 & $-0.31 \pm 0.44$ & $-0.37 \pm 0.11$ & $6.04 \pm 0.14$ & $1.75 \pm 0.25$ & $-2.9 \pm 0.3$ & $-7.8 \pm 0.8$ & CTTS\\
W5427 & $-0.52 \pm 0.33$ & $-0.02 \pm 0.12$ & $6.20 \pm 0.29$ & $-0.58 \pm 1.04$ & $-4.7 \pm 1.0$ &  & \\
W5448 & $-0.56 \pm 0.37$ & $0.07 \pm 0.10$ & $6.54 \pm 0.45$ & $-0.51 \pm 1.12$ & $-4.6 \pm 1.1$ &  & \\
W5470 & $-0.56 \pm 0.35$ & $-0.11 \pm 0.11$ & $6.46 \pm 0.26$ & $-0.65 \pm 1.08$ & $-5.1 \pm 1.1$ &  & \\
W5491 & $-0.34 \pm 0.38$ & $-0.30 \pm 0.11$ & $6.09 \pm 0.10$ & $-0.59 \pm 1.17$ & $-5.1 \pm 1.2$ &  & \\
W5496 & $-0.55 \pm 0.34$ & $-0.10 \pm 0.12$ & $6.21 \pm 0.21$ & $-0.40 \pm 1.02$ & $-4.7 \pm 1.0$ &  & \\
W5503 & $-0.53 \pm 0.37$ & $-0.07 \pm 0.12$ & $6.41 \pm 0.34$ & $-0.50 \pm 1.07$ & $-4.8 \pm 1.0$ &  & \\
W5506 & $-0.13 \pm 0.48$ & $-0.18 \pm 0.20$ & $6.18 \pm 0.38$ & $1.87 \pm 0.14$ & $-2.4 \pm 0.4$ & $-7.4 \pm 0.8$ & CTTS\\
W5508 & $-0.64 \pm 0.33$ & $0.01 \pm 0.10$ & $6.43 \pm 0.30$ & $-0.31 \pm 0.97$ & $-4.5 \pm 0.9$ &  & \\
W5511 & $-0.55 \pm 0.37$ & $0.04 \pm 0.10$ & $6.50 \pm 0.41$ & $-0.39 \pm 1.06$ & $-4.5 \pm 1.0$ &  & \\
W5512 & $-0.48 \pm 0.38$ & $-0.16 \pm 0.12$ & $6.33 \pm 0.31$ & $-0.55 \pm 1.10$ & $-5.0 \pm 1.1$ &  & \\
W5533 & $-0.65 \pm 0.33$ & $0.06 \pm 0.10$ & $6.35 \pm 0.32$ & $-0.15 \pm 1.02$ & $-4.2 \pm 1.0$ &  & \\
W5537 & $-0.38 \pm 0.36$ & $-0.25 \pm 0.11$ & $6.11 \pm 0.14$ & $-0.81 \pm 1.12$ & $-5.3 \pm 1.1$ &  & \\
W5538 & $-0.57 \pm 0.35$ & $-0.05 \pm 0.11$ & $6.39 \pm 0.28$ & $-0.35 \pm 1.03$ & $-4.6 \pm 1.0$ &  & \\
W5546 & $-0.45 \pm 0.39$ & $-0.14 \pm 0.14$ & $6.12 \pm 0.30$ & $-0.65 \pm 1.12$ & $-4.9 \pm 1.1$ &  & \\
W5556 & $-0.35 \pm 0.39$ & $-0.26 \pm 0.12$ & $6.04 \pm 0.12$ & $-0.95 \pm 1.22$ & $-5.4 \pm 1.2$ &  & \\
W5560 & $-0.49 \pm 0.39$ & $-0.22 \pm 0.14$ & $5.96 \pm 0.15$ & $-0.38 \pm 1.27$ & $-4.6 \pm 1.3$ &  & \\
W5563 & $-0.56 \pm 0.43$ & $-0.26 \pm 0.18$ & $5.73 \pm 0.28$ & $-0.86 \pm 1.76$ & $-5.0 \pm 1.7$ &  & \\
W5564 & $-0.48 \pm 0.38$ & $-0.12 \pm 0.12$ & $6.41 \pm 0.32$ & $-0.52 \pm 1.04$ & $-4.9 \pm 1.0$ &  & \\
W5567 & $-0.25 \pm 0.45$ & $-0.40 \pm 0.18$ & $5.44 \pm 0.37$ & $-0.77 \pm 1.16$ & $-5.2 \pm 1.2$ &  & \\
W5582 & $-0.62 \pm 0.31$ & $0.08 \pm 0.03$ & $7.60 \pm 0.31$ & $-0.24 \pm 0.95$ & $-4.3 \pm 0.9$ &  & \\
W5594 & $-0.54 \pm 0.38$ & $-0.23 \pm 0.12$ & $6.09 \pm 0.17$ & $-0.28 \pm 1.33$ & $-4.7 \pm 1.3$ &  & \\
W5604 & $-0.54 \pm 0.41$ & $-0.16 \pm 0.13$ & $6.39 \pm 0.26$ & $0.23 \pm 1.50$ & $-4.3 \pm 1.5$ &  & \\
W5607 & $-0.50 \pm 0.35$ & $-0.10 \pm 0.13$ & $6.05 \pm 0.21$ & $-0.67 \pm 1.12$ & $-4.8 \pm 1.1$ &  & \\
W5609 & $-0.56 \pm 0.38$ & $-0.03 \pm 0.12$ & $6.38 \pm 0.38$ & $-0.46 \pm 1.18$ & $-4.6 \pm 1.2$ &  & \\
W5620 & $-0.46 \pm 0.40$ & $-0.48 \pm 0.04$ & $6.09 \pm 0.05$ & $0.25 \pm 1.05$ & $-4.7 \pm 1.1$ &  & \\
W5634 & $-0.49 \pm 0.41$ & $0.21 \pm 0.05$ & $7.05 \pm 0.50$ & $-0.83 \pm 1.32$ & $-4.5 \pm 1.3$ &  & \\
W5661 & $-0.57 \pm 0.36$ & $-0.24 \pm 0.14$ & $5.60 \pm 0.27$ & $-0.88 \pm 1.18$ & $-4.9 \pm 1.1$ &  & \\
W5680 & $-0.41 \pm 0.39$ & $-0.37 \pm 0.14$ & $5.75 \pm 0.30$ & $-0.38 \pm 1.03$ & $-4.7 \pm 1.1$ &  & \\
W5690 & $-0.40 \pm 0.39$ & $-0.45 \pm 0.09$ & $6.07 \pm 0.08$ & $-0.03 \pm 1.04$ & $-4.9 \pm 1.0$ &  & \\
W5693 & $-0.49 \pm 0.43$ & $-0.14 \pm 0.21$ & $5.69 \pm 0.46$ & $-0.90 \pm 1.21$ & $-4.7 \pm 1.2$ &  & \\
W5697 & $-0.48 \pm 0.36$ & $0.17 \pm 0.04$ & $7.45 \pm 0.32$ & $-0.81 \pm 1.21$ & $-4.5 \pm 1.2$ &  & \\
W5778 & $-0.64 \pm 0.40$ & $-0.11 \pm 0.18$ & $5.73 \pm 0.29$ & $0.95 \pm 1.23$ & $-2.9 \pm 1.2$ &  & \\
W5780 & $-0.55 \pm 0.36$ & $-0.07 \pm 0.11$ & $6.47 \pm 0.32$ & $-0.46 \pm 1.04$ & $-4.8 \pm 1.0$ &  & \\
W5801 & $-0.45 \pm 0.49$ & $-0.14 \pm 0.22$ & $5.74 \pm 0.45$ & $1.72 \pm 0.22$ & $-2.2 \pm 0.3$ & $-6.8 \pm 0.8$ & CTTS\\
W5812 & $-0.52 \pm 0.36$ & $-0.12 \pm 0.12$ & $6.28 \pm 0.28$ & $-0.49 \pm 1.07$ & $-4.8 \pm 1.0$ &  & \\
W5858 & $-0.55 \pm 0.42$ & $0.14 \pm 0.10$ & $6.62 \pm 0.55$ & $-0.47 \pm 1.20$ & $-4.3 \pm 1.1$ &  & \\
W5870 & $-0.46 \pm 0.36$ & $0.19 \pm 0.04$ & $7.42 \pm 0.35$ & $-0.62 \pm 1.17$ & $-4.2 \pm 1.1$ &  & \\
W5871 & $-0.57 \pm 0.38$ & $-0.05 \pm 0.18$ & $5.74 \pm 0.36$ & $-0.52 \pm 1.10$ & $-4.2 \pm 1.1$ &  & \\
W5893 & $-0.43 \pm 0.39$ & $-0.15 \pm 0.17$ & $5.51 \pm 0.34$ & $-2.02 \pm 1.04$ & $-5.8 \pm 1.0$ &  & \\
W5895 & $-0.55 \pm 0.39$ & $-0.02 \pm 0.11$ & $6.45 \pm 0.35$ & $2.05 \pm 0.11$ & $-2.2 \pm 0.2$ & $-7.2 \pm 0.7$ & CTTS\\
W5909 & $-0.41 \pm 0.43$ & $-0.23 \pm 0.14$ & $6.16 \pm 0.25$ & $1.49 \pm 0.64$ & $-2.9 \pm 0.7$ & $-8.1 \pm 1.2$ & CTTS\\
W5936 & $-0.53 \pm 0.38$ & $-0.03 \pm 0.12$ & $6.31 \pm 0.30$ & $1.94 \pm 0.12$ & $-2.2 \pm 0.2$ & $-7.2 \pm 0.7$ & CTTS\\
W5962 & $-0.50 \pm 0.38$ & $0.14 \pm 0.05$ & $7.26 \pm 0.45$ & $-0.56 \pm 1.20$ & $-4.4 \pm 1.2$ &  & \\
W5970 & $-0.51 \pm 0.35$ & $-0.05 \pm 0.14$ & $6.00 \pm 0.22$ & $-0.63 \pm 1.07$ & $-4.6 \pm 1.0$ &  & \\
W5988 & $-0.60 \pm 0.34$ & $0.01 \pm 0.10$ & $6.51 \pm 0.34$ & $-0.38 \pm 1.00$ & $-4.6 \pm 1.0$ &  & \\
W6027 & $-0.55 \pm 0.37$ & $-0.03 \pm 0.10$ & $6.59 \pm 0.35$ & $-0.45 \pm 1.02$ & $-4.8 \pm 1.0$ &  & \\
W6035 & $-0.56 \pm 0.35$ & $-0.07 \pm 0.10$ & $6.61 \pm 0.30$ & $-0.42 \pm 1.01$ & $-4.9 \pm 1.0$ &  & \\
W6188 & $-0.62 \pm 0.35$ & $0.09 \pm 0.09$ & $6.55 \pm 0.42$ & $-0.38 \pm 1.05$ & $-4.4 \pm 1.0$ &  & \\
W6235 & $-0.68 \pm 0.34$ & $0.09 \pm 0.11$ & $6.34 \pm 0.35$ & $-0.22 \pm 0.99$ & $-4.2 \pm 1.0$ &  & \\
W6300 & $-0.59 \pm 0.35$ & $0.00 \pm 0.14$ & $5.89 \pm 0.25$ & $1.77 \pm 0.19$ & $-2.0 \pm 0.2$ & $-6.7 \pm 0.8$ & CTTS\\
W6310 & $-0.54 \pm 0.38$ & $0.00 \pm 0.12$ & $6.31 \pm 0.35$ & $-0.46 \pm 1.09$ & $-4.5 \pm 1.1$ &  & \\
W6501 & $-0.56 \pm 0.36$ & $0.00 \pm 0.04$ & $7.34 \pm 0.37$ & $-0.39 \pm 1.06$ & $-4.9 \pm 1.0$ &  & \\
W6534 & $-0.64 \pm 0.37$ & $0.04 \pm 0.09$ & $6.50 \pm 0.37$ & $1.48 \pm 0.51$ & $-2.7 \pm 0.5$ & $-8.0 \pm 1.1$ & CTTS\\
W6565 & $-0.52 \pm 0.44$ & $-0.04 \pm 0.20$ & $5.79 \pm 0.40$ & $1.82 \pm 0.22$ & $-1.9 \pm 0.3$ & $-6.4 \pm 0.8$ & CTTS\\
W662 & $-0.44 \pm 0.41$ & $-0.57 \pm 0.07$ & $6.38 \pm 0.06$ & $0.30 \pm 1.08$ & $-5.2 \pm 1.1$ &  & \\
W6647 & $-0.47 \pm 0.40$ & $-0.09 \pm 0.15$ & $6.23 \pm 0.34$ & $-0.52 \pm 1.10$ & $-4.7 \pm 1.1$ &  & \\
W6697 & $-0.72 \pm 0.33$ & $0.07 \pm 0.10$ & $6.25 \pm 0.28$ & $0.24 \pm 1.03$ & $-3.7 \pm 1.0$ &  & \\
W6858 & $-0.50 \pm 0.36$ & $-0.03 \pm 0.14$ & $6.09 \pm 0.27$ & $-0.47 \pm 1.03$ & $-4.5 \pm 1.0$ &  & \\
W6871 & $-0.62 \pm 0.41$ & $0.26 \pm 0.06$ & $6.62 \pm 0.44$ & $-0.22 \pm 1.07$ & $-3.8 \pm 1.0$ &  & \\
W6920 & $-0.54 \pm 0.39$ & $-0.20 \pm 0.12$ & $6.30 \pm 0.20$ & $0.80 \pm 1.12$ & $-3.7 \pm 1.1$ &  & \\
W7105 & $-0.53 \pm 0.37$ & $-0.10 \pm 0.12$ & $6.43 \pm 0.31$ & $-0.61 \pm 1.14$ & $-5.0 \pm 1.1$ &  & \\
W8957 & $-0.68 \pm 0.34$ & $0.05 \pm 0.12$ & $6.01 \pm 0.22$ & $0.40 \pm 1.25$ & $-3.4 \pm 1.2$ &  & \\


==> tables/table_photometry.tex <==
C11059 & J063955.90+094239.8 &  19.41$\pm$0.03 & 18.14$\pm$0.03 & 17.56$\pm$0.02  & 15.44$\pm$0.06 & 14.69$\pm$0.05 & 14.28$\pm$0.08 \\
C11997 & J063957.95+094104.7 &  17.91$\pm$0.01 & 16.50$\pm$0.01 & 16.16$\pm$0.01  & 14.36$\pm$0.04 & 13.65$\pm$0.03 & 13.35$\pm$0.04 \\
C12135 & J063958.30+092848.6 &  18.51$\pm$0.01 & 17.66$\pm$0.02 & 16.74$\pm$0.01  & 14.99$\pm$0.04 & 14.34$\pm$0.05 & 14.11$\pm$0.07 \\
C12598 & J063959.23+100607.7 &  17.26$\pm$0.00 & 16.18$\pm$0.01 & 16.07$\pm$0.00  & 13.91$\pm$0.02 & 12.80$\pm$0.03 & 12.10$\pm$0.02 \\
C13507 & J064001.30+094300.5 &  19.10$\pm$0.04 & 16.91$\pm$0.01 & 18.14$\pm$0.04  & 15.00$\pm$0.04 & 13.17$\pm$0.02 & 11.94$\pm$0.03 \\
C14005 & J064002.67+093524.3 &  16.86$\pm$0.00 & 15.87$\pm$0.00 & 15.35$\pm$0.00  & 13.70$\pm$0.03 & 12.99$\pm$0.03 & 12.71$\pm$0.03 \\
C15152 & J064005.22+095056.6 &  16.27$\pm$0.00 & 15.50$\pm$0.00 & 14.87$\pm$0.00  & 13.19$\pm$0.02 & 12.48$\pm$0.02 & 12.26$\pm$0.02 \\
C15247 & J064005.53+092226.1 &  16.54$\pm$0.00 & 15.65$\pm$0.00 & 15.44$\pm$0.00  & 13.95$\pm$0.03 & 13.12$\pm$0.02 & 12.73$\pm$0.03 \\
C15285 & J064005.53+094554.8 &  18.54$\pm$0.02 & 18.14$\pm$0.04 & 17.16$\pm$0.02  & 15.14$\pm$0.05 & 14.28$\pm$0.04 & 13.93$\pm$0.05 \\
C15519 & J064006.00+094942.7 &  16.44$\pm$0.00 & 15.62$\pm$0.00 & 15.18$\pm$0.00  & 13.46$\pm$0.03 & 12.76$\pm$0.03 & 12.45$\pm$0.03 \\
C16567 & J064008.39+094647.6 &  18.36$\pm$0.01 & 17.85$\pm$0.02 & 17.00$\pm$0.01  & 14.79$\pm$0.06 & 13.93$\pm$0.05 & 13.60$\pm$0.05 \\
C16928 & J064009.31+095002.8 &  19.39$\pm$0.03 & 18.89$\pm$0.05 & 17.81$\pm$0.02  & 15.37$\pm$0.06 & 14.41$\pm$0.04 & 14.01$\pm$0.06 \\
C17553 & J064010.88+094007.3 &  17.72$\pm$0.01 & 16.92$\pm$0.01 & 16.11$\pm$0.01  & 14.33$\pm$0.03 & 13.63$\pm$0.04 & 13.43$\pm$0.04 \\
C17614 & J064011.11+092127.1 &  17.45$\pm$0.00 & 16.02$\pm$0.00 & 16.11$\pm$0.01  & 14.48$\pm$0.03 & 13.77$\pm$0.03 & 13.51$\pm$0.04 \\
C18487 & J064013.38+100549.4 &  17.96$\pm$0.02 & 16.63$\pm$0.02 & 16.35$\pm$0.02  & 14.41$\pm$0.04 & 13.56$\pm$0.02 & 13.22$\pm$0.04 \\
C18627 & J064013.70+095630.6 &  15.95$\pm$0.00 & 14.58$\pm$0.00 & 14.73$\pm$0.00  & 12.92$\pm$0.03 & 12.13$\pm$0.02 & 11.58$\pm$0.02 \\
C18688 & J064013.93+092439.2 &  18.23$\pm$0.01 & 17.31$\pm$0.02 & 16.55$\pm$0.01  & 14.89$\pm$0.05 & 14.32$\pm$0.05 & 14.10$\pm$0.06 \\
C19191 & J064015.15+100157.9 &  17.03$\pm$0.00 & 16.29$\pm$0.01 & 15.98$\pm$0.01  & 14.55$\pm$0.04 & 13.25$\pm$0.03 & 12.35$\pm$0.03 \\
C19299 & J064015.45+094300.5 &  17.62$\pm$0.01 & 17.29$\pm$0.01 & 16.48$\pm$0.01  & 14.82$\pm$0.04 & 14.36$\pm$0.05 & 14.02$\pm$0.06 \\
C19556 & J064016.10+095407.2 &  19.73$\pm$0.04 & 18.09$\pm$0.03 & 17.48$\pm$0.02  & 14.93$\pm$0.05 & 14.09$\pm$0.03 & 13.46$\pm$0.05 \\
C19649 & J064016.31+101843.7 &  17.37$\pm$0.00 & 16.32$\pm$0.01 & 15.79$\pm$0.00  & 14.06$\pm$0.06 & 13.29$\pm$0.05 & 12.90$\pm$0.04 \\
C19751 & J064016.69+094022.6 &  18.40$\pm$0.02 & 16.06$\pm$0.01 & 17.09$\pm$0.02  & 15.21$\pm$0.07 & 14.64$\pm$0.06 & 14.36$\pm$0.09 \\
C19877 & J064016.99+094633.2 &  15.75$\pm$0.00 & 15.20$\pm$0.00 & 14.70$\pm$0.00  & 13.27$\pm$0.03 & 12.56$\pm$0.03 & 12.40$\pm$0.03 \\
C20156 & J064017.80+092547.8 &  17.96$\pm$0.01 & 16.30$\pm$0.01 & 16.74$\pm$0.01  & 14.95$\pm$0.05 & 14.13$\pm$0.04 & 13.63$\pm$0.05 \\
C20254 & J064018.02+095022.1 &  17.47$\pm$0.01 & 16.54$\pm$0.01 & 15.78$\pm$0.01  & 14.03$\pm$0.03 & 13.33$\pm$0.03 & 13.04$\pm$0.03 \\
C20428 & J064018.46+095206.1 &  18.42$\pm$0.01 & 17.51$\pm$0.02 & 16.50$\pm$0.01  & 14.55$\pm$0.04 & 13.89$\pm$0.04 & 13.65$\pm$0.05 \\
C20504 & J064018.69+093700.8 &  18.47$\pm$0.02 & 17.18$\pm$0.02 & 16.62$\pm$0.01  & 13.74$\pm$0.02 & 12.34$\pm$0.03 & 11.51$\pm$0.02 \\
C20506 & J064018.65+100024.8 &  17.54$\pm$0.01 & 16.21$\pm$0.01 & 16.07$\pm$0.01  & 14.43$\pm$0.04 & 13.39$\pm$0.02 & 12.71$\pm$0.03 \\
C20522 & J064018.68+095242.1 &  17.86$\pm$0.01 & 17.44$\pm$0.02 & 16.34$\pm$0.01  & 14.04$\pm$0.03 & 13.24$\pm$0.03 & 12.89$\pm$0.03 \\
C20623 & J064018.94+093814.9 &  19.06$\pm$0.02 & 17.91$\pm$0.02 & 16.82$\pm$0.01  & 14.62$\pm$0.05 & 13.94$\pm$0.04 & 13.70$\pm$0.06 \\
C20696 & J064019.17+093935.1 &  18.78$\pm$0.03 & 17.04$\pm$0.02 & 17.05$\pm$0.02  & 14.96$\pm$0.05 & 14.20$\pm$0.05 & 13.87$\pm$0.06 \\
C20824 & J064019.50+095018.6 &  18.56$\pm$0.02 & 17.40$\pm$0.02 & 16.68$\pm$0.01  & 14.82$\pm$0.05 & 14.22$\pm$0.05 & 13.89$\pm$0.05 \\
C20830 & J064019.55+092746.8 &  20.18$\pm$0.05 & 18.41$\pm$0.03 & 18.12$\pm$0.03  & 15.97$\pm$0.12 & 15.36$\pm$0.09 & 15.00$\pm$0.14 \\
C20939 & J064019.84+101148.5 &  16.94$\pm$0.01 & 16.58$\pm$0.03 & 16.20$\pm$0.02  & 14.81$\pm$0.05 & 14.40$\pm$0.05 & 14.18$\pm$0.08 \\
C21090 & J064020.27+095606.4 &  15.74$\pm$0.00 & 14.65$\pm$0.00 & 14.22$\pm$0.00  & 12.30$\pm$0.03 & 11.52$\pm$0.03 & 11.21$\pm$0.02 \\
C21202 & J064020.64+094050.0 &  18.03$\pm$0.01 & 16.93$\pm$0.01 & 15.81$\pm$0.00  & 13.50$\pm$0.02 & 12.78$\pm$0.02 & 12.41$\pm$0.02 \\
C21501 & J064021.51+090603.1 &  16.62$\pm$0.00 & 15.57$\pm$0.00 & 15.38$\pm$0.00  & 13.57$\pm$0.04 & 12.62$\pm$0.03 & 12.05$\pm$0.03 \\
C21607 & J064021.66+094822.5 &  18.98$\pm$0.02 & 17.57$\pm$0.02 & 17.22$\pm$0.01  & 15.05$\pm$0.06 & 13.97$\pm$0.04 & 13.49$\pm$0.04 \\
C21959 & J064022.62+094946.3 &  16.52$\pm$0.00 & 15.91$\pm$0.00 & 15.39$\pm$0.00  & 13.88$\pm$0.03 & 13.12$\pm$0.03 & 12.87$\pm$0.03 \\
C22078 & J064022.95+095312.6 &  19.50$\pm$0.03 & 18.71$\pm$0.05 & 17.42$\pm$0.01  & 15.49$\pm$0.06 & 14.78$\pm$0.06 & 14.34$\pm$0.09 \\
C22226 & J064023.42+095455.6 &  17.82$\pm$0.01 & 16.80$\pm$0.01 & 15.97$\pm$0.01  & 14.01$\pm$0.04 & 13.35$\pm$0.04 & 12.97$\pm$0.04 \\
C22323 & J064023.66+095500.6 &  19.24$\pm$0.02 & 18.09$\pm$0.03 & 16.96$\pm$0.01  & 14.68$\pm$0.04 & 14.04$\pm$0.04 & 13.60$\pm$0.05 \\
C22348 & J064023.73+095523.9 &  16.71$\pm$0.00 & 15.43$\pm$0.00 & 15.21$\pm$0.00  & 13.12$\pm$0.03 & 12.26$\pm$0.02 & 11.81$\pm$0.02 \\
C22501 & J064024.16+093412.5 &  17.09$\pm$0.01 & 15.96$\pm$0.01 & 16.02$\pm$0.01  & 13.47$\pm$0.02 & 12.52$\pm$0.03 & 11.84$\pm$0.02 \\
C22751 & J064024.84+095311.5 &  16.80$\pm$0.00 & 16.08$\pm$0.01 & 15.40$\pm$0.00  & 13.59$\pm$0.06 & 12.81:       & 12.52$\pm$0.06 \\
C22982 & J064025.47+094826.0 &  15.17$\pm$0.00 & 14.71$\pm$0.00 & 14.38$\pm$0.00  & 13.24$\pm$0.04 & 12.61$\pm$0.04 & 12.45$\pm$0.04 \\
C23000 & J064025.51+094709.3 &  19.01$\pm$0.02 & 18.02$\pm$0.03 & 16.61$\pm$0.01  & 14.38$\pm$0.04 & 13.82$\pm$0.03 & 13.50$\pm$0.05 \\
C23061 & J064025.65+095959.8 &  17.14$\pm$0.01 & 15.56$\pm$0.01 & 15.95$\pm$0.02  & 13.93$\pm$0.03 & 13.13$\pm$0.03 & 12.65$\pm$0.03 \\
C23131 & J064025.87+095057.6 &  16.66$\pm$0.00 & 15.29$\pm$0.00 & 15.77$\pm$0.00  & 13.85$\pm$0.03 & 13.07$\pm$0.02 & 12.60$\pm$0.02 \\
C23215 & J064026.16+093709.3 &  17.55$\pm$0.01 & 16.68$\pm$0.01 & 15.95$\pm$0.01  & 14.23$\pm$0.04 & 13.52$\pm$0.03 & 13.30$\pm$0.05 \\
C23314 & J064026.39+095659.0 &  19.63$\pm$0.06 & 17.96$\pm$0.04 & 17.26$\pm$0.02  & 14.52$\pm$0.03 & 13.89$\pm$0.04 & 13.50$\pm$0.05 \\
C23474 & J064026.86+094412.6 &  18.93$\pm$0.02 & 17.85$\pm$0.02 & 16.70$\pm$0.01  & 14.66$\pm$0.04 & 13.97$\pm$0.04 & 13.62$\pm$0.05 \\
C23553 & J064027.12+094736.2 &  20.23$\pm$0.07 & 19.41$\pm$0.10 & 17.67$\pm$0.02  & 15.37$\pm$0.06 & 14.78$\pm$0.05 & 14.40$\pm$0.09 \\
C23686 & J064027.44+095230.4 &  18.17$\pm$0.01 & 17.24$\pm$0.01 & 16.23$\pm$0.01  & 14.32$\pm$0.03 & 13.63$\pm$0.02 & 13.36$\pm$0.04 \\
C23781 & J064027.72+093159.7 &  17.30$\pm$0.01 & 16.52$\pm$0.01 & 15.90$\pm$0.00  & 14.27$\pm$0.03 & 13.54$\pm$0.03 & 13.29$\pm$0.04 \\
C23909 & J064028.08+093533.8 &  17.57$\pm$0.01 & 16.72$\pm$0.01 & 16.05$\pm$0.01  & 14.44$\pm$0.04 & 13.70$\pm$0.03 & 13.50$\pm$0.05 \\
C24113 & J064028.58+093547.6 &  15.43$\pm$0.00 & 14.84$\pm$0.00 & 14.31$\pm$0.00  & 12.79$\pm$0.02 & 12.07$\pm$0.03 & 11.85$\pm$0.03 \\
C24217 & J064028.86+093305.6 &  16.88$\pm$0.00 & 16.06$\pm$0.01 & 15.38$\pm$0.00  & 13.66$\pm$0.02 & 12.97$\pm$0.03 & 12.78$\pm$0.02 \\
C24250 & J064028.95+094217.1 &  14.96$\pm$0.00 & 14.49$\pm$0.00 & 14.13$\pm$0.00  & 12.91$\pm$0.03 & 12.21$\pm$0.02 & 12.02$\pm$0.02 \\
C24349 & J064029.25+094407.5 &  17.01$\pm$0.00 & 16.02$\pm$0.01 & 15.66$\pm$0.00  & 14.06$\pm$0.03 & 13.34$\pm$0.03 & 13.06$\pm$0.03 \\
C24362 & J064029.22+101000.1 &  20.03$\pm$0.05 & 18.70$\pm$0.05 & 18.27$\pm$0.04  & 16.12$\pm$0.10 & 15.44$\pm$0.11 & 15.04$\pm$0.15 \\
C24373 & J064029.29+100544.2 &  18.49$\pm$0.04 & 17.60$\pm$0.07 & 16.60$\pm$0.03  & 14.40$\pm$0.03 & 13.87$\pm$0.03 & 13.53$\pm$0.04 \\
C24554 & J064029.77+094221.3 &  16.21$\pm$0.00 & 15.29$\pm$0.00 & 15.25$\pm$0.00  & 13.72$\pm$0.03 & 12.81$\pm$0.02 & 12.13$\pm$0.02 \\
C24602 & J064029.89+095010.4 &  13.83$\pm$0.00 & 13.45$\pm$0.00 & 13.21$\pm$0.00  & 12.22$\pm$0.03 & 11.68$\pm$0.03 & 11.56$\pm$0.03 \\
C24893 & J064030.77+094807.6 &  17.48$\pm$0.01 & 16.75$\pm$0.01 & 16.27$\pm$0.01  & 14.71$\pm$0.04 & 14.06$\pm$0.04 & 13.66$\pm$0.05 \\
C24924 & J064030.85+093440.5 &  14.12$\pm$0.00 & 13.40$\pm$0.00 & 13.39$\pm$0.00  & 12.69$\pm$0.02 & 11.51$\pm$0.02 & 10.67$\pm$0.02 \\
C24984 & J064030.98+100625.5 &  18.31$\pm$0.02 & 17.09$\pm$0.02 & 16.35$\pm$0.01  & 14.46$\pm$0.04 & 13.75$\pm$0.04 & 13.47$\pm$0.04 \\
C25214 & J064031.67+094959.4 &  20.09$\pm$0.05 & 19.27$\pm$0.07 & 17.76$\pm$0.02  & 15.57$\pm$0.06 & 14.90$\pm$0.06 & 14.61$\pm$0.10 \\
C25248 & J064031.80+093329.4 &  19.35$\pm$0.05 & 18.37$\pm$0.05 & 17.33$\pm$0.02  & 15.42$\pm$0.05 & 14.85$\pm$0.05 & 14.60$\pm$0.10 \\
C25302 & J064031.89+100708.3 &  18.69$\pm$0.03 & 17.36$\pm$0.03 & 16.95$\pm$0.03  & 15.06$\pm$0.04 & 14.42$\pm$0.04 & 14.08$\pm$0.06 \\
C25335 & J064032.01+094935.5 &  16.39$\pm$0.00 & 14.50$\pm$0.00 & 15.32$\pm$0.01  & 13.76$\pm$0.03 & 13.01$\pm$0.03 & 12.57$\pm$0.02 \\
C25404 & J064032.19+095722.1 &  18.85$\pm$0.02 & 17.45$\pm$0.01 & 16.82$\pm$0.01  & 14.75$\pm$0.04 & 14.03$\pm$0.04 & 13.76$\pm$0.05 \\
C25550 & J064032.58+094933.2 &  19.29$\pm$0.03 & 18.25$\pm$0.03 & 17.07$\pm$0.01  & 14.94$\pm$0.04 & 14.28$\pm$0.03 & 14.05$\pm$0.06 \\
C25738 & J064033.12+094954.8 &  19.14$\pm$0.04 & 17.93$\pm$0.04 & 17.29$\pm$0.02  & 14.36$\pm$0.04 & 12.98$\pm$0.03 & 12.16$\pm$0.02 \\
C25835 & J064033.33+100427.2 &  19.91$\pm$0.04 & 18.95$\pm$0.07 & 17.84$\pm$0.03  & 15.38$\pm$0.05 & 14.60$\pm$0.05 & 14.14$\pm$0.06 \\
C25875 & J064033.45+095702.7 &  18.57$\pm$0.01 & 17.67$\pm$0.02 & 16.62$\pm$0.01  & 14.69$\pm$0.04 & 14.08$\pm$0.04 & 13.81$\pm$0.05 \\
C25891 & J064033.50+093458.6 &  17.56$\pm$0.01 & 16.76$\pm$0.01 & 16.11$\pm$0.01  & 14.51$\pm$0.03 & 13.79$\pm$0.03 & 13.57$\pm$0.04 \\
C25927 & J064033.56+093336.4 &  17.92$\pm$0.01 & 17.03$\pm$0.01 & 16.23$\pm$0.01  & 14.41$\pm$0.03 & 13.73$\pm$0.03 & 13.47$\pm$0.04 \\
C26021 & J064033.78+094843.8 &  16.44$\pm$0.00 & 15.65$\pm$0.00 & 15.00$\pm$0.00  & 13.45$\pm$0.03 & 12.72$\pm$0.02 & 12.35$\pm$0.02 \\
C26103 & J064034.01+094829.2 &  18.91$\pm$0.02 & 17.45$\pm$0.02 & 17.12$\pm$0.01  & 14.71$\pm$0.04 & 13.77$\pm$0.03 & 13.19$\pm$0.03 \\
C26120 & J064034.01+100720.1 &  18.25$\pm$0.01 & 16.26$\pm$0.01 & 17.13$\pm$0.01  & 15.31$\pm$0.05 & 14.53$\pm$0.04 & 14.11$\pm$0.08 \\
C26166 & J064034.18+094352.6 &  18.60$\pm$0.02 & 17.78$\pm$0.02 & 16.68$\pm$0.01  & 14.81$\pm$0.03 & 14.10$\pm$0.04 & 13.76$\pm$0.05 \\
C26216 & J064034.30+095622.9 &  19.65$\pm$0.03 & 18.34$\pm$0.03 & 17.46$\pm$0.01  & 15.20$\pm$0.04 & 14.78$\pm$0.06 & 14.19$\pm$0.07 \\
C26264 & J064034.46+093518.3 &  16.57$\pm$0.00 & 15.77$\pm$0.00 & 15.16$\pm$0.00  & 13.55$\pm$0.02 & 12.82$\pm$0.02 & 12.53$\pm$0.03 \\
C26400 & J064034.89+095407.2 &  17.48$\pm$0.01 & 16.57$\pm$0.01 & 15.61$\pm$0.00  & 13.74$\pm$0.03 & 13.05$\pm$0.02 & 12.81$\pm$0.03 \\
C26829 & J064036.08+094736.2 &  18.76$\pm$0.02 & 17.76$\pm$0.02 & 16.54$\pm$0.01  & 14.46$\pm$0.05 & 13.88$\pm$0.04 & 13.67$\pm$0.06 \\
C26854 & J064036.22+092804.2 &  18.42$\pm$0.01 & 17.34$\pm$0.01 & 16.41$\pm$0.01  & 14.51$\pm$0.03 & 13.98$\pm$0.03 & 13.67$\pm$0.05 \\
C26862 & J064036.22+094001.6 &  18.36$\pm$0.01 & 17.46$\pm$0.02 & 16.52$\pm$0.01  & 14.57$\pm$0.03 & 13.91$\pm$0.03 & 13.64$\pm$0.04 \\
C26966 & J064036.52+095045.6 &  15.87$\pm$0.00 & 14.90$\pm$0.00 & 14.59$\pm$0.00  & 12.93$\pm$0.03 & 12.14$\pm$0.03 & 11.71$\pm$0.03 \\
C26999 & J064036.63+094823.0 &  15.10$\pm$0.00 & 14.62$\pm$0.00 & 14.26$\pm$0.00  & 13.04$\pm$0.02 & 12.33$\pm$0.02 & 12.21$\pm$0.03 \\
C27205 & J064037.20+093109.9 &  16.39$\pm$0.00 & 15.65$\pm$0.00 & 14.93$\pm$0.00  & 13.33$\pm$0.03 & 12.55$\pm$0.02 & 12.33$\pm$0.03 \\
C27213 & J064037.21+095310.3 &  17.85$\pm$0.01 & 16.47$\pm$0.01 & 16.20$\pm$0.01  & 14.06$\pm$0.03 & 13.02$\pm$0.03 & 12.39$\pm$0.03 \\
C27301 & J064037.45+095521.3 &  15.70$\pm$0.00 & 15.20$\pm$0.00 & 14.81$\pm$0.00  & 13.53$\pm$0.03 & 12.81$\pm$0.02 & 12.65$\pm$0.03 \\
C27379 & J064037.68+093939.8 &  16.29$\pm$0.00 & 15.75$\pm$0.00 & 15.30$\pm$0.00  & 14.00$\pm$0.03 & 13.27$\pm$0.03 & 13.14$\pm$0.03 \\
C27435 & J064037.86+093454.1 &  15.97$\pm$0.00 & 15.15$\pm$0.00 & 14.67$\pm$0.00  & 12.91$\pm$0.02 & 12.19$\pm$0.03 & 11.83$\pm$0.02 \\
C27436 & J064037.85+094950.9 &  16.48$\pm$0.00 & 15.75$\pm$0.00 & 15.02$\pm$0.00  & 13.43$\pm$0.03 & 12.66$\pm$0.03 & 12.45$\pm$0.02 \\
C27558 & J064038.19+092952.5 &  16.66$\pm$0.00 & 15.95$\pm$0.01 & 15.42$\pm$0.00  & 13.93$\pm$0.03 & 13.19$\pm$0.03 & 12.89$\pm$0.03 \\
C27854 & J064039.02+093600.0 &  15.78$\pm$0.00 & 15.23$\pm$0.00 & 14.75$\pm$0.00  & 13.30$\pm$0.02 & 12.56$\pm$0.02 & 12.40$\pm$0.02 \\
C27963 & J064039.34+093445.6 &  16.43$\pm$0.00 & 15.32$\pm$0.00 & 15.29$\pm$0.00  & 12.65$\pm$0.02 & 11.14$\pm$0.03 & 9.95$\pm$0.02 \\
C28298 & J064040.43+093134.8 &  19.57$\pm$0.04 & 18.68$\pm$0.05 & 17.57$\pm$0.02  & 15.61$\pm$0.06 & 15.02$\pm$0.08 & 14.75$\pm$0.12 \\
C28305 & J064040.44+095102.6 &  16.68$\pm$0.01 & 16.05$\pm$0.01 & 15.50$\pm$0.01  & 14.02$\pm$0.03 & 13.33$\pm$0.04 & 13.07$\pm$0.04 \\
C28324 & J064040.53+092919.7 &  18.70$\pm$0.03 & 17.74$\pm$0.03 & 16.83$\pm$0.01  & 15.03$\pm$0.04 & 14.29$\pm$0.05 & 13.96$\pm$0.07 \\
C28457 & J064040.92+092759.5 &  17.25$\pm$0.00 & 16.39$\pm$0.01 & 15.53$\pm$0.00  & 13.74$\pm$0.03 & 13.05$\pm$0.03 & 12.87$\pm$0.03 \\
C28505 & J064041.03+094757.7 &  15.40$\pm$0.00 & 14.86$\pm$0.00 & 14.47$\pm$0.00  & 13.14$\pm$0.03 & 12.43$\pm$0.03 & 12.17$\pm$0.02 \\
C28541 & J064041.14+093357.9 &  16.36$\pm$0.00 & 14.44$\pm$0.00 & 15.47$\pm$0.00  & 13.12$\pm$0.02 & 12.25$\pm$0.02 & 11.45$\pm$0.02 \\
C28544 & J064041.14+095256.5 &  15.03$\pm$0.00 & 14.32$\pm$0.00 & 14.15$\pm$0.00  & 12.53$\pm$0.03 & 11.77$\pm$0.02 & 11.25$\pm$0.02 \\
C28772 & J064041.79+094952.3 &  15.77$\pm$0.00 & 15.18$\pm$0.00 & 14.74$\pm$0.00  & 13.17$\pm$0.03 & 12.52$\pm$0.03 & 12.33$\pm$0.03 \\
C28790 & J064041.85+094138.6 &  17.79$\pm$0.01 & 16.94$\pm$0.01 & 16.09$\pm$0.01  & 14.35$\pm$0.03 & 13.66$\pm$0.03 & 13.46$\pm$0.05 \\
C28907 & J064042.21+094011.1 &  15.00$\pm$0.00 & 14.10$\pm$0.00 & 14.18$\pm$0.00  & 12.86$\pm$0.03 & 12.14$\pm$0.03 & 11.80$\pm$0.03 \\
C28949 & J064042.32+093425.1 &  17.56$\pm$0.01 & 16.78$\pm$0.01 & 15.94$\pm$0.01  & 14.27$\pm$0.04 & 13.48$\pm$0.03 & 13.35$\pm$0.04 \\
C28983 & J064042.44+093220.6 &  14.97$\pm$0.00 & 14.57$\pm$0.00 & 14.27$\pm$0.00  & 13.23$\pm$0.03 & 12.64$\pm$0.03 & 12.52$\pm$0.03 \\
C28991 & J064042.46+095517.3 &  18.04$\pm$0.01 & 17.25$\pm$0.02 & 16.42$\pm$0.01  & 14.81$\pm$0.05 & 14.09$\pm$0.04 & 13.94$\pm$0.07 \\
C29037 & J064042.62+095347.7 &  15.53$\pm$0.00 & 15.04$\pm$0.00 & 14.68$\pm$0.00  & 13.51$\pm$0.03 & 12.83$\pm$0.03 & 12.69$\pm$0.04 \\
C29082 & J064042.78+093335.1 &  16.10$\pm$0.00 & 15.52$\pm$0.00 & 15.04$\pm$0.00  & 13.87$\pm$0.03 & 13.00$\pm$0.03 & 12.67$\pm$0.03 \\
C29089 & J064042.81+093036.5 &  17.67$\pm$0.01 & 16.78$\pm$0.01 & 16.18$\pm$0.01  & 14.68$\pm$0.04 & 13.99$\pm$0.04 & 13.69$\pm$0.04 \\
C29297 & J064043.40+093034.2 &  17.02$\pm$0.00 & 16.17$\pm$0.01 & 15.77$\pm$0.00  & 13.97$\pm$0.03 & 13.11$\pm$0.03 & 12.39$\pm$0.03 \\
C29357 & J064043.59+093720.6 &  19.08$\pm$0.02 & 17.99$\pm$0.03 & 16.84$\pm$0.01  & 14.65$\pm$0.04 & 14.03$\pm$0.04 & 13.80$\pm$0.05 \\
C29385 & J064043.66+093835.7 &  17.98$\pm$0.01 & 17.14$\pm$0.01 & 16.29$\pm$0.01  & 14.57$\pm$0.04 & 13.94$\pm$0.03 & 13.71$\pm$0.06 \\
C29465 & J064043.85+094755.9 &  18.31$\pm$0.01 & 17.50$\pm$0.02 & 16.58$\pm$0.01  & 14.78$\pm$0.04 & 14.17$\pm$0.04 & 13.93$\pm$0.06 \\
C29467 & J064043.86+094830.6 &  16.36$\pm$0.00 & 15.71$\pm$0.00 & 15.13$\pm$0.00  & 13.53$\pm$0.03 & 12.85$\pm$0.03 & 12.66$\pm$0.03 \\
C29493 & J064043.93+095516.9 &  19.34$\pm$0.04 & 18.66$\pm$0.06 & 17.35$\pm$0.02  & 14.25$\pm$0.04 & 12.94$\pm$0.03 & 12.47$\pm$0.04 \\
C29547 & J064044.13+094957.6 &  17.65$\pm$0.01 & 17.11$\pm$0.02 & 15.96$\pm$0.01  & 13.13$\pm$0.03 & 12.07$\pm$0.03 & 11.56$\pm$0.03 \\
C29591 & J064044.24+095339.4 &  17.63$\pm$0.01 & 16.72$\pm$0.01 & 15.73$\pm$0.00  & 13.79$\pm$0.03 & 13.10$\pm$0.04 & 12.85$\pm$0.04 \\
C29702 & J064044.59+093226.2 &  17.34$\pm$0.01 & 16.02$\pm$0.01 & 15.81$\pm$0.00  & 14.05$\pm$0.04 & 13.34$\pm$0.03 & 12.98$\pm$0.04 \\
C29785 & J064044.80+094947.8 &  17.13$\pm$0.01 & 16.34$\pm$0.01 & 15.82$\pm$0.00  & 14.28$\pm$0.03 & 13.62$\pm$0.03 & 13.41$\pm$0.05 \\
C29815 & J064044.93+094909.2 &  17.31$\pm$0.01 & 16.58$\pm$0.01 & 15.94$\pm$0.01  & 14.43$\pm$0.04 & 13.81$\pm$0.04 & 13.55$\pm$0.05 \\
C29851 & J064045.04+094541.9 &  15.58$\pm$0.00 & 15.05$\pm$0.00 & 14.58$\pm$0.00  & 13.11$\pm$0.02 & 12.40$\pm$0.02 & 12.24$\pm$0.04 \\
C29865 & J064045.06+095127.6 &  17.01$\pm$0.00 & 16.29$\pm$0.01 & 15.69$\pm$0.00  & 14.15$\pm$0.04 & 13.50$\pm$0.05 & 13.23$\pm$0.05 \\
C29916 & J064045.23+091606.6 &  17.36$\pm$0.00 & 16.60$\pm$0.01 & 15.94$\pm$0.01  & 14.12$\pm$0.03 & 13.42$\pm$0.03 & 13.15$\pm$0.03 \\
C30006 & J064045.48+094910.2 &  16.69$\pm$0.00 & 16.28$\pm$0.01 & 15.39$\pm$0.00  & 13.27$\pm$0.03 & 12.65$\pm$0.03 & 12.20$\pm$0.03 \\
C30045 & J064045.64+091212.7 &  19.48$\pm$0.02 & 18.34$\pm$0.02 & 17.74$\pm$0.02  & 15.22$\pm$0.05 & 14.55$\pm$0.06 & 14.14$\pm$0.07 \\
C30125 & J064045.88+093844.4 &  17.80$\pm$0.01 & 16.82$\pm$0.01 & 15.49$\pm$0.00  & 13.22$\pm$0.03 & 12.61$\pm$0.02 & 12.34$\pm$0.03 \\
C30190 & J064046.10+094750.2 &  16.80$\pm$0.00 & 16.08$\pm$0.01 & 15.43$\pm$0.00  & 13.89$\pm$0.04 & 13.15$\pm$0.03 & 13.02$\pm$0.04 \\
C30230 & J064046.22+095140.0 &  19.06$\pm$0.03 & 17.56$\pm$0.02 & 16.81$\pm$0.01  & 14.43$\pm$0.04 & 13.74$\pm$0.04 & 13.30$\pm$0.05 \\
C30330 & J064046.54+093352.4 &  17.81$\pm$0.01 & 17.01$\pm$0.01 & 16.30$\pm$0.01  & 14.77$\pm$0.05 & 14.00$\pm$0.03 & 13.80$\pm$0.05 \\
C30381 & J064046.69+094812.6 &  19.58$\pm$0.06 & 18.18$\pm$0.05 & 17.32$\pm$0.02  & 14.96$\pm$0.04 & 14.43$\pm$0.04 & 14.04$\pm$0.07 \\
C30388 & J064046.69+094001.4 &  18.21$\pm$0.01 & 16.36$\pm$0.01 & 17.06$\pm$0.01  & 15.38$\pm$0.06 & 14.86$\pm$0.05 & 14.53$\pm$0.09 \\
C30443 & J064046.87+093230.9 &  17.07$\pm$0.00 & 16.20$\pm$0.01 & 15.41$\pm$0.00  & 13.73$\pm$0.04 & 13.02$\pm$0.03 & 12.77$\pm$0.04 \\
C30451 & J064046.89+095756.0 &  19.66$\pm$0.06 & 18.52$\pm$0.06 & 17.76$\pm$0.03  & 15.84$\pm$0.10 & 15.18$\pm$0.09 & 15.18$\pm$0.17 \\
C30470 & J064046.95+094848.0 &  16.14$\pm$0.00 & 15.56$\pm$0.00 & 15.12$\pm$0.00  & 13.72$\pm$0.03 & 13.04$\pm$0.03 & 12.79$\pm$0.04 \\
C30471 & J064046.95+095240.5 &  18.04$\pm$0.01 & 16.19$\pm$0.01 & 16.80$\pm$0.01  & 14.75$\pm$0.04 & 14.06$\pm$0.05 & 13.41$\pm$0.05 \\
C30512 & J064047.11+093240.1 &  15.22$\pm$0.00 & 14.32$\pm$0.00 & 14.22$\pm$0.00  & 12.77$\pm$0.03 & 12.00$\pm$0.02 & 11.69$\pm$0.03 \\
C30555 & J064047.21+095309.2 &  17.51$\pm$0.01 & 16.78$\pm$0.01 & 16.18$\pm$0.01  & 14.61$\pm$0.04 & 13.91$\pm$0.03 & 13.77$\pm$0.04 \\
C30573 & J064047.29+094727.5 &  17.22$\pm$0.01 & 16.55$\pm$0.01 & 15.86$\pm$0.00  & 14.31$\pm$0.04 & 13.68$\pm$0.03 & 13.50$\pm$0.04 \\
C30656 & J064047.56+094033.1 &  19.57$\pm$0.04 & 18.63$\pm$0.05 & 17.30$\pm$0.01  & 15.21$\pm$0.06 & 14.46$\pm$0.04 & 14.45$\pm$0.09 \\
C30761 & J064047.93+093303.1 &  17.41$\pm$0.01 & 16.62$\pm$0.01 & 15.99$\pm$0.01  & 14.41$\pm$0.03 & 13.73$\pm$0.03 & 13.47$\pm$0.04 \\
C30824 & J064048.09+095339.4 &  15.45$\pm$0.00 & 14.99$\pm$0.00 & 14.64$\pm$0.00  & 13.50$\pm$0.03 & 12.90$\pm$0.03 & 12.73$\pm$0.03 \\
C30854 & J064048.17+095911.8 &  19.64$\pm$0.06 & 18.85$\pm$0.07 & 17.61$\pm$0.02  & 15.52$\pm$0.06 & 14.88$\pm$0.05 & 14.53$\pm$0.11 \\
C30856 & J064048.20+092700.8 &  17.17$\pm$0.00 & 16.36$\pm$0.01 & 15.56$\pm$0.00  & 13.88$\pm$0.03 & 13.14$\pm$0.03 & 12.93$\pm$0.03 \\
C30880 & J064048.27+093638.7 &  15.72$\pm$0.00 & 15.05$\pm$0.00 & 14.46$\pm$0.00  & 12.92$\pm$0.03 & 12.17$\pm$0.02 & 11.95$\pm$0.03 \\
C30909 & J064048.38+094838.6 &  16.39$\pm$0.00 & 15.22$\pm$0.00 & 15.21$\pm$0.00  & 13.43$\pm$0.02 & 12.29$\pm$0.03 & 11.47$\pm$0.03 \\
C30967 & J064048.53+093416.8 &  18.44$\pm$0.02 & 17.50$\pm$0.02 & 16.67$\pm$0.01  & 14.95$\pm$0.05 & 14.23$\pm$0.05 & 13.94$\pm$0.07 \\
C30991 & J064048.63+093252.4 &  16.16$\pm$0.00 & 15.60$\pm$0.00 & 15.10$\pm$0.00  & 13.69$\pm$0.04 & 13.04$\pm$0.03 & 12.80$\pm$0.03 \\
C31021 & J064048.76+093242.5 &  15.43$\pm$0.00 & 14.93$\pm$0.00 & 14.51$\pm$0.00  & 13.28$\pm$0.03 & 12.60$\pm$0.03 & 12.40$\pm$0.03 \\
C31040 & J064048.85+094325.7 &  15.91$\pm$0.00 & 15.27$\pm$0.00 & 14.78$\pm$0.00  & 13.33$\pm$0.03 & 12.28$\pm$0.03 & 11.71$\pm$0.02 \\
C31147 & J064049.21+095738.7 &  16.63$\pm$0.00 & 15.73$\pm$0.01 & 15.35$\pm$0.01  & 13.57$\pm$0.03 & 12.74$\pm$0.04 & 12.37$\pm$0.04 \\
C31149 & J064049.22+094440.0 &  17.78$\pm$0.01 & 16.58$\pm$0.01 & 16.49$\pm$0.01  & 14.85$\pm$0.04 & 13.29$\pm$0.02 & 12.07$\pm$0.03 \\
C31178 & J064049.32+095851.4 &  17.94$\pm$0.01 & 17.49$\pm$0.02 & 16.80$\pm$0.01  & 15.24$\pm$0.06 & 14.49$\pm$0.06 & 14.27$\pm$0.09 \\
C31190 & J064049.36+095254.0 &  19.14$\pm$0.04 & 17.56$\pm$0.03 & 18.13$\pm$0.04  & 15.83$\pm$0.09 & 14.14$\pm$0.04 & 12.72$\pm$0.04 \\
C31293 & J064049.67+101701.1 &  17.72$\pm$0.02 & 16.87$\pm$0.02 & 16.00$\pm$0.01  & 14.30$\pm$0.04 & 13.62$\pm$0.03 & 13.24$\pm$0.04 \\
C31309 & J064049.74+095258.6 &  17.69$\pm$0.01 & 16.85$\pm$0.01 & 16.02$\pm$0.01  & 14.20$\pm$0.03 & 13.56$\pm$0.03 & 13.33$\pm$0.05 \\
C31352 & J064049.89+093649.5 &  14.77$\pm$0.00 & 13.94$\pm$0.00 & 13.98$\pm$0.00  & 12.40$\pm$0.03 & 11.61$\pm$0.03 & 11.16$\pm$0.02 \\
C31375 & J064049.99+095112.7 &  18.36$\pm$0.01 & 16.54$\pm$0.01 & 16.74$\pm$0.01  & 14.88$\pm$0.04 & 14.24$\pm$0.04 & 13.94$\pm$0.06 \\
C31411 & J064050.09+095227.5 &  17.22$\pm$0.01 & 16.36$\pm$0.01 & 15.49$\pm$0.00  & 13.57$\pm$0.04 & 13.01$\pm$0.04 & 12.66$\pm$0.05 \\
C31415 & J064050.11+093039.9 &  18.79$\pm$0.02 & 17.84$\pm$0.02 & 16.73$\pm$0.01  & 14.31$\pm$0.04 & 13.26$\pm$0.03 & 12.88$\pm$0.03 \\
C31430 & J064050.14+095704.0 &  16.96$\pm$0.00 & 16.17$\pm$0.01 & 15.43$\pm$0.00  & 13.82$\pm$0.03 & 13.08$\pm$0.03 & 12.84$\pm$0.05 \\
C31514 & J064050.35+095039.1 &  19.72$\pm$0.04 & 18.79$\pm$0.05 & 17.58$\pm$0.02  & 15.37$\pm$0.07 & 14.84$\pm$0.06 & 14.41$\pm$0.09 \\
C31556 & J064050.47+095530.8 &  19.66$\pm$0.06 & 18.45$\pm$0.06 & 17.72$\pm$0.03  & 15.71$\pm$0.08 & 14.91$\pm$0.05 & 14.56$\pm$0.09 \\
C31566 & J064050.50+094545.4 &  18.06$\pm$0.01 & 17.24$\pm$0.02 & 16.50$\pm$0.01  & 14.82$\pm$0.04 & 14.30$\pm$0.04 & 13.93$\pm$0.06 \\
C31611 & J064050.64+093131.5 &  18.73$\pm$0.02 & 17.75$\pm$0.02 & 16.40$\pm$0.01  & 14.15$\pm$0.06 & 13.57$\pm$0.03 & 13.20$\pm$0.04 \\
C31662 & J064050.79+094155.4 &  18.40$\pm$0.01 & 17.34$\pm$0.02 & 16.39$\pm$0.01  & 14.35$\pm$0.03 & 13.78$\pm$0.03 & 13.56$\pm$0.04 \\
C31669 & J064050.81+095257.6 &  19.47$\pm$0.04 & 17.97$\pm$0.03 & 17.51$\pm$0.02  & 15.18$\pm$0.05 & 14.46$\pm$0.04 & 13.96$\pm$0.06 \\
C31681 & J064050.87+095239.8 &  19.40$\pm$0.05 & 18.35$\pm$0.06 & 17.19$\pm$0.02  & 15.12$\pm$0.05 & 14.49$\pm$0.04 & 14.09$\pm$0.07 \\
C31682 & J064050.86+095553.0 &  15.00$\pm$0.00 & 14.51$\pm$0.00 & 14.15$\pm$0.00  & 12.86$\pm$0.02 & 12.19$\pm$0.03 & 11.97$\pm$0.02 \\
C31767 & J064051.14+095037.9 &  18.39$\pm$0.01 & 17.18$\pm$0.01 & 16.47$\pm$0.01  & 14.51$\pm$0.04 & 13.84$\pm$0.02 & 13.32$\pm$0.04 \\
C31826 & J064051.30+095328.7 &  19.95$\pm$0.06 & 18.87$\pm$0.06 & 17.57$\pm$0.02  & 15.35$\pm$0.05 & 14.78$\pm$0.06 & 14.50$\pm$0.09 \\
C31849 & J064051.37+093013.3 &  17.38$\pm$0.01 & 16.51$\pm$0.01 & 15.68$\pm$0.00  & 13.87$\pm$0.03 & 13.19$\pm$0.03 & 12.97$\pm$0.03 \\
C31874 & J064051.41+095324.2 &  19.15$\pm$0.03 & 18.07$\pm$0.03 & 16.89$\pm$0.01  & 14.69$\pm$0.04 & 14.08$\pm$0.05 & 13.88$\pm$0.06 \\
C31888 & J064051.47+093146.8 &  17.67$\pm$0.01 & 17.02$\pm$0.01 & 16.38$\pm$0.01  & 15.01$\pm$0.04 & 14.35$\pm$0.05 & 14.12$\pm$0.07 \\
C31889 & J064051.47+093714.5 &  16.15$\pm$0.00 & 15.60$\pm$0.00 & 15.08$\pm$0.00  & 13.72$\pm$0.03 & 12.99$\pm$0.03 & 12.87$\pm$0.03 \\
C32005 & J064051.91+093755.9 &  15.71$\pm$0.00 & 15.45$\pm$0.00 & 15.27$\pm$0.00  & 14.37$\pm$0.04 & 13.62$\pm$0.03 & 12.89$\pm$0.03 \\
C32054 & J064052.08+095213.8 &  15.55$\pm$0.00 & 14.98$\pm$0.00 & 14.50$\pm$0.00  & 13.10$\pm$0.02 & 12.40$\pm$0.02 & 12.21$\pm$0.03 \\
C32060 & J064052.11+092913.9 &  18.71$\pm$0.03 & 17.50$\pm$0.02 & 16.78$\pm$0.01  & 14.15$\pm$0.03 & 13.34$\pm$0.04 & 12.85$\pm$0.03 \\
C32086 & J064052.20+095643.3 &  16.94$\pm$0.00 & 16.22$\pm$0.01 & 15.64$\pm$0.00  & 14.16$\pm$0.04 & 13.39$\pm$0.04 & 13.24$\pm$0.05 \\
C32087 & J064052.21+095231.1 &  16.44$\pm$0.00 & 15.78$\pm$0.00 & 15.22$\pm$0.00  & 13.73$\pm$0.03 & 12.99$\pm$0.02 & 12.74$\pm$0.04 \\
C32167 & J064052.54+095058.5 &  17.12$\pm$0.01 & 16.38$\pm$0.01 & 15.75$\pm$0.01  & 14.19$\pm$0.04 & 13.45$\pm$0.03 & 13.23$\pm$0.03 \\
C32171 & J064052.55+095206.0 &  15.55$\pm$0.00 & 14.88$\pm$0.00 & 14.32$\pm$0.00  & 12.69$\pm$0.02 & 11.97$\pm$0.02 & 11.72$\pm$0.03 \\
C32207 & J064052.68+094421.0 &  16.04$\pm$0.00 & 15.34$\pm$0.00 & 14.75$\pm$0.00  & 13.19$\pm$0.02 & 12.51$\pm$0.03 & 12.26$\pm$0.04 \\
C32219 & J064052.73+092843.7 &  18.19$\pm$0.01 & 17.09$\pm$0.01 & 16.85$\pm$0.01  & 15.06$\pm$0.05 & 14.02$\pm$0.04 & 13.38$\pm$0.04 \\
C32226 & J064052.76+094300.4 &  17.68$\pm$0.01 & 16.86$\pm$0.01 & 16.05$\pm$0.01  & 14.32$\pm$0.04 & 13.59$\pm$0.04 & 13.28$\pm$0.04 \\
C32265 & J064052.93+094454.4 &  15.01$\pm$0.00 & 14.40$\pm$0.00 & 14.10$\pm$0.00  & 12.70$\pm$0.02 & 11.86$\pm$0.02 & 11.27$\pm$0.02 \\
C32270 & J064052.96+092625.7 &  18.23$\pm$0.01 & 16.55$\pm$0.01 & 16.31$\pm$0.01  & 14.14$\pm$0.03 & 13.33$\pm$0.03 & 12.92$\pm$0.03 \\
C32295 & J064053.02+095259.5 &  16.35$\pm$0.00 & 15.72$\pm$0.00 & 15.17$\pm$0.00  & 13.40$\pm$0.02 & 12.67$\pm$0.03 & 12.46$\pm$0.03 \\
C32341 & J064053.21+092954.1 &  17.83$\pm$0.01 & 16.97$\pm$0.01 & 16.18$\pm$0.01  & 14.50$\pm$0.07 & 13.78$\pm$0.07 & 13.54$\pm$0.05 \\
C32413 & J064053.53+102252.7 &  18.28$\pm$0.02 & 16.61$\pm$0.01 & 16.46$\pm$0.01  & 14.58$\pm$0.04 & 13.45$\pm$0.03 & 12.73$\pm$0.03 \\
C32434 & J064053.63+092953.3 &  18.69$\pm$0.02 & 17.39$\pm$0.02 & 16.66$\pm$0.01  & 14.59$\pm$0.05 & 13.97$\pm$0.03 & 13.57$\pm$0.05 \\
C32443 & J064053.64+093324.8 &  14.10$\pm$0.00 & 13.40$\pm$0.00 & 13.47$\pm$0.00  & 12.35$\pm$0.03 & 11.68$\pm$0.02 & 11.32$\pm$0.02 \\
C32453 & J064053.67+095800.0 &  16.26$\pm$0.01 & 15.67$\pm$0.01 & 15.23$\pm$0.01  & 13.81$\pm$0.03 & 13.08$\pm$0.03 & 12.86$\pm$0.04 \\
C32515 & J064053.95+095058.1 &  17.93$\pm$0.01 & 17.03$\pm$0.02 & 16.14$\pm$0.01  & 14.27$\pm$0.04 & 13.61$\pm$0.04 & 13.46$\pm$0.05 \\
C32540 & J064054.11+092951.1 &  16.68$\pm$0.00 & 16.00$\pm$0.01 & 15.42$\pm$0.00  & 13.81$\pm$0.03 & 13.12$\pm$0.03 & 12.95$\pm$0.03 \\
C32541 & J064054.11+095224.5 &  18.37$\pm$0.02 & 16.41$\pm$0.01 & 17.28$\pm$0.02  & 15.34$\pm$0.07 & 14.88$\pm$0.06 & 14.33$\pm$0.08 \\
C32545 & J064054.13+094843.4 &  16.62$\pm$0.00 & 14.59$\pm$0.00 & 15.72$\pm$0.00  & 14.16$\pm$0.03 & 13.43$\pm$0.02 & 13.07$\pm$0.03 \\
C32567 & J064054.19+095552.0 &  16.04$\pm$0.00 & 15.47$\pm$0.00 & 15.03$\pm$0.00  & 13.69$\pm$0.02 & 12.94$\pm$0.03 & 12.76$\pm$0.03 \\
C32568 & J064054.20+095616.9 &  20.08$\pm$0.09 & 18.73$\pm$0.08 & 17.76$\pm$0.03  & 15.38$\pm$0.08 & 14.79$\pm$0.10 & 14.30$\pm$0.12 \\
C32585 & J064054.26+094920.4 &  15.72$\pm$0.00 & 14.30$\pm$0.00 & 14.64$\pm$0.00  & 13.10$\pm$0.03 & 12.28$\pm$0.03 & 11.80$\pm$0.03 \\
C32812 & J064055.15+093318.6 &  19.15$\pm$0.03 & 18.12$\pm$0.03 & 17.19$\pm$0.01  & 15.35$\pm$0.05 & 14.59$\pm$0.05 & 14.49$\pm$0.09 \\
C32824 & J064055.19+095049.8 &  15.29$\pm$0.00 & 14.76$\pm$0.00 & 14.38$\pm$0.00  & 13.07$\pm$0.02 & 12.42$\pm$0.03 & 12.23$\pm$0.03 \\
C32846 & J064055.28+093325.0 &  19.23$\pm$0.03 & 18.22$\pm$0.03 & 17.18$\pm$0.01  & 15.11$\pm$0.06 & 14.50$\pm$0.06 & 14.45$\pm$0.11 \\
C32868 & J064055.36+095215.9 &  18.37$\pm$0.01 & 17.42$\pm$0.02 & 16.26$\pm$0.01  & 14.16$\pm$0.05 & 13.58$\pm$0.05 & 13.25$\pm$0.05 \\
C32879 & J064055.43+093723.7 &  15.00$\pm$0.00 & 14.49$\pm$0.00 & 14.04$\pm$0.00  & 12.70$\pm$0.03 & 12.02$\pm$0.03 & 11.80$\pm$0.03 \\
C32892 & J064055.50+093121.4 &  13.54$\pm$0.00 & 13.01$\pm$0.00 & 12.60$\pm$0.00  & 11.50$\pm$0.03 & 10.80$\pm$0.02 & 10.66$\pm$0.02 \\
C32919 & J064055.62+093824.9 &  17.61$\pm$0.01 & 16.72$\pm$0.01 & 15.75$\pm$0.00  & 14.12$\pm$0.03 & 13.39$\pm$0.03 & 13.04$\pm$0.04 \\
C32922 & J064055.62+095212.5 &  19.79$\pm$0.07 & 18.52$\pm$0.06 & 17.29$\pm$0.02  & 15.06$\pm$0.05 & 14.49$\pm$0.05 & 14.22$\pm$0.07 \\
C32959 & J064055.73+095707.7 &  18.67$\pm$0.04 & 17.64$\pm$0.05 & 16.67$\pm$0.02  & 14.75$\pm$0.04 & 14.05$\pm$0.04 & 13.81$\pm$0.05 \\
C32960 & J064055.74+094645.6 &  17.66$\pm$0.01 & 16.72$\pm$0.01 & 15.81$\pm$0.00  & 13.94$\pm$0.03 & 13.28$\pm$0.04 & 12.90$\pm$0.03 \\
C32974 & J064055.79+094018.2 &  16.98$\pm$0.00 & 16.26$\pm$0.01 & 15.63$\pm$0.00  & 13.92$\pm$0.03 & 13.22$\pm$0.03 & 12.95$\pm$0.04 \\
C32993 & J064055.87+093717.8 &  18.88$\pm$0.03 & 17.70$\pm$0.03 & 16.66$\pm$0.01  & 14.46$\pm$0.04 & 13.87$\pm$0.03 & 13.56$\pm$0.05 \\
C32994 & J064055.87+095130.5 &  16.82$\pm$0.00 & 16.09$\pm$0.01 & 15.45$\pm$0.00  & 13.86$\pm$0.03 & 13.15$\pm$0.02 & 12.92$\pm$0.03 \\
C33060 & J064056.14+091607.4 &  19.82$\pm$0.03 & 18.74$\pm$0.03 & 17.66$\pm$0.02  & 15.23$\pm$0.06 & 14.38$\pm$0.05 & 13.93$\pm$0.06 \\
C33066 & J064056.17+093630.9 &  15.66$\pm$0.00 & 14.92$\pm$0.00 & 14.44$\pm$0.00  & 11.89$\pm$0.02 & 10.82$\pm$0.02 & 10.05$\pm$0.02 \\
C33082 & J064056.26+093932.6 &  16.38$\pm$0.00 & 15.64$\pm$0.00 & 15.20$\pm$0.00  & 13.22$\pm$0.03 & 12.32$\pm$0.03 & 11.76$\pm$0.02 \\
C33085 & J064056.27+094038.0 &  19.11$\pm$0.02 & 18.20$\pm$0.03 & 17.46$\pm$0.02  & 15.89$\pm$0.08 & 15.29$\pm$0.09 & 14.78$\pm$0.11 \\
C33098 & J064056.31+093417.9 &  16.94$\pm$0.01 & 16.33$\pm$0.01 & 15.90$\pm$0.01  & 14.67$\pm$0.03 & 14.00$\pm$0.03 & 13.71$\pm$0.05 \\
C33122 & J064056.40+093553.3 &  15.98$\pm$0.00 & 14.69$\pm$0.00 & 14.84$\pm$0.00  & 12.77$\pm$0.03 & 11.79$\pm$0.02 & 11.02$\pm$0.02 \\
C33153 & J064056.49+092953.8 &  17.81$\pm$0.01 & 16.85$\pm$0.01 & 15.71$\pm$0.00  & 13.62$\pm$0.03 & 12.94$\pm$0.03 & 12.72$\pm$0.03 \\
C33245 & J064056.84+095156.6 &  16.96$\pm$0.00 & 16.20$\pm$0.01 & 15.52$\pm$0.00  & 14.02$\pm$0.03 & 13.30$\pm$0.02 & 13.01$\pm$0.04 \\
C33309 & J064057.07+095642.7 &  18.51$\pm$0.03 & 17.60$\pm$0.05 & 16.64$\pm$0.02  & 14.72$\pm$0.04 & 14.11$\pm$0.04 & 13.81$\pm$0.07 \\
C33395 & J064057.46+092617.0 &  19.03$\pm$0.02 & 18.01$\pm$0.02 & 17.28$\pm$0.01  & 15.50$\pm$0.06 & 15.02$\pm$0.07 & 14.56$\pm$0.09 \\
C33396 & J064057.46+092923.4 &  16.75$\pm$0.00 & 16.10$\pm$0.01 & 15.49$\pm$0.00  & 14.11$\pm$0.03 & 13.45$\pm$0.03 & 13.19$\pm$0.04 \\
C33404 & J064057.48+095457.4 &  18.68$\pm$0.02 & 17.85$\pm$0.03 & 16.77$\pm$0.01  & 14.82$\pm$0.04 & 14.26$\pm$0.04 & 14.04$\pm$0.06 \\
C33406 & J064057.50+094920.8 &  17.28$\pm$0.01 & 16.41$\pm$0.01 & 15.49$\pm$0.00  & 13.70$\pm$0.02 & 13.06$\pm$0.02 & 12.78$\pm$0.04 \\
C33435 & J064057.59+095812.7 &  18.45$\pm$0.02 & 17.20$\pm$0.02 & 16.47$\pm$0.01  & 14.06$\pm$0.04 & 13.30$\pm$0.04 & 12.82$\pm$0.05 \\
C33457 & J064057.67+093150.1 &  18.37$\pm$0.01 & 17.55$\pm$0.02 & 16.37$\pm$0.01  & 14.48$\pm$0.03 & 13.88$\pm$0.03 & 13.64$\pm$0.04 \\
C33507 & J064057.85+094120.2 &  15.56$\pm$0.00 & 14.70$\pm$0.00 & 14.44$\pm$0.00  & 12.87$\pm$0.03 & 11.91$\pm$0.03 & 11.27$\pm$0.02 \\
C33540 & J064058.00+094131.5 &  19.21$\pm$0.03 & 18.19$\pm$0.03 & 17.14$\pm$0.01  & 15.10$\pm$0.05 & 14.40$\pm$0.05 & 14.16$\pm$0.06 \\
C33568 & J064058.10+093653.4 &  17.74$\pm$0.01 & 16.46$\pm$0.01 & 15.56$\pm$0.00  & 13.31$\pm$0.03 & 12.48$\pm$0.02 & 12.08$\pm$0.02 \\
C33578 & J064058.14+095235.4 &  19.56$\pm$0.05 & 18.39$\pm$0.05 & 17.15$\pm$0.02  & 15.06$\pm$0.05 & 14.36$\pm$0.06 & 14.28$\pm$0.09 \\
C33599 & J064058.21+095544.6 &  16.56$\pm$0.00 & 15.79$\pm$0.00 & 15.10$\pm$0.00  & 13.46$\pm$0.02 & 12.77$\pm$0.03 & 12.53$\pm$0.03 \\
C33600 & J064058.22+095230.8 &  19.38$\pm$0.03 & 17.09$\pm$0.01 & 18.30$\pm$0.03  & 16.39$\pm$0.15 & 15.78$\pm$0.13 & 15.05$\pm$0.16 \\
C33624 & J064058.35+093756.8 &  20.64$\pm$0.10 & 19.11$\pm$0.07 & 17.82$\pm$0.02  & 14.84$\pm$0.03 & 14.07$\pm$0.03 & 13.71$\pm$0.04 \\
C33640 & J064058.40+092725.0 &  17.49$\pm$0.01 & 16.54$\pm$0.01 & 15.63$\pm$0.00  & 13.62$\pm$0.03 & 12.91$\pm$0.03 & 12.68$\pm$0.03 \\
C33648 & J064058.43+093744.5 &  20.10$\pm$0.09 & 18.94$\pm$0.08 & 17.31$\pm$0.02  & 14.16$\pm$0.03 & 13.39$\pm$0.03 & 12.99$\pm$0.03 \\
C33700 & J064058.64+094554.6 &  15.49$\pm$0.00 & 14.94$\pm$0.00 & 14.49$\pm$0.00  & 13.27$\pm$0.02 & 12.57$\pm$0.03 & 12.35$\pm$0.03 \\
C33709 & J064058.68+093613.2 &  16.57$\pm$0.00 & 15.51$\pm$0.00 & 14.67$\pm$0.00  & 12.41$\pm$0.02 & 11.58$\pm$0.02 & 11.13$\pm$0.02 \\
C33749 & J064058.84+093918.8 &  16.46$\pm$0.00 & 15.62$\pm$0.01 & 15.27$\pm$0.00  & 13.66$\pm$0.03 & 12.98$\pm$0.02 & 12.72$\pm$0.02 \\
C33801 & J064059.04+094906.2 &  16.56$\pm$0.00 & 15.86$\pm$0.00 & 15.23$\pm$0.00  & 13.73$\pm$0.02 & 12.96$\pm$0.02 & 12.82$\pm$0.03 \\
C33806 & J064059.06+093322.2 &  16.72$\pm$0.00 & 15.29$\pm$0.00 & 15.56$\pm$0.00  & 13.94$\pm$0.03 & 13.09$\pm$0.04 & 12.60$\pm$0.04 \\
C33866 & J064059.32+094616.6 &  15.38$\pm$0.00 & 14.59$\pm$0.00 & 14.25$\pm$0.00  & 12.78$\pm$0.02 & 11.92$\pm$0.03 & 11.51$\pm$0.02 \\
C33877 & J064059.37+093333.4 &  17.00$\pm$0.00 & 16.29$\pm$0.01 & 15.93$\pm$0.01  & 12.91$\pm$0.03 & 11.87$\pm$0.03 & 11.19$\pm$0.02 \\
C33882 & J064059.40+095735.6 &  16.86$\pm$0.01 & 16.33$\pm$0.02 & 15.95$\pm$0.02  & 14.75$\pm$0.06 & 14.05$\pm$0.04 & 13.78$\pm$0.05 \\
C33922 & J064059.56+093906.4 &  17.53$\pm$0.01 & 16.28$\pm$0.01 & 16.04$\pm$0.01  & 13.69$\pm$0.03 & 12.79$\pm$0.02 & 12.27$\pm$0.03 \\
C33944 & J064059.67+094904.7 &  19.18$\pm$0.03 & 17.50$\pm$0.02 & 17.53$\pm$0.02  & 15.06$\pm$0.05 & 13.77$\pm$0.03 & 12.92$\pm$0.04 \\
C33966 & J064059.79+100212.6 &  17.89$\pm$0.02 & 16.27$\pm$0.02 & 16.67$\pm$0.04  & 14.66$\pm$0.04 & 13.82$\pm$0.04 & 13.50$\pm$0.04 \\
C33976 & J064059.83+095148.9 &  16.18$\pm$0.00 & 15.50$\pm$0.00 & 14.93$\pm$0.00  & 13.46$\pm$0.02 & 12.78$\pm$0.03 & 12.61$\pm$0.03 \\
C33988 & J064059.87+094932.9 &  17.73$\pm$0.01 & 16.97$\pm$0.01 & 16.21$\pm$0.01  & 14.53$\pm$0.04 & 13.95$\pm$0.04 & 13.70$\pm$0.05 \\
C34090 & J064100.28+092834.1 &  17.86$\pm$0.01 & 15.98$\pm$0.00 & 16.66$\pm$0.01  & 14.67$\pm$0.04 & 13.86$\pm$0.03 & 13.34$\pm$0.04 \\
C34127 & J064100.41+094115.3 &  18.83$\pm$0.02 & 17.87$\pm$0.02 & 16.84$\pm$0.01  & 14.93$\pm$0.07 & 14.21$\pm$0.06 & 13.89$\pm$0.08 \\
C34182 & J064100.65+100214.4 &  18.19$\pm$0.03 & 17.37$\pm$0.06 & 16.44$\pm$0.03  & 14.58$\pm$0.03 & 13.99$\pm$0.03 & 13.84$\pm$0.06 \\
C34222 & J064100.81+095207.6 &  16.78$\pm$0.01 & 16.14$\pm$0.01 & 15.72$\pm$0.01  & 14.03$\pm$0.02 & 13.12$\pm$0.02 & 12.63$\pm$0.03 \\
C34223 & J064100.83+093014.3 &  19.15$\pm$0.03 & 17.66$\pm$0.02 & 17.08$\pm$0.01  & 14.82$\pm$0.04 & 14.28$\pm$0.05 & 13.93$\pm$0.06 \\
C34280 & J064101.05+092233.5 &  18.99$\pm$0.02 & 18.14$\pm$0.03 & 17.06$\pm$0.01  & 15.09$\pm$0.05 & 14.45$\pm$0.05 & 14.08$\pm$0.07 \\
C34324 & J064101.23+091339.9 &  17.17$\pm$0.00 & 16.72$\pm$0.01 & 16.17$\pm$0.01  & 14.66$\pm$0.03 & 14.06$\pm$0.04 & 13.94$\pm$0.06 \\
C34426 & J064101.61+093728.7 &  17.31$\pm$0.01 & 15.61$\pm$0.00 & 16.25$\pm$0.01  & 14.75$\pm$0.03 & 13.83$\pm$0.04 & 13.33$\pm$0.04 \\
C34452 & J064101.69+092303.7 &  19.86$\pm$0.04 & 18.66$\pm$0.04 & 17.57$\pm$0.02  & 15.33$\pm$0.05 & 14.75$\pm$0.06 & 14.46$\pm$0.09 \\
C34464 & J064101.73+095551.4 &  16.66$\pm$0.00 & 15.84$\pm$0.00 & 15.01$\pm$0.00  & 13.28$\pm$0.03 & 12.54$\pm$0.03 & 12.30$\pm$0.03 \\
C34532 & J064101.95+095003.8 &  18.02$\pm$0.01 & 17.05$\pm$0.01 & 16.33$\pm$0.01  & 14.31$\pm$0.03 & 13.74$\pm$0.04 & 13.51$\pm$0.04 \\
C34638 & J064102.45+095225.0 &  16.91$\pm$0.00 & 16.21$\pm$0.01 & 15.65$\pm$0.00  & 14.17$\pm$0.03 & 13.52$\pm$0.02 & 13.27$\pm$0.03 \\
C34671 & J064102.59+093513.1 &  14.79$\pm$0.00 & 14.35$\pm$0.00 & 14.03$\pm$0.00  & 12.85$\pm$0.02 & 12.23$\pm$0.03 & 12.05$\pm$0.02 \\
C34675 & J064102.59+093640.2 &  19.11$\pm$0.04 & 17.68$\pm$0.03 & 16.87$\pm$0.01  & 14.34$\pm$0.03 & 13.53$\pm$0.02 & 13.14$\pm$0.04 \\
C34678 & J064102.62+095102.6 &  18.40$\pm$0.02 & 17.41$\pm$0.02 & 16.33$\pm$0.01  & 14.20$\pm$0.03 & 13.66$\pm$0.04 & 13.38$\pm$0.04 \\
C34713 & J064102.76+094836.4 &  20.35$\pm$0.08 & 19.32$\pm$0.09 & 18.12$\pm$0.03  & 15.85$\pm$0.08 & 15.37$\pm$0.08 & 15.23$\pm$0.17 \\
C34722 & J064102.79+092315.2 &  17.44$\pm$0.00 & 16.67$\pm$0.01 & 15.93$\pm$0.00  & 14.30$\pm$0.03 & 13.57$\pm$0.03 & 13.41$\pm$0.05 \\
C34726 & J064102.84+095522.2 &  18.55$\pm$0.02 & 17.62$\pm$0.02 & 16.55$\pm$0.01  & 14.56$\pm$0.04 & 13.93$\pm$0.03 & 13.61$\pm$0.05 \\
C34733 & J064102.85+100712.0 &  16.40$\pm$0.01 & 15.61$\pm$0.01 & 15.17$\pm$0.01  & 13.98$\pm$0.02 & 13.22$\pm$0.03 & 12.87$\pm$0.03 \\
C34739 & J064102.87+095352.8 &  17.24$\pm$0.01 & 16.37$\pm$0.01 & 15.58$\pm$0.01  & 13.78$\pm$0.02 & 13.11$\pm$0.03 & 12.88$\pm$0.03 \\
C34786 & J064103.09+092904.5 &  17.84$\pm$0.01 & 16.95$\pm$0.01 & 16.10$\pm$0.01  & 14.29$\pm$0.04 & 13.58$\pm$0.03 & 13.31$\pm$0.03 \\
C34803 & J064103.19+092603.0 &  17.00$\pm$0.00 & 16.29$\pm$0.01 & 15.78$\pm$0.00  & 14.22$\pm$0.04 & 13.50$\pm$0.03 & 13.31$\pm$0.04 \\
C34859 & J064103.46+093211.7 &  19.70$\pm$0.04 & 18.58$\pm$0.04 & 17.13$\pm$0.01  & 14.54$\pm$0.03 & 13.75$\pm$0.03 & 13.38$\pm$0.04 \\
C34909 & J064103.61+093029.0 &  16.79$\pm$0.00 & 15.73$\pm$0.00 & 14.89$\pm$0.00  & 12.81$\pm$0.03 & 12.03$\pm$0.03 & 11.69$\pm$0.03 \\
C34945 & J064103.74+092739.8 &  15.45$\pm$0.00 & 14.97$\pm$0.00 & 14.61$\pm$0.00  & 13.34$\pm$0.03 & 12.67$\pm$0.02 & 12.49$\pm$0.03 \\
C34989 & J064103.89+091935.2 &  20.81$\pm$0.10 & 18.95$\pm$0.06 & 18.35$\pm$0.04  & 15.24$\pm$0.05 & 14.27$\pm$0.05 & 13.74$\pm$0.06 \\
C35020 & J064104.00+092824.3 &  18.48$\pm$0.01 & 17.45$\pm$0.01 & 16.47$\pm$0.01  & 14.52$\pm$0.06 & 13.87$\pm$0.05 & 13.58$\pm$0.05 \\
C35042 & J064104.07+093521.1 &  15.98$\pm$0.00 & 15.30$\pm$0.00 & 14.67$\pm$0.00  & 13.02$\pm$0.03 & 12.34$\pm$0.02 & 12.10$\pm$0.02 \\
C35072 & J064104.20+093655.6 &  18.83$\pm$0.02 & 17.85$\pm$0.02 & 16.70$\pm$0.01  & 14.67$\pm$0.04 & 13.98$\pm$0.03 & 13.84$\pm$0.04 \\
C35074 & J064104.20+092840.5 &  19.83$\pm$0.03 & 19.03$\pm$0.05 & 17.66$\pm$0.01  & 15.60$\pm$0.07 & 14.93$\pm$0.06 & 14.55$\pm$0.09 \\
C35091 & J064104.32+093547.7 &  17.90$\pm$0.01 & 16.94$\pm$0.02 & 16.08$\pm$0.01  & 14.25$\pm$0.03 & 13.60$\pm$0.03 & 13.30$\pm$0.03 \\
C35101 & J064104.37+092730.6 &  17.63$\pm$0.01 & 16.82$\pm$0.01 & 16.08$\pm$0.01  & 14.41$\pm$0.03 & 13.71$\pm$0.04 & 13.49$\pm$0.05 \\
C35111 & J064104.44+093643.4 &  16.86$\pm$0.01 & 15.53$\pm$0.01 & 15.66$\pm$0.01  & 13.93$\pm$0.03 & 13.11$\pm$0.02 & 12.64$\pm$0.02 \\
C35119 & J064104.49+095212.7 &  18.45$\pm$0.01 & 17.64$\pm$0.02 & 16.75$\pm$0.01  & 14.94$\pm$0.04 & 14.38$\pm$0.05 & 14.17$\pm$0.07 \\
C35122 & J064104.51+093013.4 &  17.34$\pm$0.01 & 16.51$\pm$0.01 & 15.71$\pm$0.00  & 13.97$\pm$0.03 & 13.21$\pm$0.03 & 13.03$\pm$0.04 \\
C35132 & J064104.55+092609.2 &  18.13$\pm$0.02 & 17.17$\pm$0.02 & 16.45$\pm$0.01  & 14.62$\pm$0.04 & 13.91$\pm$0.03 & 13.71$\pm$0.05 \\
C35140 & J064104.58+093830.9 &  17.14$\pm$0.00 & 15.58$\pm$0.00 & 15.59$\pm$0.00  & 13.77$\pm$0.03 & 13.03$\pm$0.03 & 12.55$\pm$0.03 \\
C35186 & J064104.82+094433.3 &  18.71$\pm$0.02 & 17.19$\pm$0.01 & 17.04$\pm$0.01  & 14.33$\pm$0.03 & 13.52$\pm$0.03 & 12.92$\pm$0.04 \\
C35188 & J064104.83+095225.4 &  20.01$\pm$0.06 & 18.79$\pm$0.05 & 17.45$\pm$0.02  & 15.11$\pm$0.04 & 14.51$\pm$0.04 & 14.28$\pm$0.08 \\
C35239 & J064105.07+094922.8 &  18.43$\pm$0.01 & 17.42$\pm$0.02 & 16.15$\pm$0.01  & 13.99$\pm$0.03 & 13.41$\pm$0.02 & 13.07$\pm$0.04 \\
C35263 & J064105.14+094855.5 &  15.72$\pm$0.00 & 15.22$\pm$0.00 & 14.85$\pm$0.00  & 13.58$\pm$0.02 & 12.94$\pm$0.03 & 12.75$\pm$0.03 \\
C35309 & J064105.34+092812.5 &  19.28$\pm$0.03 & 17.43$\pm$0.02 & 17.54$\pm$0.02  & 15.30$\pm$0.05 & 14.71$\pm$0.05 & 14.15$\pm$0.07 \\
C35310 & J064105.35+095556.2 &  19.36$\pm$0.05 & 18.29$\pm$0.05 & 17.25$\pm$0.02  & 15.26$\pm$0.05 & 14.65$\pm$0.05 & 14.38$\pm$0.11 \\
C35319 & J064105.37+093313.4 &  14.79$\pm$0.00 & 14.25$\pm$0.00 & 13.87$\pm$0.00  & 12.48$\pm$0.03 & 11.85$\pm$0.02 & 11.64$\pm$0.02 \\
C35339 & J064105.49+095653.4 &  18.70$\pm$0.03 & 17.70$\pm$0.05 & 16.62$\pm$0.02  & 14.41$\pm$0.03 & 13.77$\pm$0.03 & 13.61$\pm$0.06 \\
C35351 & J064105.55+093140.6 &  17.35$\pm$0.01 & 16.43$\pm$0.01 & 15.58$\pm$0.01  & 13.13$\pm$0.04 & 12.36$\pm$0.04 & 12.07$\pm$0.04 \\
C35443 & J064105.98+093139.8 &  18.06$\pm$0.01 & 17.28$\pm$0.01 & 16.48$\pm$0.01  & 14.33$\pm$0.03 & 13.42$\pm$0.03 & 13.06$\pm$0.04 \\
C35444 & J064105.98+093914.2 &  18.17$\pm$0.02 & 16.74$\pm$0.01 & 16.02$\pm$0.01  & 13.73$\pm$0.03 & 13.12$\pm$0.03 & 12.74$\pm$0.03 \\
C35490 & J064106.24+093308.8 &  18.69$\pm$0.02 & 17.57$\pm$0.02 & 16.53$\pm$0.01  & 14.11$\pm$0.03 & 13.35$\pm$0.03 & 13.05$\pm$0.03 \\
C35491 & J064106.23+092503.6 &  17.25$\pm$0.00 & 16.17$\pm$0.01 & 15.26$\pm$0.00  & 13.12$\pm$0.02 & 12.49$\pm$0.02 & 12.17$\pm$0.03 \\
C35520 & J064106.42+093506.1 &  19.98$\pm$0.05 & 19.13$\pm$0.07 & 18.29$\pm$0.03  & 16.42$\pm$0.12 & 15.95$\pm$0.15 & $>$ 15.22    \\
C35524 & J064106.43+092838.8 &  16.68$\pm$0.00 & 15.57$\pm$0.00 & 15.44$\pm$0.00  & 13.85$\pm$0.03 & 13.12$\pm$0.03 & 12.98$\pm$0.03 \\
C35536 & J064106.51+095345.3 &  17.19$\pm$0.01 & 16.52$\pm$0.01 & 15.87$\pm$0.00  & 14.38$\pm$0.04 & 13.68$\pm$0.04 & 13.45$\pm$0.04 \\
C35615 & J064106.90+092924.0 &  16.93$\pm$0.00 & 16.08$\pm$0.01 & 15.60$\pm$0.00  & 13.41$\pm$0.02 & 12.55$\pm$0.02 & 11.93$\pm$0.02 \\
C35631 & J064106.97+094054.5 &  17.51$\pm$0.01 & 16.58$\pm$0.01 & 15.59$\pm$0.00  & 13.57$\pm$0.03 & 12.84$\pm$0.03 & 12.59$\pm$0.03 \\
C35673 & J064107.16+092729.4 &  14.40$\pm$0.00 & 13.44$\pm$0.00 & 13.73$\pm$0.00  & 12.55$\pm$0.04 & 11.65$\pm$0.04 & 11.04$\pm$0.04 \\
C35681 & J064107.22+094225.5 &  19.16$\pm$0.03 & 18.33$\pm$0.04 & 17.18$\pm$0.01  & 15.30$\pm$0.05 & 14.65$\pm$0.04 & 14.54$\pm$0.09 \\
C35692 & J064107.29+094956.6 &  17.63$\pm$0.01 & 16.70$\pm$0.01 & 15.62$\pm$0.00  & 13.65$\pm$0.03 & 12.98$\pm$0.03 & 12.76$\pm$0.03 \\
C35697 & J064107.30+093118.0 &  17.05$\pm$0.00 & 16.22$\pm$0.01 & 15.53$\pm$0.00  & 13.96$\pm$0.06 & 13.39$\pm$0.05 & 13.13$\pm$0.05 \\
C35719 & J064107.41+093111.0 &  17.17$\pm$0.01 & 16.32$\pm$0.01 & 15.62$\pm$0.00  & 14.03$\pm$0.03 & 13.42$\pm$0.03 & 13.21$\pm$0.03 \\
C35732 & J064107.45+093433.6 &  19.03$\pm$0.03 & 17.82$\pm$0.03 & 17.15$\pm$0.02  & 15.15$\pm$0.05 & 14.47$\pm$0.05 & 14.31$\pm$0.08 \\
C35738 & J064107.49+093336.9 &  19.40$\pm$0.03 & 18.07$\pm$0.03 & 16.93$\pm$0.01  & 14.39$\pm$0.03 & 13.67$\pm$0.03 & 13.29$\pm$0.04 \\
C35756 & J064107.57+094133.6 &  17.81$\pm$0.01 & 16.45$\pm$0.01 & 16.21$\pm$0.01  & 14.46$\pm$0.05 & 13.77$\pm$0.06 & 13.48$\pm$0.07 \\
C35800 & J064107.77+094115.0 &  15.22$\pm$0.00 & 14.67$\pm$0.00 & 14.18$\pm$0.00  & 12.81$\pm$0.03 & 12.04$\pm$0.02 & 11.85$\pm$0.02 \\
C35803 & J064107.77+092813.5 &  15.78$\pm$0.00 & 15.14$\pm$0.00 & 14.57$\pm$0.00  & 13.11$\pm$0.02 & 12.34$\pm$0.02 & 12.18$\pm$0.02 \\
C35846 & J064107.99+093446.9 &  18.31$\pm$0.01 & 17.53$\pm$0.02 & 16.56$\pm$0.01  & 13.98$\pm$0.03 & 12.69$\pm$0.03 & 12.12$\pm$0.02 \\
C35851 & J064108.02+093040.3 &  15.06$\pm$0.00 & 14.63$\pm$0.00 & 14.32$\pm$0.00  & 13.26$\pm$0.03 & 12.64$\pm$0.03 & 12.48$\pm$0.03 \\
C35881 & J064108.18+095415.7 &  19.82$\pm$0.05 & 18.84$\pm$0.06 & 17.41$\pm$0.02  & 15.03$\pm$0.05 & 14.47$\pm$0.04 & 14.28$\pm$0.09 \\
C35894 & J064108.22+093409.4 &  17.31$\pm$0.01 & 16.34$\pm$0.01 & 15.43$\pm$0.01  & 12.97$\pm$0.03 & 11.90$\pm$0.03 & 11.50$\pm$0.04 \\
C35896 & J064108.22+093830.4 &  18.88$\pm$0.02 & 17.75$\pm$0.02 & 16.80$\pm$0.01  & 13.63$\pm$0.03 & 12.31$\pm$0.03 & 11.55$\pm$0.02 \\
C35908 & J064108.28+093022.8 &  17.41$\pm$0.01 & 15.99$\pm$0.01 & 15.91$\pm$0.01  & 13.77$\pm$0.03 & 12.95$\pm$0.03 & 12.55$\pm$0.04 \\
C35926 & J064108.39+094036.1 &  18.18$\pm$0.01 & 17.25$\pm$0.01 & 16.41$\pm$0.01  & 14.54$\pm$0.03 & 13.86$\pm$0.04 & 13.65$\pm$0.04 \\
C35931 & J064108.45+093752.5 &  19.40$\pm$0.03 & 18.27$\pm$0.03 & 17.02$\pm$0.01  & 14.62$\pm$0.03 & 13.98$\pm$0.04 & 13.69$\pm$0.05 \\
C35942 & J064108.57+094251.5 &  15.85$\pm$0.00 & 15.26$\pm$0.00 & 14.73$\pm$0.00  & 13.28$\pm$0.03 & 12.58$\pm$0.03 & 12.38$\pm$0.03 \\
C35948 & J064108.59+093003.6 &  20.13$\pm$0.09 & 18.67$\pm$0.07 & 17.57$\pm$0.02  & 15.44$\pm$0.06 & 14.40$\pm$0.19 & 13.82$\pm$0.24 \\
C35958 & J064108.65+095346.6 &  20.03$\pm$0.09 & 18.98$\pm$0.10 & 18.04$\pm$0.04  & 15.65$\pm$0.09 & 15.26$\pm$0.09 & 14.80$\pm$0.12 \\
C36002 & J064108.86+095301.2 &  17.37$\pm$0.01 & 16.44$\pm$0.01 & 15.87$\pm$0.01  & 14.07$\pm$0.03 & 13.23$\pm$0.03 & 12.76$\pm$0.07 \\
C36016 & J064108.93+095647.7 &  18.95$\pm$0.02 & 17.88$\pm$0.02 & 17.09$\pm$0.01  & 15.19$\pm$0.05 & 14.60$\pm$0.06 & 14.32$\pm$0.09 \\
C36018 & J064108.93+094114.8 &  14.67$\pm$0.00 & 14.26$\pm$0.00 & 13.98$\pm$0.00  & 12.90$\pm$0.03 & 12.28$\pm$0.02 & 12.17$\pm$0.02 \\
C36032 & J064108.96+093346.0 &  16.67$\pm$0.00 & 15.37$\pm$0.00 & 14.88$\pm$0.00  & 12.96$\pm$0.02 & 12.14$\pm$0.02 & 11.80$\pm$0.03 \\
C36070 & J064109.20+095157.1 &  19.31$\pm$0.03 & 18.37$\pm$0.04 & 17.25$\pm$0.01  & 15.23$\pm$0.06 & 14.50$\pm$0.06 & 14.15$\pm$0.09 \\
C36071 & J064109.20+095301.5 &  16.74$\pm$0.00 & 16.00$\pm$0.01 & 15.35$\pm$0.00  & 13.63$\pm$0.05 & 12.95$\pm$0.06 & 12.71$\pm$0.03 \\
C36135 & J064109.52+093525.5 &  15.25$\pm$0.00 & 14.61$\pm$0.00 & 13.99$\pm$0.00  & 12.44$\pm$0.03 & 11.67$\pm$0.02 & 11.52$\pm$0.02 \\
C36169 & J064109.67+094820.5 &  18.20$\pm$0.02 & 17.31$\pm$0.02 & 16.37$\pm$0.01  & 14.56$\pm$0.04 & 13.92$\pm$0.03 & 13.60$\pm$0.04 \\
C36198 & J064109.85+101502.6 &  17.88$\pm$0.04 & 16.80$\pm$0.06 & 16.23$\pm$0.04  & 13.19$\pm$0.02 & 11.80$\pm$0.02 & 10.85$\pm$0.02 \\
C36216 & J064109.93+093020.1 &  16.97$\pm$0.01 & 16.13$\pm$0.01 & 15.64$\pm$0.01  & 13.98$\pm$0.03 & 13.30$\pm$0.02 & 13.25:       \\
C36252 & J064110.15+093128.5 &  17.05$\pm$0.00 & 16.15$\pm$0.01 & 15.35$\pm$0.00  & 13.48$\pm$0.03 & 12.79$\pm$0.03 & 12.61$\pm$0.03 \\
C36287 & J064110.28+093325.1 &  16.83$\pm$0.00 & 16.02$\pm$0.01 & 15.27$\pm$0.00  & 13.52$\pm$0.03 & 12.80$\pm$0.03 & 12.56$\pm$0.02 \\
C36368 & J064110.71+095742.5 &  16.26$\pm$0.01 & 15.62$\pm$0.01 & 15.14$\pm$0.01  & 13.47$\pm$0.03 & 12.76$\pm$0.03 & 12.51$\pm$0.03 \\
C36389 & J064110.80+094641.2 &  17.04$\pm$0.00 & 16.19$\pm$0.01 & 15.33$\pm$0.00  & 13.52$\pm$0.03 & 12.88$\pm$0.03 & 12.67$\pm$0.03 \\
C36407 & J064110.86+095318.3 &  18.08$\pm$0.01 & 17.07$\pm$0.01 & 15.91$\pm$0.01  & 13.68$\pm$0.03 & 13.18$\pm$0.03 & 12.82$\pm$0.04 \\
C36437 & J064111.00+093555.7 &  16.79$\pm$0.00 & 15.67$\pm$0.00 & 15.48$\pm$0.00  & 13.36$\pm$0.03 & 12.23$\pm$0.02 & 11.50$\pm$0.03 \\
C36493 & J064111.28+091948.6 &  18.97$\pm$0.01 & 18.13$\pm$0.02 & 17.03$\pm$0.01  & 13.47$\pm$0.03 & 12.02$\pm$0.02 & 11.20$\pm$0.03 \\
C36596 & J064111.91+093743.9 &  18.70$\pm$0.02 & 17.86$\pm$0.03 & 16.86$\pm$0.01  & 14.66$\pm$0.04 & 13.36$\pm$0.03 & 12.57$\pm$0.03 \\
C36597 & J064111.94+095941.2 &  17.40$\pm$0.02 & 16.61$\pm$0.03 & 15.88$\pm$0.02  & 14.20$\pm$0.04 & 13.52$\pm$0.04 & 13.32$\pm$0.05 \\
C36634 & J064112.08+091448.9 &  19.34$\pm$0.02 & 18.70$\pm$0.03 & 18.16$\pm$0.03  & 16.47$\pm$0.14 & 16.24$\pm$0.21 & 15.58$\pm$0.24 \\
C36662 & J064112.26+094012.1 &  18.85$\pm$0.02 & 17.97$\pm$0.03 & 16.71$\pm$0.01  & 14.74$\pm$0.04 & 14.10$\pm$0.03 & 13.70$\pm$0.05 \\
C36696 & J064112.43+095500.1 &  18.12$\pm$0.01 & 17.29$\pm$0.01 & 16.42$\pm$0.01  & 14.75$\pm$0.04 & 14.13$\pm$0.04 & 13.89$\pm$0.06 \\
C36702 & J064112.42+091324.7 &  20.06$\pm$0.03 & 19.05$\pm$0.04 & 17.48$\pm$0.01  & 14.79$\pm$0.04 & 14.18$\pm$0.04 & 13.79$\pm$0.06 \\
C36709 & J064112.50+094620.4 &  17.63$\pm$0.01 & 16.78$\pm$0.01 & 15.85$\pm$0.00  & 13.92$\pm$0.03 & 13.29$\pm$0.02 & 13.10$\pm$0.03 \\
C36710 & J064112.47+090851.0 &  18.60$\pm$0.01 & 17.70$\pm$0.01 & 16.80$\pm$0.01  & 14.98$\pm$0.05 & 14.28$\pm$0.04 & 14.17$\pm$0.08 \\
C36714 & J064112.52+093508.8 &  18.21$\pm$0.02 & 17.21$\pm$0.02 & 16.11$\pm$0.01  & 14.11$\pm$0.03 & 13.56$\pm$0.03 & 13.25$\pm$0.04 \\
C36794 & J064112.89+094600.8 &  18.14$\pm$0.01 & 17.20$\pm$0.01 & 16.38$\pm$0.01  & 14.50$\pm$0.04 & 13.89$\pm$0.03 & 13.70$\pm$0.05 \\
C36810 & J064112.92+090525.7 &  18.35$\pm$0.01 & 16.93$\pm$0.01 & 16.97$\pm$0.01  & 14.51$\pm$0.04 & 13.67$\pm$0.03 & 13.27$\pm$0.05 \\
C36813 & J064112.96+093532.3 &  16.14$\pm$0.00 & 15.47$\pm$0.00 & 14.82$\pm$0.00  & 13.22$\pm$0.03 & 12.43$\pm$0.02 & 12.28$\pm$0.03 \\
C36818 & J064113.02+092739.3 &  16.20$\pm$0.00 & 15.46$\pm$0.00 & 14.85$\pm$0.00  & 13.25$\pm$0.06 & 12.50$\pm$0.06 & 12.30$\pm$0.05 \\
C36828 & J064113.06+093138.1 &  18.69$\pm$0.02 & 16.83$\pm$0.01 & 17.14$\pm$0.01  & 14.91$\pm$0.04 & 14.17$\pm$0.04 & 13.72$\pm$0.05 \\
C36831 & J064113.07+092304.4 &  17.91$\pm$0.00 & 17.11$\pm$0.01 & 16.32$\pm$0.00  & 14.64$\pm$0.04 & 13.86$\pm$0.03 & 13.65$\pm$0.05 \\
C36835 & J064113.12+093106.7 &  18.53$\pm$0.02 & 17.40$\pm$0.02 & 16.52$\pm$0.01  & 14.39$\pm$0.04 & 13.67$\pm$0.03 & 13.39$\pm$0.05 \\
C36839 & J064113.13+092436.6 &  18.59$\pm$0.02 & 17.56$\pm$0.03 & 16.77$\pm$0.01  & 14.94$\pm$0.05 & 14.41$\pm$0.03 & 14.28$\pm$0.09 \\
C36876 & J064113.31+094958.4 &  19.02$\pm$0.02 & 18.18$\pm$0.03 & 17.39$\pm$0.01  & 15.98$\pm$0.09 & 15.11$\pm$0.06 & 14.85$\pm$0.14 \\
C36877 & J064113.31+095154.5 &  16.65$\pm$0.00 & 15.99$\pm$0.01 & 15.44$\pm$0.00  & 14.00$\pm$0.03 & 13.33$\pm$0.03 & 13.07$\pm$0.04 \\
C36879 & J064113.30+093150.3 &  16.86$\pm$0.00 & 15.51$\pm$0.00 & 14.90$\pm$0.00  & 12.74$\pm$0.03 & 12.03$\pm$0.02 & 11.68$\pm$0.03 \\
C36887 & J064113.36+100330.2 &  18.46$\pm$0.04 & 17.48$\pm$0.06 & 16.60$\pm$0.03  & 14.85$\pm$0.05 & 14.09$\pm$0.05 & 13.81$\pm$0.06 \\
C36888 & J064113.33+092807.4 &  15.60$\pm$0.00 & 15.04$\pm$0.00 & 14.70$\pm$0.00  & 13.42$\pm$0.03 & 12.73$\pm$0.02 & 12.55$\pm$0.03 \\
C36891 & J064113.37+093813.8 &  17.88$\pm$0.01 & 16.97$\pm$0.02 & 16.04$\pm$0.01  & 13.48$\pm$0.03 & 12.31$\pm$0.03 & 11.77$\pm$0.03 \\
C36902 & J064113.41+093023.7 &  20.57$\pm$0.09 & 18.95$\pm$0.06 & 18.44$\pm$0.04  & 15.37$\pm$0.06 & 13.84$\pm$0.04 & 12.88$\pm$0.03 \\
C37041 & J064114.14+092640.5 &  15.87$\pm$0.00 & 15.22$\pm$0.00 & 14.80$\pm$0.00  & 13.22$\pm$0.03 & 12.52$\pm$0.02 & 12.33$\pm$0.02 \\
C37068 & J064114.31+095404.6 &  19.32$\pm$0.03 & 18.31$\pm$0.04 & 17.05$\pm$0.01  & 14.76$\pm$0.04 & 14.16$\pm$0.04 & 13.93$\pm$0.06 \\
C37103 & J064114.47+093321.4 &  14.73$\pm$0.00 & 14.25$\pm$0.00 & 13.86$\pm$0.00  & 12.60$\pm$0.03 & 11.94$\pm$0.03 & 11.72$\pm$0.03 \\
C37104 & J064114.48+093714.4 &  16.30$\pm$0.00 & 15.68$\pm$0.00 & 15.20$\pm$0.00  & 13.88$\pm$0.03 & 13.19$\pm$0.04 & 12.95$\pm$0.04 \\
C37171 & J064114.84+093235.8 &  16.21$\pm$0.00 & 15.39$\pm$0.00 & 14.53$\pm$0.00  & 12.52$\pm$0.03 & 11.69$\pm$0.02 & 11.43$\pm$0.02 \\
C37217 & J064115.11+092644.3 &  16.05$\pm$0.00 & 15.18$\pm$0.00 & 14.89$\pm$0.00  & 13.00$\pm$0.03 & 12.06$\pm$0.02 & 11.60$\pm$0.02 \\
C37237 & J064115.21+093757.7 &  16.24$\pm$0.00 & 15.31$\pm$0.00 & 15.14$\pm$0.00  & 13.72$\pm$0.03 & 12.99$\pm$0.02 & 12.70$\pm$0.02 \\
C37363 & J064115.99+092609.5 &  15.92$\pm$0.00 & 14.62$\pm$0.00 & 14.73$\pm$0.00  & 12.70$\pm$0.03 & 11.91$\pm$0.04 & 11.45$\pm$0.03 \\
C37366 & J064116.00+091635.1 &  19.53$\pm$0.02 & 17.77$\pm$0.01 & 18.34$\pm$0.02  & 16.00$\pm$0.12 & 14.11$\pm$0.04 & 12.83$\pm$0.04 \\
C37387 & J064116.11+092643.5 &  18.57$\pm$0.01 & 17.52$\pm$0.02 & 16.58$\pm$0.01  & 14.62$\pm$0.04 & 13.93$\pm$0.02 & 13.57$\pm$0.05 \\
C37535 & J064116.85+093620.6 &  16.87$\pm$0.01 & 16.00$\pm$0.01 & 15.24$\pm$0.00  & 13.53$\pm$0.03 & 12.86$\pm$0.04 & 12.62$\pm$0.04 \\
C37581 & J064117.06+093252.3 &  17.44$\pm$0.01 & 16.61$\pm$0.01 & 15.93$\pm$0.01  & 14.27$\pm$0.03 & 13.59$\pm$0.04 & 13.36$\pm$0.04 \\
C37590 & J064117.11+095240.6 &  16.67$\pm$0.00 & 16.04$\pm$0.01 & 15.49$\pm$0.00  & 14.06$\pm$0.03 & 13.35$\pm$0.03 & 13.21$\pm$0.03 \\
C37612 & J064117.16+093012.4 &  19.24$\pm$0.04 & 18.74$\pm$0.07 & 17.20$\pm$0.02  & 13.74$\pm$0.03 & 11.99$\pm$0.02 & 11.36$\pm$0.03 \\
C37707 & J064117.51+092806.4 &  18.19$\pm$0.01 & 16.01$\pm$0.00 & 17.33$\pm$0.01  & 15.48$\pm$0.06 & 14.67$\pm$0.05 & 14.30$\pm$0.07 \\
C37748 & J064117.71+092926.2 &  14.96$\pm$0.00 & 14.29$\pm$0.00 & 13.70$\pm$0.00  & 12.12$\pm$0.03 & 11.35$\pm$0.02 & 11.14$\pm$0.02 \\
C37798 & J064117.93+093337.0 &  14.94$\pm$0.00 & 14.41$\pm$0.00 & 13.98$\pm$0.00  & 12.63$\pm$0.02 & 11.97$\pm$0.02 & 11.78$\pm$0.03 \\
C37800 & J064117.95+100402.1 &  17.96$\pm$0.05 & 17.06$\pm$0.08 & 16.19$\pm$0.04  & 14.46$\pm$0.04 & 13.79$\pm$0.03 & 13.52$\pm$0.05 \\
C37804 & J064117.93+092901.1 &  17.29$\pm$0.01 & 15.60$\pm$0.00 & 15.73$\pm$0.00  & 13.33$\pm$0.03 & 12.30$\pm$0.02 & 11.85$\pm$0.02 \\
C37902 & J064118.30+092833.0 &  17.43$\pm$0.01 & 16.72$\pm$0.01 & 15.94$\pm$0.01  & 14.33$\pm$0.04 & 13.63$\pm$0.03 & 13.38$\pm$0.04 \\
C37904 & J064118.32+094406.8 &  16.90$\pm$0.00 & 16.17$\pm$0.01 & 15.54$\pm$0.00  & 14.00$\pm$0.03 & 13.32$\pm$0.02 & 13.03$\pm$0.03 \\
C37927 & J064118.39+093129.5 &  17.70$\pm$0.01 & 16.74$\pm$0.01 & 16.01$\pm$0.01  & 14.31$\pm$0.02 & 13.74$\pm$0.02 & 13.45$\pm$0.04 \\
C38035 & J064118.83+093019.9 &  18.75$\pm$0.02 & 17.80$\pm$0.02 & 16.88$\pm$0.01  & 15.04$\pm$0.05 & 14.41$\pm$0.05 & 14.03$\pm$0.06 \\
C38110 & J064119.12+092629.4 &  16.53$\pm$0.00 & 14.93$\pm$0.00 & 15.21$\pm$0.00  & 13.40$\pm$0.03 & 12.55$\pm$0.02 & 12.16$\pm$0.02 \\
C38146 & J064119.26+093048.7 &  19.11$\pm$0.03 & 18.19$\pm$0.03 & 16.93$\pm$0.01  & 14.83$\pm$0.05 & 14.14$\pm$0.04 & 13.84$\pm$0.06 \\
C38152 & J064119.29+093807.2 &  20.26$\pm$0.07 & 18.58$\pm$0.04 & 17.75$\pm$0.02  & 14.16$\pm$0.03 & 12.82$\pm$0.02 & 12.08$\pm$0.03 \\
C38178 & J064119.38+092146.9 &  14.98$\pm$0.00 & 14.63$\pm$0.00 & 14.46$\pm$0.00  & 13.77$\pm$0.03 & 13.25$\pm$0.03 & 13.23$\pm$0.04 \\
C38296 & J064119.85+092704.9 &  17.32$\pm$0.00 & 16.50$\pm$0.01 & 15.65$\pm$0.00  & 13.92$\pm$0.03 & 13.21$\pm$0.03 & 13.01$\pm$0.04 \\
C38384 & J064120.22+094908.4 &  19.18$\pm$0.03 & 18.26$\pm$0.03 & 17.19$\pm$0.01  & 15.28$\pm$0.06 & 14.69$\pm$0.05 & 14.43$\pm$0.08 \\
C38449 & J064120.54+094730.1 &  16.38$\pm$0.00 & 15.73$\pm$0.00 & 15.14$\pm$0.00  & 13.63$\pm$0.02 & 12.95$\pm$0.03 & 12.71$\pm$0.03 \\
C38523 & J064120.75+093012.0 &  16.37$\pm$0.00 & 15.62$\pm$0.00 & 15.16$\pm$0.00  & 13.54$\pm$0.03 & 12.90$\pm$0.03 & 12.64$\pm$0.03 \\
C38553 & J064120.86+093444.8 &  19.31$\pm$0.03 & 18.35$\pm$0.04 & 17.20$\pm$0.01  & 15.10$\pm$0.06 & 14.48$\pm$0.06 & 14.31$\pm$0.09 \\
C38598 & J064121.05+093241.6 &  20.17$\pm$0.07 & 19.18$\pm$0.08 & 17.71$\pm$0.02  & 15.25$\pm$0.05 & 14.72$\pm$0.05 & 14.43$\pm$0.08 \\
C38632 & J064121.19+093214.5 &  16.95$\pm$0.00 & 16.19$\pm$0.01 & 15.58$\pm$0.00  & 14.08$\pm$0.03 & 13.40$\pm$0.03 & 13.19$\pm$0.04 \\
C38691 & J064121.48+095301.6 &  20.10$\pm$0.06 & 18.75$\pm$0.05 & 18.34$\pm$0.03  & 15.99$\pm$0.11 & 15.38$\pm$0.10 & 15.19$\pm$0.18 \\
C38841 & J064122.03+092028.4 &  17.80$\pm$0.01 & 17.01$\pm$0.01 & 16.38$\pm$0.01  & 14.80$\pm$0.05 & 14.01$\pm$0.03 & 13.81$\pm$0.05 \\
C39036 & J064122.81+092938.9 &  15.28$\pm$0.00 & 14.88$\pm$0.00 & 14.62$\pm$0.00  & 13.72$\pm$0.03 & 13.12$\pm$0.03 & 12.94$\pm$0.03 \\
C39085 & J064122.98+092930.7 &  18.06$\pm$0.01 & 17.38$\pm$0.02 & 16.65$\pm$0.01  & 15.17$\pm$0.06 & 14.57$\pm$0.05 & 14.27$\pm$0.08 \\
C39139 & J064123.17+093522.7 &  19.68$\pm$0.06 & 18.58$\pm$0.06 & 17.38$\pm$0.02  & 15.03$\pm$0.05 & 14.46$\pm$0.06 & 14.18$\pm$0.07 \\
C39156 & J064123.20+093036.4 &  16.80$\pm$0.00 & 16.00$\pm$0.01 & 15.50$\pm$0.00  & 13.92$\pm$0.03 & 13.20$\pm$0.02 & 13.03$\pm$0.04 \\
C39192 & J064123.34+093804.5 &  19.41$\pm$0.03 & 18.38$\pm$0.04 & 17.33$\pm$0.01  & 15.35$\pm$0.06 & 14.72$\pm$0.07 & 14.71$\pm$0.11 \\
C39235 & J064123.46+094558.6 &  16.07$\pm$0.00 & 15.46$\pm$0.00 & 14.96$\pm$0.00  & 13.52$\pm$0.03 & 12.85$\pm$0.03 & 12.67$\pm$0.03 \\
C39289 & J064123.64+094716.4 &  17.36$\pm$0.01 & 16.59$\pm$0.01 & 15.93$\pm$0.01  & 14.21$\pm$0.03 & 13.60$\pm$0.04 & 13.35$\pm$0.04 \\
C39377 & J064124.02+101432.1 &  16.39$\pm$0.01 & 14.98$\pm$0.01 & 15.26$\pm$0.01  & 14.01$\pm$0.03 & 13.31$\pm$0.03 & 13.10$\pm$0.03 \\
C39439 & J064124.19+094830.9 &  18.13$\pm$0.01 & 16.50$\pm$0.01 & 16.61$\pm$0.01  & 14.69$\pm$0.04 & 14.00$\pm$0.04 & 13.63$\pm$0.05 \\
C39467 & J064124.26+093154.1 &  14.84$\pm$0.00 & 14.41$\pm$0.00 & 14.08$\pm$0.00  & 13.05$\pm$0.02 & 12.40$\pm$0.02 & 12.25$\pm$0.02 \\
C39532 & J064124.55+093735.6 &  16.61$\pm$0.00 & 15.76$\pm$0.00 & 15.13$\pm$0.00  & 13.47$\pm$0.03 & 12.72$\pm$0.02 & 12.56$\pm$0.03 \\
C39676 & J064125.09+093600.2 &  17.75$\pm$0.01 & 16.86$\pm$0.01 & 15.85$\pm$0.00  & 14.03$\pm$0.03 & 13.38$\pm$0.02 & 13.08$\pm$0.04 \\
C39811 & J064125.63+093443.0 &  15.23$\pm$0.00 & 14.42$\pm$0.00 & 14.33$\pm$0.00  & 13.06$\pm$0.02 & 12.39$\pm$0.02 & 12.10$\pm$0.03 \\
C40196 & J064127.00+093013.1 &  16.64$\pm$0.00 & 15.79$\pm$0.00 & 15.31$\pm$0.00  & 13.81$\pm$0.03 & 13.07$\pm$0.03 & 12.88$\pm$0.02 \\
C40291 & J064127.31+093206.5 &  17.94$\pm$0.01 & 17.01$\pm$0.01 & 15.96$\pm$0.01  & 14.02$\pm$0.03 & 13.35$\pm$0.03 & 13.15$\pm$0.04 \\
C40299 & J064127.34+094200.4 &  18.37$\pm$0.01 & 17.37$\pm$0.02 & 16.42$\pm$0.01  & 14.49$\pm$0.03 & 13.91$\pm$0.03 & 13.52$\pm$0.04 \\
C40516 & J064128.09+093249.9 &  18.93$\pm$0.03 & 17.89$\pm$0.03 & 16.90$\pm$0.01  & 14.89$\pm$0.06 & 14.16$\pm$0.07 & 13.96$\pm$0.09 \\
C40687 & J064128.74+092710.8 &  16.73$\pm$0.00 & 16.06$\pm$0.00 & 15.30$\pm$0.00  & 13.63$\pm$0.03 & 12.90$\pm$0.02 & 12.69$\pm$0.03 \\
C40714 & J064128.85+093454.1 &  16.83$\pm$0.00 & 16.10$\pm$0.01 & 15.42$\pm$0.00  & 13.92$\pm$0.03 & 13.17$\pm$0.03 & 12.90$\pm$0.03 \\
C40866 & J064129.45+093918.2 &  16.49$\pm$0.00 & 15.84$\pm$0.01 & 15.31$\pm$0.00  & 13.78$\pm$0.02 & 13.09$\pm$0.02 & 12.90$\pm$0.04 \\
C41332 & J064130.97+092020.1 &  17.99$\pm$0.01 & 17.10$\pm$0.01 & 16.29$\pm$0.01  & 14.56$\pm$0.04 & 13.85$\pm$0.02 & 13.64$\pm$0.05 \\
C41403 & J064131.27+094326.0 &  18.19$\pm$0.02 & 17.20$\pm$0.02 & 16.26$\pm$0.01  & 14.38$\pm$0.07 & 13.65$\pm$0.09 & 13.28$\pm$0.07 \\
C41828 & J064132.50+093807.4 &  14.31$\pm$0.00 & 13.84$\pm$0.00 & 13.48$\pm$0.00  & 12.27$\pm$0.02 & 11.63$\pm$0.02 & 11.47$\pm$0.02 \\
C41880 & J064132.67+094250.8 &  17.89$\pm$0.01 & 15.75$\pm$0.00 & 16.65$\pm$0.01  & 14.74$\pm$0.04 & 14.08$\pm$0.03 & 13.57$\pm$0.05 \\
C42487 & J064134.45+092253.6 &  19.21$\pm$0.02 & 17.76$\pm$0.01 & 17.07$\pm$0.01  & 14.72$\pm$0.04 & 13.99$\pm$0.06 & 13.47$\pm$0.06 \\
C42515 & J064134.56+093632.5 &  16.29$\pm$0.00 & 15.50$\pm$0.00 & 15.14$\pm$0.00  & 13.71$\pm$0.03 & 13.00$\pm$0.02 & 12.81$\pm$0.02 \\
C42845 & J064135.48+091850.3 &  18.38$\pm$0.01 & 17.34$\pm$0.01 & 16.41$\pm$0.01  & 14.46$\pm$0.03 & 13.83$\pm$0.02 & 13.49$\pm$0.04 \\
C42979 & J064135.89+094042.0 &  17.73$\pm$0.01 & 16.87$\pm$0.01 & 16.15$\pm$0.01  & 14.48$\pm$0.04 & 13.76$\pm$0.03 & 13.50$\pm$0.06 \\
C43103 & J064136.23+093920.5 &  15.81$\pm$0.00 & 15.27$\pm$0.00 & 14.90$\pm$0.00  & 13.66$\pm$0.03 & 12.91$\pm$0.03 & 12.82$\pm$0.04 \\
C43537 & J064137.44+093727.9 &  15.65$\pm$0.00 & 15.29$\pm$0.00 & 15.06$\pm$0.00  & 14.23$\pm$0.03 & 13.70$\pm$0.03 & 13.50$\pm$0.05 \\
C44065 & J064138.77+093211.8 &  14.57$\pm$0.00 & 13.50$\pm$0.00 & 13.93$\pm$0.00  & 12.88$\pm$0.03 & 12.11$\pm$0.02 & 11.72$\pm$0.02 \\
C44423 & J064139.60+093319.9 &  16.95$\pm$0.00 & 16.24$\pm$0.00 & 15.63$\pm$0.00  & 14.04$\pm$0.03 & 13.31$\pm$0.03 & 13.10$\pm$0.04 \\
C45081 & J064141.37+093848.6 &  20.35$\pm$0.07 & 18.96$\pm$0.06 & 18.21$\pm$0.03  & 15.14$\pm$0.05 & 14.54$\pm$0.07 & 14.08$\pm$0.07 \\
C45307 & J064141.88+091928.1 &  18.02$\pm$0.01 & 16.57$\pm$0.01 & 16.41$\pm$0.01  & 14.72$\pm$0.04 & 14.03$\pm$0.04 & 13.61$\pm$0.05 \\
C45397 & J064142.17+094225.3 &  18.93$\pm$0.02 & 17.80$\pm$0.03 & 16.70$\pm$0.01  & 14.54$\pm$0.04 & 13.97$\pm$0.04 & 13.78$\pm$0.06 \\
C45710 & J064142.87+092508.4 &  16.05$\pm$0.00 & 14.85$\pm$0.00 & 15.02$\pm$0.00  & 13.57$\pm$0.03 & 12.77$\pm$0.03 & 12.30$\pm$0.03 \\
C45726 & J064142.97+095329.6 &  18.76$\pm$0.02 & 17.79$\pm$0.02 & 16.67$\pm$0.01  & 14.78$\pm$0.05 & 14.06$\pm$0.05 & 13.64$\pm$0.05 \\
C45996 & J064143.59+093941.2 &  17.94$\pm$0.01 & 17.01$\pm$0.02 & 16.11$\pm$0.01  & 14.26$\pm$0.04 & 13.69$\pm$0.04 & 13.34$\pm$0.05 \\
C46131 & J064143.88+090921.2 &  17.68$\pm$0.01 & 17.25$\pm$0.01 & 16.67$\pm$0.01  & 15.20$\pm$0.06 & 14.70$\pm$0.06 & 14.36$\pm$0.09 \\
C46271 & J064144.22+092502.4 &  16.00$\pm$0.00 & 15.26$\pm$0.00 & 14.63$\pm$0.00  & 13.33$\pm$0.03 & 12.61$\pm$0.02 & 12.33$\pm$0.03 \\
C46531 & J064144.94+094440.4 &  14.99$\pm$0.00 & 14.53$\pm$0.00 & 14.22$\pm$0.00  & 13.18$\pm$0.03 & 12.56$\pm$0.03 & 12.38$\pm$0.02 \\
C46679 & J064145.31+094709.0 &  16.81$\pm$0.00 & 16.41$\pm$0.01 & 15.82$\pm$0.00  & 14.46$\pm$0.04 & 13.93$\pm$0.05 & 13.72$\pm$0.06 \\
C46734 & J064145.48+095542.4 &  18.13$\pm$0.01 & 17.19$\pm$0.01 & 16.31$\pm$0.01  & 14.49$\pm$0.04 & 13.90$\pm$0.04 & 13.39$\pm$0.04 \\
C46974 & J064146.03+095437.3 &  18.02$\pm$0.01 & 17.15$\pm$0.01 & 16.35$\pm$0.01  & 14.64$\pm$0.04 & 14.00$\pm$0.04 & 13.73$\pm$0.05 \\
C47486 & J064147.11+093804.7 &  15.23$\pm$0.00 & 14.74$\pm$0.00 & 14.40$\pm$0.00  & 13.19$\pm$0.03 & 12.55$\pm$0.03 & 12.37$\pm$0.03 \\
C47640 & J064147.44+093752.6 &  16.58$\pm$0.00 & 15.92$\pm$0.01 & 15.36$\pm$0.01  & 13.83$\pm$0.02 & 13.13$\pm$0.02 & 12.91$\pm$0.04 \\
C48145 & J064148.60+095411.6 &  15.82$\pm$0.00 & 15.40$\pm$0.00 & 15.15$\pm$0.00  & 14.23$\pm$0.03 & 13.67$\pm$0.04 & 13.50$\pm$0.05 \\
C48240 & J064148.83+100703.0 &  16.12$\pm$0.00 & 15.11$\pm$0.01 & 14.97$\pm$0.01  & 13.28$\pm$0.03 & 12.20$\pm$0.03 & 11.39$\pm$0.02 \\
C48749 & J064149.91+094105.2 &  17.07$\pm$0.00 & 16.70$\pm$0.01 & 16.24$\pm$0.01  & 15.05$\pm$0.05 & 14.60$\pm$0.05 & 14.41$\pm$0.10 \\
C49287 & J064151.13+093012.7 &  18.60$\pm$0.01 & 17.49$\pm$0.02 & 16.85$\pm$0.01  & 14.92$\pm$0.04 & 14.31$\pm$0.05 & 13.91$\pm$0.05 \\
C49334 & J064151.28+094532.4 &  19.49$\pm$0.03 & 18.46$\pm$0.04 & 17.33$\pm$0.02  & 15.19$\pm$0.05 & 14.57$\pm$0.05 & 14.18$\pm$0.07 \\
C50879 & J064154.93+094252.7 &  17.09$\pm$0.00 & 15.18$\pm$0.00 & 15.88$\pm$0.00  & 14.33$\pm$0.03 & 13.64$\pm$0.04 & 13.40$\pm$0.04 \\
C51126 & J064155.41+093019.0 &  16.35$\pm$0.00 & 16.07$\pm$0.01 & 15.51$\pm$0.00  & 14.25$\pm$0.03 & 13.87$\pm$0.03 & 13.60$\pm$0.05 \\
C54567 & J064203.22+093849.5 &  18.76$\pm$0.02 & 16.93$\pm$0.01 & 17.31$\pm$0.01  & 15.10$\pm$0.05 & 14.41$\pm$0.07 & 13.71$\pm$0.05 \\
C57195 & J064208.70+094121.3 &  14.36$\pm$0.00 & 13.28$\pm$0.00 & 13.74$\pm$0.00  & 12.64$\pm$0.03 & 12.04$\pm$0.04 & 11.82$\pm$0.04 \\
C59756 & J064213.69+093900.7 &  18.39$\pm$0.01 & 17.56$\pm$0.01 & 16.90$\pm$0.01  & 14.91$\pm$0.05 & 13.67$\pm$0.03 & 12.85$\pm$0.03 \\
C63956 & J064221.91+094833.1 &  14.86$\pm$0.00 & 14.47$\pm$0.00 & 14.34$\pm$0.00  & 13.63$\pm$0.03 & 13.40$\pm$0.03 & 13.24$\pm$0.03 \\
C8431 & J063950.35+093117.2 &  19.31$\pm$0.04 & 17.75$\pm$0.03 & 17.24$\pm$0.02  & 14.96$\pm$0.05 & 14.43$\pm$0.04 & 13.95$\pm$0.05 \\
C8481 & J063950.33+100813.6 &  18.97$\pm$0.01 & 17.58$\pm$0.02 & 17.19$\pm$0.01  & 15.29$\pm$0.05 & 14.69$\pm$0.05 & 14.31$\pm$0.07 \\
C9452 & J063952.48+095729.0 &  17.34$\pm$0.00 & 16.81$\pm$0.01 & 16.29$\pm$0.01  & 15.02$\pm$0.05 & 14.36$\pm$0.05 & 14.26$\pm$0.08 \\
S2779 & J064059.55+093510.9 &  14.72$\pm$0.00 & 14.13$\pm$0.00 & 13.53$\pm$0.00  & 11.59$\pm$0.03 & 10.70$\pm$0.03 & 10.31$\pm$0.02 \\
S2783 & J064059.68+092843.8 &  15.51$\pm$0.00 & 14.60$\pm$0.00 & 14.54$\pm$0.00  & 13.19$\pm$0.03 & 12.41$\pm$0.03 & 12.08$\pm$0.03 \\
S2791 & J064060.00+092850.0 &  15.28$\pm$0.00 & 14.79$\pm$0.00 & 14.42$\pm$0.00  & 13.09$\pm$0.03 & 12.41$\pm$0.03 & 12.20$\pm$0.03 \\
S2795 & J064100.25+095849.7 &  13.19$\pm$0.00 & 12.84$\pm$0.00 & 12.71$\pm$0.00  & 11.85$\pm$0.02 & 11.36$\pm$0.02 & 11.20$\pm$0.03 \\
S2818 & J064100.79+095122.3 &  14.04$\pm$0.00 & 13.60$\pm$0.00 & 13.28$\pm$0.00  & 12.19$\pm$0.03 & 11.60$\pm$0.03 & 11.40$\pm$0.03 \\
S2985 & J064106.20+093623.0 &  13.05$\pm$0.00 & 12.55$\pm$0.00 & 12.53$\pm$0.00  & 11.64$\pm$0.02 & 11.02$\pm$0.02 & 10.55$\pm$0.02 \\
W1172 & J063932.76+090413.8 &  15.38$\pm$0.00 & 14.49$\pm$0.00 & 14.51$\pm$0.00  & 13.02$\pm$0.03 & 12.19$\pm$0.03 & 11.74$\pm$0.02 \\
W1243 & J063933.40+095201.7 &  15.49$\pm$0.00 & 14.76$\pm$0.00 & 14.28$\pm$0.00  & 12.63$\pm$0.02 & 11.90$\pm$0.02 & 11.66$\pm$0.02 \\
W1322 & J063934.41+095451.2 &  15.77$\pm$0.00 & 15.00$\pm$0.00 & 14.60$\pm$0.00  & 12.99$\pm$0.02 & 12.22$\pm$0.02 & 11.93$\pm$0.02 \\
W1616 & J063939.39+094521.4 &  14.94$\pm$0.00 & 14.24$\pm$0.00 & 14.22$\pm$0.00  & 12.90$\pm$0.03 & 12.04$\pm$0.02 & 11.54$\pm$0.02 \\
W1735 & J063941.47+094619.6 &  14.22$\pm$0.00 & 13.46$\pm$0.00 & 13.65$\pm$0.00  & 12.57$\pm$0.03 & 11.92$\pm$0.02 & 11.69$\pm$0.02 \\
W2320 & J063951.89+101239.4 &  14.52$\pm$0.00 & 13.96$\pm$0.00 & 13.91$\pm$0.00  & 12.89$\pm$0.03 & 12.59$\pm$0.03 & 12.43$\pm$0.03 \\
W2690 & J063959.25+092724.5 &  15.49$\pm$0.00 & 14.69$\pm$0.00 & 14.69$\pm$0.00  & 13.23$\pm$0.03 & 12.46$\pm$0.02 & 12.06$\pm$0.02 \\
W3248 & J064009.61+094143.5 &  12.95$\pm$0.00 & 12.62$\pm$0.00 & 12.43$\pm$0.00  & 11.71$\pm$0.03 & 11.26$\pm$0.03 & 11.01$\pm$0.03 \\
W3407 & J064012.58+100540.6 &  14.98$\pm$0.00 & 14.26$\pm$0.00 & 14.10$\pm$0.00  & 12.51$\pm$0.03 & 11.79$\pm$0.03 & 11.40$\pm$0.03 \\
W3468 & J064014.04+092028.6 &  13.14$\pm$0.00 & 12.80$\pm$0.00 & 12.65$\pm$0.00  & 11.93$\pm$0.03 & 11.47$\pm$0.02 & 11.33$\pm$0.03 \\
W3778 & J064020.09+092828.6 &  15.38$\pm$0.00 & 14.85$\pm$0.00 & 14.52$\pm$0.00  & 13.15$\pm$0.03 & 12.50$\pm$0.03 & 12.24$\pm$0.03 \\
W3814 & J064020.96+092354.3 &  14.72$\pm$0.00 & 14.18$\pm$0.00 & 13.33$\pm$0.00  & 11.08$\pm$0.02 & 10.15$\pm$0.03 & 9.78$\pm$0.02 \\
W3820 & J064021.02+093632.0 &  13.04$\pm$0.00 & 12.70$\pm$0.00 & 12.49$\pm$0.00  & 11.62$\pm$0.02 & 11.16$\pm$0.03 & 11.02$\pm$0.02 \\
W3902 & J064023.09+092742.4 &  15.93$\pm$0.00 & 14.71$\pm$0.00 & 15.07$\pm$0.00  & 13.15$\pm$0.02 & 12.31$\pm$0.02 & 11.77$\pm$0.02 \\
W3905 & J064023.13+095619.8 &  13.10$\pm$0.00 & 12.69$\pm$0.00 & 12.44$\pm$0.00  & 11.46$\pm$0.03 & 10.89$\pm$0.03 & 10.71$\pm$0.02 \\
W4031 & J064026.25+093801.5 &  14.34$\pm$0.00 & 13.78$\pm$0.00 & 13.31$\pm$0.00  & 11.97$\pm$0.02 & 11.21$\pm$0.02 & 11.03$\pm$0.02 \\
W4221 & J064030.61+094610.6 &  14.71$\pm$0.00 & 14.30$\pm$0.00 & 13.99$\pm$0.00  & 12.86$\pm$0.02 & 12.23$\pm$0.02 & 12.06$\pm$0.02 \\
W4267 & J064031.64+094823.3 &  14.96$\pm$0.00 & 13.86$\pm$0.00 & 14.23$\pm$0.00  & 13.02$\pm$0.03 & 12.35$\pm$0.03 & 12.18$\pm$0.02 \\
W4317 & J064032.79+095129.3 &  15.02$\pm$0.00 & 14.49$\pm$0.00 & 14.05$\pm$0.00  & 12.68$\pm$0.03 & 12.00$\pm$0.03 & 11.79$\pm$0.02 \\
W4428 & J064035.18+095156.7 &  15.38$\pm$0.00 & 14.67$\pm$0.00 & 14.16$\pm$0.00  & 12.61$\pm$0.02 & 11.83$\pm$0.02 & 11.47$\pm$0.02 \\
W4459 & J064036.33+091857.6 &  15.00$\pm$0.00 & 14.37$\pm$0.00 & 14.08$\pm$0.00  & 12.71$\pm$0.02 & 12.05$\pm$0.02 & 11.83$\pm$0.02 \\
W4572 & J064039.12+095058.7 &  14.72$\pm$0.00 & 13.85$\pm$0.00 & 13.86$\pm$0.00  & 12.29$\pm$0.03 & 11.25$\pm$0.02 & 10.51$\pm$0.02 \\
W4634 & J064041.01+092754.3 &  15.87$\pm$0.00 & 15.32$\pm$0.00 & 15.03$\pm$0.00  & 13.69$\pm$0.03 & 12.94$\pm$0.04 & 12.67$\pm$0.03 \\
W4654 & J064041.32+095102.4 &  15.07$\pm$0.00 & 14.04$\pm$0.00 & 14.12$\pm$0.00  & 12.81$\pm$0.03 & 12.02$\pm$0.02 & 11.71$\pm$0.02 \\
W4657 & J064041.36+095413.9 &  13.25$\pm$0.00 & 12.81$\pm$0.00 & 12.70$\pm$0.00  & 11.64$\pm$0.03 & 10.95$\pm$0.02 & 10.43$\pm$0.02 \\
W4658 & J064041.42+094809.6 &  15.00$\pm$0.00 & 14.51$\pm$0.00 & 14.17$\pm$0.00  & 12.81$\pm$0.03 & 12.16$\pm$0.02 & 11.97$\pm$0.02 \\
W4722 & J064043.22+094707.3 &  15.43$\pm$0.00 & 14.67$\pm$0.00 & 14.50$\pm$0.00  & 12.80$\pm$0.04 & 12.09$\pm$0.04 & 11.64$\pm$0.05 \\
W4731 & J064043.35+095059.5 &  14.43$\pm$0.00 & 13.99$\pm$0.00 & 13.68$\pm$0.00  & 12.57$\pm$0.03 & 11.95$\pm$0.03 & 11.73$\pm$0.03 \\
W4735 & J064043.43+092840.9 &  15.78$\pm$0.00 & 15.12$\pm$0.00 & 14.66$\pm$0.00  & 13.23$\pm$0.03 & 12.50$\pm$0.03 & 12.36$\pm$0.03 \\
W4790 & J064044.58+094812.6 &  14.72$\pm$0.00 & 14.23$\pm$0.00 & 13.84$\pm$0.00  & 12.58$\pm$0.03 & 11.89$\pm$0.03 & 11.73$\pm$0.03 \\
W4800 & J064044.85+095744.3 &  14.24$\pm$0.00 & 13.77$\pm$0.00 & 13.42$\pm$0.00  & 12.26$\pm$0.03 & 11.57$\pm$0.03 & 11.42$\pm$0.03 \\
W4814 & J064045.17+092844.4 &  13.88$\pm$0.00 & 13.30$\pm$0.00 & 13.27$\pm$0.00  & 12.39$\pm$0.03 & 11.67$\pm$0.02 & 11.35$\pm$0.03 \\
W4904 & J064047.36+094849.4 &  15.28$\pm$0.00 & 14.68$\pm$0.00 & 14.23$\pm$0.00  & 12.82$\pm$0.03 & 12.11$\pm$0.04 & 11.92$\pm$0.03 \\
W4906 & J064047.50+094929.0 &  13.65$\pm$0.00 & 12.96$\pm$0.00 & 12.95$\pm$0.00  & 11.53$\pm$0.03 & 10.67$\pm$0.03 & 10.02$\pm$0.03 \\
W4982 & J064049.29+092350.3 &  15.49$\pm$0.00 & 14.58$\pm$0.00 & 14.54$\pm$0.00  & 13.04$\pm$0.02 & 12.31$\pm$0.02 & 12.04$\pm$0.02 \\
W5004 & J064049.81+094731.1 &  16.05$\pm$0.00 & 15.08$\pm$0.00 & 14.14$\pm$0.00  & 12.28$\pm$0.02 & 11.72$\pm$0.02 & 11.43$\pm$0.02 \\
W5044 & J064050.59+095457.3 &  14.34$\pm$0.00 & 13.67$\pm$0.00 & 13.61$\pm$0.00  & 12.47$\pm$0.02 & 11.69$\pm$0.03 & 11.28$\pm$0.03 \\
W5078 & J064051.35+102805.1 &  14.58$\pm$0.00 & 13.55$\pm$0.00 & 13.29$\pm$0.00  & 11.40$\pm$0.02 & 10.73$\pm$0.03 & 10.12$\pm$0.02 \\
W5088 & J064051.55+094324.3 &  13.88$\pm$0.00 & 13.35$\pm$0.00 & 13.23$\pm$0.00  & 12.36$\pm$0.02 & 11.62$\pm$0.03 & 11.16$\pm$0.03 \\
W5091 & J064051.59+092844.5 &  15.17$\pm$0.00 & 14.30$\pm$0.00 & 14.36$\pm$0.00  & 12.99$\pm$0.03 & 12.20$\pm$0.02 & 11.79$\pm$0.03 \\
W510 & J063922.70+095430.7 &  17.69$\pm$0.01 & 16.45$\pm$0.01 & 16.18$\pm$0.01  & 14.25$\pm$0.03 & 13.64$\pm$0.03 & 13.30$\pm$0.04 \\
W5102 & J064052.01+094504.8 &  15.37$\pm$0.00 & 14.73$\pm$0.00 & 14.18$\pm$0.00  & 12.58$\pm$0.02 & 11.83$\pm$0.02 & 11.64$\pm$0.03 \\
W5237 & J064055.72+095113.8 &  14.97$\pm$0.00 & 14.40$\pm$0.00 & 14.12$\pm$0.00  & 12.87$\pm$0.02 & 12.20$\pm$0.03 & 12.01$\pm$0.03 \\
W5314 & J064057.83+095629.9 &  13.30$\pm$0.00 & 12.95$\pm$0.00 & 12.80$\pm$0.00  & 11.98$\pm$0.02 & 11.46$\pm$0.02 & 11.32$\pm$0.03 \\
W5350 & J064058.92+092852.8 &  16.17$\pm$0.00 & 15.37$\pm$0.00 & 14.66$\pm$0.00  & 13.00$\pm$0.03 & 12.30$\pm$0.02 & 12.05$\pm$0.03 \\
W5367 & J064059.45+095945.4 &  14.82$\pm$0.00 & 14.36$\pm$0.01 & 14.17$\pm$0.01  & 12.78$\pm$0.03 & 12.09$\pm$0.03 & 11.69$\pm$0.02 \\
W5395 & J064100.51+094503.1 &  14.86$\pm$0.00 & 14.29$\pm$0.00 & 14.11$\pm$0.00  & 12.74$\pm$0.02 & 12.02$\pm$0.03 & 11.53$\pm$0.03 \\
W5396 & J064100.51+092915.9 &  15.00$\pm$0.00 & 14.55$\pm$0.00 & 14.14$\pm$0.00  & 12.44$\pm$0.03 & 11.65$\pm$0.03 & 11.22$\pm$0.02 \\
W5405 & J064100.99+093244.5 &  12.83$\pm$0.00 & 12.30$\pm$0.00 & 12.03$\pm$0.00  & 10.58$\pm$0.02 & 9.71$\pm$0.02 & 9.21$\pm$0.02 \\
W5411 & J064101.42+093408.2 &  14.24$\pm$0.00 & 13.82$\pm$0.00 & 13.49$\pm$0.00  & 12.35$\pm$0.03 & 11.71$\pm$0.03 & 11.55$\pm$0.02 \\
W5413 & J064101.53+101456.1 &  15.95$\pm$0.00 & 14.75$\pm$0.00 & 14.63$\pm$0.00  & 12.93$\pm$0.02 & 12.18$\pm$0.03 & 11.66$\pm$0.02 \\
W5427 & J064101.85+093841.2 &  14.12$\pm$0.00 & 13.71$\pm$0.00 & 13.38$\pm$0.00  & 12.24$\pm$0.03 & 11.61$\pm$0.03 & 11.38$\pm$0.03 \\
W5448 & J064102.54+093455.8 &  14.04$\pm$0.00 & 13.65$\pm$0.00 & 13.40$\pm$0.00  & 12.36$\pm$0.03 & 11.82$\pm$0.02 & 11.65$\pm$0.03 \\
W5470 & J064103.28+095755.0 &  15.13$\pm$0.00 & 14.65$\pm$0.01 & 14.32$\pm$0.00  & 13.05$\pm$0.02 & 12.38$\pm$0.02 & 12.24$\pm$0.03 \\
W5491 & J064103.94+095809.5 &  15.78$\pm$0.00 & 15.09$\pm$0.01 & 14.52$\pm$0.01  & 12.99$\pm$0.02 & 12.31$\pm$0.03 & 12.06$\pm$0.03 \\
W5496 & J064104.04+094908.8 &  14.60$\pm$0.00 & 14.11$\pm$0.00 & 13.75$\pm$0.00  & 12.58$\pm$0.02 & 11.91$\pm$0.03 & 11.72$\pm$0.03 \\
W5503 & J064104.18+095202.0 &  14.75$\pm$0.00 & 14.29$\pm$0.00 & 13.96$\pm$0.00  & 12.77$\pm$0.03 & 12.15$\pm$0.03 & 11.95$\pm$0.03 \\
W5506 & J064104.29+092452.2 &  15.36$\pm$0.00 & 14.24$\pm$0.00 & 14.38$\pm$0.00  & 12.72$\pm$0.02 & 11.93$\pm$0.02 & 11.46$\pm$0.02 \\
W5508 & J064104.34+094822.1 &  14.29$\pm$0.00 & 13.89$\pm$0.00 & 13.62$\pm$0.00  & 12.57$\pm$0.02 & 11.99$\pm$0.03 & 11.83$\pm$0.03 \\
W5511 & J064104.44+095126.1 &  14.23$\pm$0.00 & 13.80$\pm$0.00 & 13.52$\pm$0.00  & 12.49$\pm$0.02 & 11.88$\pm$0.02 & 11.71$\pm$0.03 \\
W5512 & J064104.47+095318.4 &  15.22$\pm$0.00 & 14.68$\pm$0.00 & 14.28$\pm$0.00  & 12.98$\pm$0.03 & 12.27$\pm$0.03 & 11.98$\pm$0.03 \\
W5533 & J064104.97+095046.1 &  13.91$\pm$0.00 & 13.46$\pm$0.00 & 13.25$\pm$0.00  & 12.24$\pm$0.02 & 11.54$\pm$0.03 & 11.09$\pm$0.03 \\
W5537 & J064105.10+094848.0 &  15.44$\pm$0.00 & 14.86$\pm$0.00 & 14.33$\pm$0.00  & 12.88$\pm$0.02 & 12.16$\pm$0.02 & 11.94$\pm$0.02 \\
W5538 & J064105.10+095144.5 &  14.66$\pm$0.00 & 14.18$\pm$0.00 & 13.89$\pm$0.00  & 12.74$\pm$0.02 & 12.13$\pm$0.03 & 11.98$\pm$0.03 \\
W5546 & J064105.22+095315.8 &  14.70$\pm$0.00 & 14.18$\pm$0.00 & 13.78$\pm$0.00  & 12.47$\pm$0.02 & 11.82$\pm$0.02 & 11.64$\pm$0.03 \\
W5556 & J064105.69+095418.7 &  15.45$\pm$0.00 & 14.82$\pm$0.00 & 14.29$\pm$0.00  & 12.74$\pm$0.02 & 12.02$\pm$0.03 & 11.84$\pm$0.02 \\
W5560 & J064105.75+093101.3 &  14.80$\pm$0.00 & 14.13$\pm$0.00 & 13.76$\pm$0.00  & 12.37$\pm$0.03 & 11.59$\pm$0.02 & 11.30$\pm$0.02 \\
W5563 & J064105.78+094817.5 &  14.78$\pm$0.00 & 13.99$\pm$0.00 & 13.76$\pm$0.00  & 12.02$\pm$0.02 & 11.26$\pm$0.02 & 10.80$\pm$0.03 \\
W5564 & J064105.82+095247.8 &  15.12$\pm$0.00 & 14.62$\pm$0.00 & 14.22$\pm$0.00  & 12.99$\pm$0.02 & 12.29$\pm$0.02 & 12.07$\pm$0.03 \\
W5567 & J064105.94+092717.4 &  15.81$\pm$0.00 & 14.99$\pm$0.00 & 14.16$\pm$0.00  & 12.27$\pm$0.02 & 11.54$\pm$0.02 & 11.31$\pm$0.02 \\
W5582 & J064106.60+093545.1 &  13.82$\pm$0.00 & 13.55$\pm$0.00 & 13.41$\pm$0.00  & 12.81$\pm$0.02 & 12.50$\pm$0.02 & 12.44$\pm$0.03 \\
W5594 & J064106.85+090216.1 &  15.13$\pm$0.00 & 14.43$\pm$0.00 & 14.11$\pm$0.00  & 12.70$\pm$0.03 & 11.92$\pm$0.02 & 11.65$\pm$0.02 \\
W5604 & J064107.12+091238.3 &  15.36$\pm$0.00 & 14.62$\pm$0.00 & 14.52$\pm$0.00  & 13.07$\pm$0.02 & 12.34$\pm$0.03 & 11.96$\pm$0.02 \\
W5607 & J064107.16+092748.0 &  14.32$\pm$0.00 & 13.81$\pm$0.00 & 13.46$\pm$0.00  & 12.20$\pm$0.02 & 11.54$\pm$0.02 & 11.36$\pm$0.02 \\
W5609 & J064107.27+095831.2 &  14.46$\pm$0.00 & 13.97$\pm$0.00 & 13.73$\pm$0.00  & 12.54$\pm$0.02 & 11.87$\pm$0.02 & 11.68$\pm$0.03 \\
W5620 & J064107.47+101504.5 &  16.88$\pm$0.01 & 15.83$\pm$0.01 & 15.07$\pm$0.01  & 13.24$\pm$0.03 & 12.47$\pm$0.03 & 12.15$\pm$0.02 \\
W5634 & J064107.78+094403.0 &  13.12$\pm$0.00 & 12.81$\pm$0.00 & 12.63$\pm$0.00  & 11.89$\pm$0.02 & 11.51$\pm$0.03 & 11.38$\pm$0.03 \\
W5661 & J064108.83+092343.1 &  14.11$\pm$0.00 & 13.57$\pm$0.00 & 13.19$\pm$0.00  & 11.71$\pm$0.02 & 11.05$\pm$0.02 & 10.85$\pm$0.03 \\
W5680 & J064109.49+095150.0 &  15.21$\pm$0.00 & 14.51$\pm$0.00 & 13.86$\pm$0.00  & 12.34$\pm$0.02 & 11.63$\pm$0.03 & 11.41$\pm$0.03 \\
W5690 & J064109.74+102136.2 &  16.65$\pm$0.01 & 15.67$\pm$0.01 & 14.88$\pm$0.01  & 13.14$\pm$0.02 & 12.38$\pm$0.03 & 12.00$\pm$0.03 \\
W5693 & J064109.83+092712.2 &  13.81$\pm$0.00 & 13.33$\pm$0.00 & 12.96$\pm$0.00  & 11.54$\pm$0.02 & 10.88$\pm$0.02 & 10.64$\pm$0.02 \\
W5697 & J064110.10+091432.4 &  13.01$\pm$0.00 & 12.73$\pm$0.00 & 12.61$\pm$0.00  & 12.01$\pm$0.02 & 11.73$\pm$0.02 & 11.63$\pm$0.02 \\
W5778 & J064112.58+095231.3 &  13.55$\pm$0.00 & 12.82$\pm$0.00 & 12.87$\pm$0.00  & 11.49$\pm$0.03 & 10.69$\pm$0.03 & 10.20$\pm$0.03 \\
W5780 & J064112.83+095243.5 &  14.87$\pm$0.00 & 14.41$\pm$0.00 & 14.08$\pm$0.00  & 12.91$\pm$0.03 & 12.26$\pm$0.03 & 12.09$\pm$0.03 \\
W5801 & J064113.21+092610.4 &  13.81$\pm$0.00 & 12.91$\pm$0.00 & 13.04$\pm$0.00  & 11.61$\pm$0.03 & 10.81$\pm$0.02 & 10.34$\pm$0.02 \\
W5812 & J064113.62+091353.4 &  14.88$\pm$0.00 & 14.38$\pm$0.00 & 14.02$\pm$0.00  & 12.78$\pm$0.03 & 12.08$\pm$0.03 & 11.90$\pm$0.02 \\
W5858 & J064115.43+094639.7 &  13.52$\pm$0.00 & 13.16$\pm$0.00 & 12.93$\pm$0.00  & 12.04$\pm$0.03 & 11.48$\pm$0.03 & 11.42$\pm$0.04 \\
W5870 & J064115.72+093818.3 &  12.79$\pm$0.00 & 12.53$\pm$0.00 & 12.41$\pm$0.00  & 11.88$\pm$0.02 & 11.61$\pm$0.02 & 11.56$\pm$0.03 \\
W5871 & J064115.75+092616.9 &  13.28$\pm$0.00 & 12.81$\pm$0.00 & 12.51$\pm$0.00  & 11.31$\pm$0.03 & 10.67$\pm$0.03 & 10.44$\pm$0.02 \\
W5893 & J064116.69+092952.3 &  13.85$\pm$0.00 & 13.33$\pm$0.00 & 12.91$\pm$0.00  & 11.27$\pm$0.03 & 10.50$\pm$0.02 & 10.07$\pm$0.02 \\
W5895 & J064116.78+092730.2 &  14.39$\pm$0.00 & 13.24$\pm$0.00 & 13.76$\pm$0.00  & 12.65$\pm$0.03 & 11.88$\pm$0.03 & 11.50$\pm$0.03 \\
W5909 & J064117.25+095432.4 &  15.27$\pm$0.00 & 14.35$\pm$0.00 & 14.32$\pm$0.00  & 12.83$\pm$0.02 & 12.05$\pm$0.03 & 11.55$\pm$0.02 \\
W5936 & J064118.28+093353.6 &  14.32$\pm$0.00 & 13.27$\pm$0.00 & 13.63$\pm$0.00  & 12.49$\pm$0.02 & 11.84$\pm$0.02 & 11.61$\pm$0.02 \\
W5962 & J064119.46+093028.6 &  13.48$\pm$0.00 & 13.16$\pm$0.00 & 12.99$\pm$0.00  & 12.29$\pm$0.02 & 11.84$\pm$0.02 & 11.79$\pm$0.03 \\
W5970 & J064119.64+093144.4 &  13.93$\pm$0.00 & 13.48$\pm$0.00 & 13.13$\pm$0.00  & 11.93$\pm$0.02 & 11.28$\pm$0.02 & 11.11$\pm$0.02 \\
W5988 & J064120.55+094535.5 &  14.43$\pm$0.00 & 14.02$\pm$0.00 & 13.75$\pm$0.00  & 12.69$\pm$0.02 & 12.07$\pm$0.02 & 11.98$\pm$0.03 \\
W6027 & J064121.80+094530.9 &  14.81$\pm$0.00 & 14.39$\pm$0.00 & 14.08$\pm$0.00  & 12.95$\pm$0.02 & 12.37$\pm$0.02 & 12.14$\pm$0.02 \\
W6035 & J064122.03+094312.8 &  15.10$\pm$0.00 & 14.65$\pm$0.00 & 14.30$\pm$0.00  & 13.17$\pm$0.02 & 12.49$\pm$0.02 & 12.38$\pm$0.02 \\
W6188 & J064127.16+093506.2 &  13.88$\pm$0.00 & 13.51$\pm$0.00 & 13.26$\pm$0.00  & 12.32$\pm$0.02 & 11.73$\pm$0.02 & 11.59$\pm$0.02 \\
W6235 & J064128.78+093839.0 &  13.67$\pm$0.00 & 13.28$\pm$0.00 & 13.04$\pm$0.00  & 12.10$\pm$0.02 & 11.55$\pm$0.02 & 11.39$\pm$0.02 \\
W6300 & J064131.12+092658.3 &  13.29$\pm$0.00 & 12.40$\pm$0.00 & 12.65$\pm$0.00  & 11.50$\pm$0.03 & 10.69$\pm$0.02 & 10.12$\pm$0.02 \\
W6310 & J064131.60+094832.9 &  14.17$\pm$0.00 & 13.73$\pm$0.00 & 13.47$\pm$0.00  & 12.32$\pm$0.02 & 11.71$\pm$0.03 & 11.55$\pm$0.02 \\
W6501 & J064137.76+090809.4 &  15.02$\pm$0.00 & 14.64$\pm$0.00 & 14.42$\pm$0.00  & 13.50$\pm$0.03 & 12.95$\pm$0.02 & 12.84$\pm$0.03 \\
W6534 & J064138.92+100935.5 &  14.20$\pm$0.00 & 13.42$\pm$0.00 & 13.41$\pm$0.00  & 12.59$\pm$0.03 & 11.92$\pm$0.03 & 11.74$\pm$0.03 \\
W6565 & J064139.74+094028.0 &  13.25$\pm$0.00 & 12.31$\pm$0.00 & 12.60$\pm$0.00  & 11.34$\pm$0.02 & 10.57$\pm$0.02 & 10.07$\pm$0.02 \\
W662 & J063924.66+100831.8 &  18.31$\pm$0.01 & 17.18$\pm$0.01 & 16.29$\pm$0.01  & 14.12$\pm$0.03 & 13.46$\pm$0.03 & 13.10$\pm$0.04 \\
W6647 & J064142.73+094256.6 &  14.61$\pm$0.00 & 14.12$\pm$0.00 & 13.74$\pm$0.00  & 12.52$\pm$0.03 & 11.91$\pm$0.03 & 11.71$\pm$0.03 \\
W6697 & J064143.82+094050.0 &  13.67$\pm$0.00 & 13.15$\pm$0.00 & 13.04$\pm$0.00  & 12.05$\pm$0.03 & 11.26$\pm$0.03 & 10.69$\pm$0.03 \\
W6858 & J064147.80+093409.7 &  14.00$\pm$0.00 & 13.55$\pm$0.00 & 13.20$\pm$0.00  & 12.06$\pm$0.02 & 11.37$\pm$0.02 & 11.15$\pm$0.03 \\
W6871 & J064148.07+094243.3 &  12.77$\pm$0.00 & 12.44$\pm$0.00 & 12.25$\pm$0.00  & 11.55$\pm$0.02 & 11.14$\pm$0.02 & 10.97$\pm$0.02 \\
W6920 & J064149.18+101935.2 &  15.36$\pm$0.00 & 14.57$\pm$0.01 & 14.42$\pm$0.01  & 13.06$\pm$0.03 & 12.27$\pm$0.02 & 11.72$\pm$0.02 \\
W7105 & J064153.16+095047.4 &  15.04$\pm$0.00 & 14.54$\pm$0.00 & 14.22$\pm$0.00  & 12.96$\pm$0.02 & 12.30$\pm$0.02 & 12.00$\pm$0.03 \\
W8957 & J064230.52+090926.2 &  13.38$\pm$0.00 & 12.80$\pm$0.00 & 12.84$\pm$0.00  & 11.60$\pm$0.02 & 11.01$\pm$0.03 & 10.56$\pm$0.02 \\

